Evaluating neural network explanation methods using hybrid documents and morphological agreement

The behavior of deep neural networks (DNNs) is hard to understand. This makes it necessary to explore post hoc explanation methods. We conduct the first comprehensive evaluation of explanation methods for NLP. To this end, we design two novel evaluation paradigms that cover two important classes of NLP problems: small context and large context problems. Both paradigms require no manual annotation and are therefore broadly applicable. We also introduce LIMSSE, an explanation method inspired by LIME that is designed for NLP. We show empirically that LIMSSE, LRP and DeepLIFT are the most effective explanation methods and recommend them for explaining DNNs in NLP.

==> examples/12_CNN_deeplift_short_138.tex <==
{\color[rgb]{0.0,0.0,0.0}{{From}}}
{\color[rgb]{0.0,0.0,0.0}{{:}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{kolstad}}}
{\color[rgb]{0.0443,0.0,0.0}{{@}}}
{\color[rgb]{0.0,0.0407,0.0}{{cae.wisc.edu}}}
{\color[rgb]{0.0989,0.0,0.0}{{(}}}
{\color[rgb]{0.0094,0.0,0.0}{{Joel}}}
{\color[rgb]{0.0,0.9091,0.0}{\textbf{Kolstad}}}
{\color[rgb]{0.2735,0.0,0.0}{{)}}}
{\color[rgb]{0.0323,0.0,0.0}{{Subject}}}
{\color[rgb]{0.0839,0.0,0.0}{{:}}}
{\color[rgb]{0.0,0.02,0.0}{{Re}}}
{\color[rgb]{0.0161,0.0,0.0}{{:}}}
{\color[rgb]{0.0083,0.0,0.0}{{Can}}}
{\color[rgb]{0.0,0.0773,0.0}{\underline{Radio}}}
{\color[rgb]{0.0,0.1039,0.0}{\underline{Freq}}}
{\color[rgb]{0.0271,0.0,0.0}{{.}}}
{\color[rgb]{0.0394,0.0,0.0}{{Be}}}
{\color[rgb]{0.0,0.0323,0.0}{{Used}}}
{\color[rgb]{0.0,0.0163,0.0}{{To}}}
{\color[rgb]{0.1371,0.0,0.0}{{Measure}}}
{\color[rgb]{0.0,0.0057,0.0}{{Distance}}}
{\color[rgb]{0.014,0.0,0.0}{{?}}}
[...]
{\color[rgb]{0.0,0.0,0.0}{{What}}}
{\color[rgb]{0.0,0.0,0.0}{{is}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{difference}}}
{\color[rgb]{0.0,0.0,0.0}{{between}}}
{\color[rgb]{0.0,0.0,0.0}{{vertical}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0279,0.0}{{horizontal}}}
{\color[rgb]{0.0024,0.0,0.0}{{?}}}
{\color[rgb]{0.0189,0.0,0.0}{{Gravity}}}
{\color[rgb]{0.0768,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0252,0.0}{{Does}}}
{\color[rgb]{0.0,0.015,0.0}{{n't}}}
{\color[rgb]{0.0,0.1405,0.0}{{gravity}}}
{\color[rgb]{0.0432,0.0,0.0}{{pull}}}
{\color[rgb]{0.0021,0.0,0.0}{{down}}}
{\color[rgb]{0.0318,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.1324,0.0}{\underline{photons}}}
{\color[rgb]{0.0397,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0043,0.0}{{cause}}}
{\color[rgb]{0.0184,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.0,0.0}\textit{\underline{doppler}}}
{\color[rgb]{0.0,0.0,0.0}{\underline{shift}}}
{\color[rgb]{0.0,0.0,0.0}{{or}}}
{\color[rgb]{0.0,0.0,0.0}{{something}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{(}}}
{\color[rgb]{0.0,0.0,0.0}{{Just}}}
{\color[rgb]{0.0,0.0,0.0}{{kidding}}}
{\color[rgb]{0.0,0.0,0.0}{{!}}}
{\color[rgb]{0.0,0.0,0.0}{{)}}}


==> examples/12_CNN_omission-5_138.tex <==
{\color[rgb]{0.1104,0.0,0.0}{{From}}}
{\color[rgb]{0.0765,0.0,0.0}{{:}}}
{\color[rgb]{0.1718,0.0,0.0}\textit{{kolstad}}}
{\color[rgb]{0.0,0.001,0.0}{{@}}}
{\color[rgb]{0.0,0.1828,0.0}{{cae.wisc.edu}}}
{\color[rgb]{0.0,0.464,0.0}{{(}}}
{\color[rgb]{0.0,0.5925,0.0}{{Joel}}}
{\color[rgb]{0.0,0.9091,0.0}{\textbf{Kolstad}}}
{\color[rgb]{0.0,0.7323,0.0}{{)}}}
{\color[rgb]{0.0,0.3462,0.0}{{Subject}}}
{\color[rgb]{0.0,0.1048,0.0}{{:}}}
{\color[rgb]{0.0068,0.0,0.0}{{Re}}}
{\color[rgb]{0.1395,0.0,0.0}{{:}}}
{\color[rgb]{0.0485,0.0,0.0}{{Can}}}
{\color[rgb]{0.0,0.297,0.0}{\underline{Radio}}}
{\color[rgb]{0.0,0.5545,0.0}{\underline{Freq}}}
{\color[rgb]{0.0,0.3607,0.0}{{.}}}
{\color[rgb]{0.0,0.2074,0.0}{{Be}}}
{\color[rgb]{0.0,0.1048,0.0}{{Used}}}
{\color[rgb]{0.1368,0.0,0.0}{{To}}}
{\color[rgb]{0.3385,0.0,0.0}{{Measure}}}
{\color[rgb]{0.0253,0.0,0.0}{{Distance}}}
{\color[rgb]{0.0,0.1821,0.0}{{?}}}
{\color[rgb]{0.0,0.1939,0.0}{{Organization}}}
{\color[rgb]{0.0,0.4772,0.0}{{:}}}
{\color[rgb]{0.0,0.4915,0.0}{{U}}}
{\color[rgb]{0.0,0.3175,0.0}{{of}}}
{\color[rgb]{0.0,0.1749,0.0}\textit{{Wisconsin-Madison}}}
{\color[rgb]{0.0,0.1787,0.0}{{College}}}
{\color[rgb]{0.0,0.0006,0.0}{{of}}}
{\color[rgb]{0.0,0.0072,0.0}{{Engineering}}}
{\color[rgb]{0.0,0.0116,0.0}{{Lines}}}
{\color[rgb]{0.0,0.0311,0.0}{{:}}}
{\color[rgb]{0.0,0.0322,0.0}{{12}}}
{\color[rgb]{0.0,0.0273,0.0}{{In}}}
{\color[rgb]{0.0,0.0369,0.0}{{article}}}
{\color[rgb]{0.0,0.0553,0.0}{{$<$}}}
{\color[rgb]{0.0,0.0289,0.0}\textit{{72020037}}}
{\color[rgb]{0.0,0.0278,0.0}{{@}}}
{\color[rgb]{0.0,0.0229,0.0}\textit{{otter.hpl.hp.com}}}
{\color[rgb]{0.0,0.0274,0.0}{{$>$}}}
{\color[rgb]{0.0,0.0385,0.0}\textit{{tgg}}}
{\color[rgb]{0.0,0.0756,0.0}{{@}}}
{\color[rgb]{0.0,0.1493,0.0}\textit{{otter.hpl.hp.com}}}
{\color[rgb]{0.0,0.1428,0.0}{{(}}}
{\color[rgb]{0.0,0.1117,0.0}{{Tom}}}
{\color[rgb]{0.0,0.071,0.0}{{Gardner}}}
{\color[rgb]{0.0,0.0777,0.0}{{)}}}
{\color[rgb]{0.0075,0.0,0.0}{{writes}}}
{\color[rgb]{0.0,0.1023,0.0}{{:}}}
{\color[rgb]{0.0,0.1496,0.0}{{$>$}}}
{\color[rgb]{0.0,0.1648,0.0}{{What}}}
{\color[rgb]{0.0,0.1285,0.0}{{is}}}
{\color[rgb]{0.0,0.1978,0.0}{{the}}}
{\color[rgb]{0.0,0.1546,0.0}{{difference}}}
{\color[rgb]{0.0,0.2759,0.0}{{between}}}
{\color[rgb]{0.0,0.2824,0.0}{{vertical}}}
{\color[rgb]{0.0,0.2586,0.0}{{and}}}
{\color[rgb]{0.0,0.2208,0.0}{{horizontal}}}
{\color[rgb]{0.0,0.3389,0.0}{{?}}}
{\color[rgb]{0.0,0.2099,0.0}{{Gravity}}}
{\color[rgb]{0.0,0.3767,0.0}{{?}}}
{\color[rgb]{0.0,0.4626,0.0}{{Does}}}
{\color[rgb]{0.0,0.4551,0.0}{{n't}}}
{\color[rgb]{0.0,0.313,0.0}{{gravity}}}
{\color[rgb]{0.0,0.4478,0.0}{{pull}}}
{\color[rgb]{0.0,0.3375,0.0}{{down}}}
{\color[rgb]{0.0,0.3471,0.0}{{the}}}
{\color[rgb]{0.0,0.4473,0.0}{\underline{photons}}}
{\color[rgb]{0.0,0.3579,0.0}{{and}}}
{\color[rgb]{0.0,0.1933,0.0}{{cause}}}
{\color[rgb]{0.0,0.1216,0.0}{{a}}}
{\color[rgb]{0.0,0.0488,0.0}\textit{\underline{doppler}}}
{\color[rgb]{0.0493,0.0,0.0}{\underline{shift}}}
{\color[rgb]{0.0,0.053,0.0}{{or}}}
{\color[rgb]{0.0,0.0543,0.0}{{something}}}
{\color[rgb]{0.0,0.0581,0.0}{{?}}}
{\color[rgb]{0.0,0.0585,0.0}{{(}}}
{\color[rgb]{0.0,0.0441,0.0}{{Just}}}
{\color[rgb]{0.0,0.0,0.0}{{kidding}}}
{\color[rgb]{0.0,0.0,0.0}{{!}}}
{\color[rgb]{0.0,0.0,0.0}{{)}}}


==> examples/13_GRU_omission-5_7.tex <==
{\color[rgb]{0.0083,0.0,0.0}{{From}}}
{\color[rgb]{0.0126,0.0,0.0}{{:}}}
{\color[rgb]{0.017,0.0,0.0}\textit{{chorley}}}
{\color[rgb]{0.0901,0.0,0.0}{{@}}}
{\color[rgb]{0.1673,0.0,0.0}\textit{{vms.ocom.okstate.edu}}}
{\color[rgb]{0.3343,0.0,0.0}{{Subject}}}
{\color[rgb]{0.5218,0.0,0.0}{{:}}}
{\color[rgb]{0.7085,0.0,0.0}{{CS}}}
{\color[rgb]{0.5763,0.0,0.0}{{``}}}
{\color[rgb]{0.4375,0.0,0.0}{{gas}}}
{\color[rgb]{0.0986,0.0,0.0}{{''}}}
{\color[rgb]{0.0,0.2752,0.0}{{and}}}
{\color[rgb]{0.0,0.6297,0.0}{\underline{allergic}}}
{\color[rgb]{0.0,0.5648,0.0}\textit{{response-}}}
{\color[rgb]{0.0,0.4977,0.0}\textit{{Ques}}}
{\color[rgb]{0.0,0.2949,0.0}{{.}}}
{\color[rgb]{0.0,0.0737,0.0}{{Lines}}}
{\color[rgb]{0.1229,0.0,0.0}{{:}}}
{\color[rgb]{0.1495,0.0,0.0}{{6}}}
{\color[rgb]{0.1806,0.0,0.0}{{Nntp-Posting-Host}}}
{\color[rgb]{0.1685,0.0,0.0}{{:}}}
{\color[rgb]{0.1558,0.0,0.0}\textit{{vms.ocom.okstate.edu}}}
{\color[rgb]{0.1422,0.0,0.0}{{Organization}}}
{\color[rgb]{0.0383,0.0,0.0}{{:}}}
{\color[rgb]{0.0,0.2018,0.0}{{OSU}}}
{\color[rgb]{0.0,0.44,0.0}{{College}}}
{\color[rgb]{0.0,0.6684,0.0}{{of}}}
{\color[rgb]{0.0,0.9007,0.0}{\underline{Osteopathic}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline{Medicine}}}
{\color[rgb]{0.0,0.6653,0.0}{{This}}}
{\color[rgb]{0.0,0.4155,0.0}{{question}}}
{\color[rgb]{0.0,0.1576,0.0}{{derives}}}
{\color[rgb]{0.08,0.0,0.0}{{from}}}
{\color[rgb]{0.1835,0.0,0.0}{{the}}}
{\color[rgb]{0.1747,0.0,0.0}{{Waco}}}
{\color[rgb]{0.1647,0.0,0.0}{{incident}}}
{\color[rgb]{0.129,0.0,0.0}{{:}}}
{\color[rgb]{0.1593,0.0,0.0}{{Could}}}
{\color[rgb]{0.1907,0.0,0.0}{{CS}}}
{\color[rgb]{0.1997,0.0,0.0}{{(}}}
{\color[rgb]{0.2179,0.0,0.0}{{``}}}
{\color[rgb]{0.2407,0.0,0.0}{{gas}}}
{\color[rgb]{0.1854,0.0,0.0}{{''}}}
{\color[rgb]{0.0506,0.0,0.0}{{)}}}
{\color[rgb]{0.0,0.0692,0.0}{{particles}}}
{\color[rgb]{0.0,0.1966,0.0}{{create}}}
{\color[rgb]{0.0,0.3216,0.0}{{an}}}
{\color[rgb]{0.0,0.4045,0.0}{\underline{allergic}}}
{\color[rgb]{0.0,0.3303,0.0}{{response}}}
{\color[rgb]{0.0,0.2563,0.0}{{which}}}
{\color[rgb]{0.0,0.1786,0.0}{{would}}}
{\color[rgb]{0.0,0.0991,0.0}{{result}}}
{\color[rgb]{0.0,0.0157,0.0}{{in}}}
{\color[rgb]{0.0,0.0106,0.0}\textit{\underline{laryngospasm}}}
{\color[rgb]{0.0,0.0051,0.0}{{and}}}
{\color[rgb]{0.0,0.0021,0.0}\textit{\underline{asphyxiation}}}
{\color[rgb]{0.0038,0.0,0.0}{{?}}}
{\color[rgb]{0.0065,0.0,0.0}{{-}}}
{\color[rgb]{0.0096,0.0,0.0}{{especially}}}
{\color[rgb]{0.0116,0.0,0.0}{{in}}}
{\color[rgb]{0.0935,0.0,0.0}{{children}}}
{\color[rgb]{0.1698,0.0,0.0}{{.}}}
{\color[rgb]{0.247,0.0,0.0}\textit{{DNC}}}
{\color[rgb]{0.3247,0.0,0.0}{{in}}}
{\color[rgb]{0.4024,0.0,0.0}{{Ok.}}}
{\color[rgb]{0.3176,0.0,0.0}\textit{{OSU-COM}}}
{\color[rgb]{0.2384,0.0,0.0}{{will}}}
{\color[rgb]{0.1601,0.0,0.0}\textit{{disavow}}}
{\color[rgb]{0.0829,0.0,0.0}{{my}}}
{\color[rgb]{0.0071,0.0,0.0}{{opinion}}}
{\color[rgb]{0.018,0.0,0.0}{{,}}}
{\color[rgb]{0.0232,0.0,0.0}{{and}}}
{\color[rgb]{0.0465,0.0,0.0}{{my}}}
{\color[rgb]{0.053,0.0,0.0}{{existence}}}
{\color[rgb]{0.0489,0.0,0.0}{{,}}}
{\color[rgb]{0.0406,0.0,0.0}{{if}}}
{\color[rgb]{0.0348,0.0,0.0}{{necessary}}}
{\color[rgb]{0.0095,0.0,0.0}{{.}}}


==> examples/CNN_newsgroup_deeplift_3737.tex <==
{\color[rgb]{0.1705,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.037,0.0}{{.}}}
{\color[rgb]{0.0,0.0365,0.0}{{Children}}}
{\color[rgb]{0.0454,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0274,0.0}{{tiny}}}
{\color[rgb]{0.0,0.149,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.095,0.0}{{passages}}}
{\color[rgb]{0.0127,0.0,0.0}{{which}}}
{\color[rgb]{0.0227,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.001,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0166,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2146,0.0,0.0}{{,}}}
{\color[rgb]{0.2083,0.0,0.0}{{or}}}
{\color[rgb]{0.0369,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.2082,0.0}{{disease}}}
{\color[rgb]{0.0083,0.0,0.0}{{.}}}
{\color[rgb]{0.009,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0034,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0059,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0023,0.0}{{Thanks}}}
{\color[rgb]{0.0181,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0033,0.0}{{...}}}
{\color[rgb]{0.0056,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0109,0.0}{{bases}}}
{\color[rgb]{0.0145,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.028,0.0}{{interpretation}}}
{\color[rgb]{0.0184,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.08,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.012,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0297,0.0}{{to}}}
{\color[rgb]{0.0,0.0332,0.0}{{my}}}
{\color[rgb]{0.0,0.0145,0.0}{{own}}}
{\color[rgb]{0.1711,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.003,0.0}{{n't}}}
{\color[rgb]{0.0,0.0182,0.0}{{possibly}}}
{\color[rgb]{0.028,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0126,0.0}{{up}}}
{\color[rgb]{0.0,0.0111,0.0}{{your}}}
{\color[rgb]{0.1065,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0136,0.0}{{.}}}
{\color[rgb]{0.0,0.0519,0.0}{{If}}}
{\color[rgb]{0.0,0.0309,0.0}{{these}}}
{\color[rgb]{0.0,0.0374,0.0}{{people}}}
{\color[rgb]{0.0,0.0146,0.0}{{are}}}
{\color[rgb]{0.2629,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0002,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0076,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0137,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0015,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_prob_dot_3737.tex <==
{\color[rgb]{0.0,0.1837,0.0}{{settings}}}
{\color[rgb]{0.018,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0406,0.0}{{Children}}}
{\color[rgb]{0.055,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0024,0.0}{{tiny}}}
{\color[rgb]{0.0,0.1599,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.0481,0.0}{{passages}}}
{\color[rgb]{0.0079,0.0,0.0}{{which}}}
{\color[rgb]{0.0245,0.0,0.0}{{are}}}
{\color[rgb]{0.0003,0.0,0.0}{{easily}}}
{\color[rgb]{0.0063,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0158,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2246,0.0,0.0}{{,}}}
{\color[rgb]{0.2239,0.0,0.0}{{or}}}
{\color[rgb]{0.0393,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.2119,0.0}{{disease}}}
{\color[rgb]{0.0097,0.0,0.0}{{.}}}
{\color[rgb]{0.0106,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0047,0.0}{\underline{J}}}
{\color[rgb]{0.0081,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0031,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0248,0.0}{{MS}}}
{\color[rgb]{0.0045,0.0,0.0}{{...}}}
{\color[rgb]{0.0,0.0088,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0007,0.0,0.0}{{bases}}}
{\color[rgb]{0.0,0.0064,0.0}{{his}}}
{\color[rgb]{0.0336,0.0,0.0}{{interpretation}}}
{\color[rgb]{0.0005,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.0284,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0089,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0652,0.0}{{to}}}
{\color[rgb]{0.0,0.0842,0.0}{{my}}}
{\color[rgb]{0.0,0.043,0.0}{{own}}}
{\color[rgb]{0.3842,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0003,0.0}{{n't}}}
{\color[rgb]{0.0,0.0076,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0191,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0009,0.0}{{up}}}
{\color[rgb]{0.0,0.0083,0.0}{{your}}}
{\color[rgb]{0.0465,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.004,0.0}{{.}}}
{\color[rgb]{0.0,0.0847,0.0}{{If}}}
{\color[rgb]{0.0,0.0689,0.0}{{these}}}
{\color[rgb]{0.0,0.0785,0.0}{{people}}}
{\color[rgb]{0.0,0.0344,0.0}{{are}}}
{\color[rgb]{0.628,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0259,0.0}{{,}}}
{\color[rgb]{0.0011,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0071,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0141,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.025,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0014,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_prob_dot_integrated_3737.tex <==
{\color[rgb]{0.0,0.0795,0.0}{{settings}}}
{\color[rgb]{0.0127,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0256,0.0}{{Children}}}
{\color[rgb]{0.0425,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0141,0.0}{{tiny}}}
{\color[rgb]{0.0,0.1434,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.0801,0.0}{{passages}}}
{\color[rgb]{0.0115,0.0,0.0}{{which}}}
{\color[rgb]{0.0265,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0002,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0175,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2145,0.0,0.0}{{,}}}
{\color[rgb]{0.207,0.0,0.0}{{or}}}
{\color[rgb]{0.0382,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.1921,0.0}{{disease}}}
{\color[rgb]{0.0063,0.0,0.0}{{.}}}
{\color[rgb]{0.0068,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0011,0.0}{\underline{J}}}
{\color[rgb]{0.002,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0008,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.006,0.0}{{MS}}}
{\color[rgb]{0.0011,0.0,0.0}{{...}}}
{\color[rgb]{0.0034,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0085,0.0}{{bases}}}
{\color[rgb]{0.0086,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.0147,0.0}{{interpretation}}}
{\color[rgb]{0.0129,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.0587,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0099,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0349,0.0}{{to}}}
{\color[rgb]{0.0,0.043,0.0}{{my}}}
{\color[rgb]{0.0,0.0205,0.0}{{own}}}
{\color[rgb]{0.2041,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0004,0.0}{{n't}}}
{\color[rgb]{0.0,0.0091,0.0}{{possibly}}}
{\color[rgb]{0.0027,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0035,0.0}{{up}}}
{\color[rgb]{0.0,0.006,0.0}{{your}}}
{\color[rgb]{0.0419,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0059,0.0}{{.}}}
{\color[rgb]{0.0,0.06,0.0}{{If}}}
{\color[rgb]{0.0,0.0426,0.0}{{these}}}
{\color[rgb]{0.0,0.0482,0.0}{{people}}}
{\color[rgb]{0.0,0.0216,0.0}{{are}}}
{\color[rgb]{0.3708,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0091,0.0}{{,}}}
{\color[rgb]{0.0004,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0025,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0066,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0126,0.0}{{valuable}}}
{\color[rgb]{0.0,0.003,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_prob_l2_3737.tex <==
{\color[rgb]{0.0,0.3926,0.0}{{settings}}}
{\color[rgb]{0.0,0.3497,0.0}{{.}}}
{\color[rgb]{0.0,0.4275,0.0}{{Children}}}
{\color[rgb]{0.0,0.352,0.0}{{have}}}
{\color[rgb]{0.0,0.3802,0.0}{{tiny}}}
{\color[rgb]{0.0,0.37,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.3178,0.0}{{passages}}}
{\color[rgb]{0.0,0.2569,0.0}{{which}}}
{\color[rgb]{0.0,0.2205,0.0}{{are}}}
{\color[rgb]{0.0,0.0961,0.0}{{easily}}}
{\color[rgb]{0.0,0.104,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.08,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.6532,0.0}{{,}}}
{\color[rgb]{0.0,0.6726,0.0}{{or}}}
{\color[rgb]{0.0,0.6674,0.0}{{heart}}}
{\color[rgb]{0.0,0.7635,0.0}{{disease}}}
{\color[rgb]{0.0,0.082,0.0}{{.}}}
{\color[rgb]{0.0,0.0903,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0665,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0588,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0592,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0721,0.0}{{MS}}}
{\color[rgb]{0.0,0.0572,0.0}{{...}}}
{\color[rgb]{0.0,0.0569,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.1064,0.0}{{bases}}}
{\color[rgb]{0.0,0.0981,0.0}{{his}}}
{\color[rgb]{0.0,0.1146,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.1004,0.0}{{on}}}
{\color[rgb]{0.0,0.1078,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0,0.4162,0.0}{{blind}}}
{\color[rgb]{0.0,0.3766,0.0}{{to}}}
{\color[rgb]{0.0,0.3884,0.0}{{my}}}
{\color[rgb]{0.0,0.3639,0.0}{{own}}}
{\color[rgb]{0.0,0.4885,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.003,0.0}{{n't}}}
{\color[rgb]{0.0,0.0461,0.0}{{possibly}}}
{\color[rgb]{0.0,0.1279,0.0}{{screwed}}}
{\color[rgb]{0.0,0.1716,0.0}{{up}}}
{\color[rgb]{0.0,0.197,0.0}{{your}}}
{\color[rgb]{0.0,0.2337,0.0}{{engine}}}
{\color[rgb]{0.0,0.1809,0.0}{{.}}}
{\color[rgb]{0.0,0.4437,0.0}{{If}}}
{\color[rgb]{0.0,0.3664,0.0}{{these}}}
{\color[rgb]{0.0,0.4078,0.0}{{people}}}
{\color[rgb]{0.0,0.3899,0.0}{{are}}}
{\color[rgb]{0.0,0.7159,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0938,0.0}{{,}}}
{\color[rgb]{0.0,0.0879,0.0}{{does}}}
{\color[rgb]{0.0,0.0998,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.1308,0.0}{{less}}}
{\color[rgb]{0.0,0.1143,0.0}{{valuable}}}
{\color[rgb]{0.0,0.1106,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_prob_l2_integrated_3737.tex <==
{\color[rgb]{0.0,0.2324,0.0}{{settings}}}
{\color[rgb]{0.0,0.2046,0.0}{{.}}}
{\color[rgb]{0.0,0.3008,0.0}{{Children}}}
{\color[rgb]{0.0,0.2956,0.0}{{have}}}
{\color[rgb]{0.0,0.3475,0.0}{{tiny}}}
{\color[rgb]{0.0,0.3652,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.3589,0.0}{{passages}}}
{\color[rgb]{0.0,0.2567,0.0}{{which}}}
{\color[rgb]{0.0,0.1935,0.0}{{are}}}
{\color[rgb]{0.0,0.0038,0.0}{{easily}}}
{\color[rgb]{0.0,0.0041,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.0919,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.6499,0.0}{{,}}}
{\color[rgb]{0.0,0.6503,0.0}{{or}}}
{\color[rgb]{0.0,0.654,0.0}{{heart}}}
{\color[rgb]{0.0,0.7195,0.0}{{disease}}}
{\color[rgb]{0.0,0.0549,0.0}{{.}}}
{\color[rgb]{0.0,0.0605,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0168,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0148,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0149,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0182,0.0}{{MS}}}
{\color[rgb]{0.0,0.0144,0.0}{{...}}}
{\color[rgb]{0.0,0.0225,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.1383,0.0}{{bases}}}
{\color[rgb]{0.0,0.1265,0.0}{{his}}}
{\color[rgb]{0.0,0.1639,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.1268,0.0}{{on}}}
{\color[rgb]{0.0,0.1664,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0,0.2347,0.0}{{blind}}}
{\color[rgb]{0.0,0.219,0.0}{{to}}}
{\color[rgb]{0.0,0.2047,0.0}{{my}}}
{\color[rgb]{0.0,0.2122,0.0}{{own}}}
{\color[rgb]{0.0,0.2668,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0043,0.0}{{n't}}}
{\color[rgb]{0.0,0.0458,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0592,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0858,0.0}{{up}}}
{\color[rgb]{0.0,0.1031,0.0}{{your}}}
{\color[rgb]{0.0,0.1235,0.0}{{engine}}}
{\color[rgb]{0.0,0.0733,0.0}{{.}}}
{\color[rgb]{0.0,0.2841,0.0}{{If}}}
{\color[rgb]{0.0,0.2312,0.0}{{these}}}
{\color[rgb]{0.0,0.2594,0.0}{{people}}}
{\color[rgb]{0.0,0.234,0.0}{{are}}}
{\color[rgb]{0.0,0.4314,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.034,0.0}{{,}}}
{\color[rgb]{0.0,0.0319,0.0}{{does}}}
{\color[rgb]{0.0,0.0362,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0834,0.0}{{less}}}
{\color[rgb]{0.0,0.0725,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0701,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_raw_dot_3737.tex <==
{\color[rgb]{0.2142,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.0603,0.0}{{.}}}
{\color[rgb]{0.0,0.0466,0.0}{{Children}}}
{\color[rgb]{0.0538,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0261,0.0}{{tiny}}}
{\color[rgb]{0.0,0.1612,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.0899,0.0}{{passages}}}
{\color[rgb]{0.0105,0.0,0.0}{{which}}}
{\color[rgb]{0.0211,0.0,0.0}{{are}}}
{\color[rgb]{0.0002,0.0,0.0}{{easily}}}
{\color[rgb]{0.0054,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0186,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2278,0.0,0.0}{{,}}}
{\color[rgb]{0.2247,0.0,0.0}{{or}}}
{\color[rgb]{0.0301,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.2372,0.0}{{disease}}}
{\color[rgb]{0.0122,0.0,0.0}{{.}}}
{\color[rgb]{0.0132,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0035,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.006,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0023,0.0}{{Thanks}}}
{\color[rgb]{0.0185,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0034,0.0}{{...}}}
{\color[rgb]{0.0057,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0115,0.0}{{bases}}}
{\color[rgb]{0.0145,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.0287,0.0}{{interpretation}}}
{\color[rgb]{0.0195,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.0836,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0109,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0321,0.0}{{to}}}
{\color[rgb]{0.0,0.0363,0.0}{{my}}}
{\color[rgb]{0.0,0.014,0.0}{{own}}}
{\color[rgb]{0.1812,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.006,0.0}{{n't}}}
{\color[rgb]{0.0,0.0297,0.0}{{possibly}}}
{\color[rgb]{0.0385,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0294,0.0}{{up}}}
{\color[rgb]{0.0,0.0158,0.0}{{your}}}
{\color[rgb]{0.1602,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0193,0.0}{{.}}}
{\color[rgb]{0.0,0.0564,0.0}{{If}}}
{\color[rgb]{0.0,0.0312,0.0}{{these}}}
{\color[rgb]{0.0,0.0398,0.0}{{people}}}
{\color[rgb]{0.0,0.0149,0.0}{{are}}}
{\color[rgb]{0.2662,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0002,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0001,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0145,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0242,0.0}{{valuable}}}
{\color[rgb]{0.0017,0.0,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_raw_dot_integrated_3737.tex <==
{\color[rgb]{0.1707,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.037,0.0}{{.}}}
{\color[rgb]{0.0,0.0367,0.0}{{Children}}}
{\color[rgb]{0.0455,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0273,0.0}{{tiny}}}
{\color[rgb]{0.0,0.1489,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.095,0.0}{{passages}}}
{\color[rgb]{0.0127,0.0,0.0}{{which}}}
{\color[rgb]{0.0226,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.001,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0167,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2148,0.0,0.0}{{,}}}
{\color[rgb]{0.2085,0.0,0.0}{{or}}}
{\color[rgb]{0.0368,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.2084,0.0}{{disease}}}
{\color[rgb]{0.0083,0.0,0.0}{{.}}}
{\color[rgb]{0.009,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0034,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0059,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0023,0.0}{{Thanks}}}
{\color[rgb]{0.018,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0033,0.0}{{...}}}
{\color[rgb]{0.0056,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0109,0.0}{{bases}}}
{\color[rgb]{0.0145,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.028,0.0}{{interpretation}}}
{\color[rgb]{0.0184,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.0799,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.012,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0298,0.0}{{to}}}
{\color[rgb]{0.0,0.0333,0.0}{{my}}}
{\color[rgb]{0.0,0.0145,0.0}{{own}}}
{\color[rgb]{0.1714,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.003,0.0}{{n't}}}
{\color[rgb]{0.0,0.0182,0.0}{{possibly}}}
{\color[rgb]{0.028,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0127,0.0}{{up}}}
{\color[rgb]{0.0,0.0111,0.0}{{your}}}
{\color[rgb]{0.1067,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0136,0.0}{{.}}}
{\color[rgb]{0.0,0.0518,0.0}{{If}}}
{\color[rgb]{0.0,0.0309,0.0}{{these}}}
{\color[rgb]{0.0,0.0375,0.0}{{people}}}
{\color[rgb]{0.0,0.0146,0.0}{{are}}}
{\color[rgb]{0.263,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0002,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0076,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0137,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0015,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_raw_l2_3737.tex <==
{\color[rgb]{0.0,0.4119,0.0}{{settings}}}
{\color[rgb]{0.0,0.3277,0.0}{{.}}}
{\color[rgb]{0.0,0.4132,0.0}{{Children}}}
{\color[rgb]{0.0,0.3113,0.0}{{have}}}
{\color[rgb]{0.0,0.3986,0.0}{{tiny}}}
{\color[rgb]{0.0,0.4163,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.3906,0.0}{{passages}}}
{\color[rgb]{0.0,0.272,0.0}{{which}}}
{\color[rgb]{0.0,0.1971,0.0}{{are}}}
{\color[rgb]{0.0,0.0858,0.0}{{easily}}}
{\color[rgb]{0.0,0.0929,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.0988,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.6654,0.0}{{,}}}
{\color[rgb]{0.0,0.6688,0.0}{{or}}}
{\color[rgb]{0.0,0.6875,0.0}{{heart}}}
{\color[rgb]{0.0,0.7525,0.0}{{disease}}}
{\color[rgb]{0.0,0.1071,0.0}{{.}}}
{\color[rgb]{0.0,0.118,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.052,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0459,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0463,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0564,0.0}{{MS}}}
{\color[rgb]{0.0,0.0447,0.0}{{...}}}
{\color[rgb]{0.0,0.0382,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.1948,0.0}{{bases}}}
{\color[rgb]{0.0,0.1819,0.0}{{his}}}
{\color[rgb]{0.0,0.231,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.1785,0.0}{{on}}}
{\color[rgb]{0.0,0.2333,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0,0.2358,0.0}{{blind}}}
{\color[rgb]{0.0,0.223,0.0}{{to}}}
{\color[rgb]{0.0,0.201,0.0}{{my}}}
{\color[rgb]{0.0,0.2116,0.0}{{own}}}
{\color[rgb]{0.0,0.2555,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.06,0.0}{{n't}}}
{\color[rgb]{0.0,0.1509,0.0}{{possibly}}}
{\color[rgb]{0.0,0.2052,0.0}{{screwed}}}
{\color[rgb]{0.0,0.2643,0.0}{{up}}}
{\color[rgb]{0.0,0.3093,0.0}{{your}}}
{\color[rgb]{0.0,0.3714,0.0}{{engine}}}
{\color[rgb]{0.0,0.1839,0.0}{{.}}}
{\color[rgb]{0.0,0.2621,0.0}{{If}}}
{\color[rgb]{0.0,0.1768,0.0}{{these}}}
{\color[rgb]{0.0,0.2041,0.0}{{people}}}
{\color[rgb]{0.0,0.1705,0.0}{{are}}}
{\color[rgb]{0.0,0.316,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0009,0.0}{{,}}}
{\color[rgb]{0.0,0.0008,0.0}{{does}}}
{\color[rgb]{0.0,0.0009,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.1236,0.0}{{less}}}
{\color[rgb]{0.0,0.1147,0.0}{{valuable}}}
{\color[rgb]{0.0,0.1048,0.0}{{?}}}

==> examples/CNN_newsgroup_grad_raw_l2_integrated_3737.tex <==
{\color[rgb]{0.0,0.3326,0.0}{{settings}}}
{\color[rgb]{0.0,0.2479,0.0}{{.}}}
{\color[rgb]{0.0,0.3347,0.0}{{Children}}}
{\color[rgb]{0.0,0.2938,0.0}{{have}}}
{\color[rgb]{0.0,0.3639,0.0}{{tiny}}}
{\color[rgb]{0.0,0.3891,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.3847,0.0}{{passages}}}
{\color[rgb]{0.0,0.2645,0.0}{{which}}}
{\color[rgb]{0.0,0.1722,0.0}{{are}}}
{\color[rgb]{0.0,0.0165,0.0}{{easily}}}
{\color[rgb]{0.0,0.0178,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.0888,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.6562,0.0}{{,}}}
{\color[rgb]{0.0,0.6518,0.0}{{or}}}
{\color[rgb]{0.0,0.6617,0.0}{{heart}}}
{\color[rgb]{0.0,0.7251,0.0}{{disease}}}
{\color[rgb]{0.0,0.0732,0.0}{{.}}}
{\color[rgb]{0.0,0.0807,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0507,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0448,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0451,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.055,0.0}{{MS}}}
{\color[rgb]{0.0,0.0436,0.0}{{...}}}
{\color[rgb]{0.0,0.0376,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.1854,0.0}{{bases}}}
{\color[rgb]{0.0,0.173,0.0}{{his}}}
{\color[rgb]{0.0,0.2193,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.17,0.0}{{on}}}
{\color[rgb]{0.0,0.2223,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0,0.2209,0.0}{{blind}}}
{\color[rgb]{0.0,0.2099,0.0}{{to}}}
{\color[rgb]{0.0,0.1797,0.0}{{my}}}
{\color[rgb]{0.0,0.2023,0.0}{{own}}}
{\color[rgb]{0.0,0.2374,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0304,0.0}{{n't}}}
{\color[rgb]{0.0,0.0907,0.0}{{possibly}}}
{\color[rgb]{0.0,0.1167,0.0}{{screwed}}}
{\color[rgb]{0.0,0.1752,0.0}{{up}}}
{\color[rgb]{0.0,0.2029,0.0}{{your}}}
{\color[rgb]{0.0,0.2468,0.0}{{engine}}}
{\color[rgb]{0.0,0.1278,0.0}{{.}}}
{\color[rgb]{0.0,0.2414,0.0}{{If}}}
{\color[rgb]{0.0,0.1749,0.0}{{these}}}
{\color[rgb]{0.0,0.1965,0.0}{{people}}}
{\color[rgb]{0.0,0.167,0.0}{{are}}}
{\color[rgb]{0.0,0.3088,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0006,0.0}{{,}}}
{\color[rgb]{0.0,0.0006,0.0}{{does}}}
{\color[rgb]{0.0,0.0007,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0794,0.0}{{less}}}
{\color[rgb]{0.0,0.0688,0.0}{{valuable}}}
{\color[rgb]{0.0,0.067,0.0}{{?}}}

==> examples/CNN_newsgroup_lime_class_3737.tex <==
{\color[rgb]{0.0,0.0002,0.0}{{settings}}}
{\color[rgb]{0.0002,0.0,0.0}{{.}}}
{\color[rgb]{0.0002,0.0,0.0}{{Children}}}
{\color[rgb]{0.0,0.0002,0.0}{{have}}}
{\color[rgb]{0.0,0.0003,0.0}{{tiny}}}
{\color[rgb]{0.0,0.5824,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.0002,0.0}{{passages}}}
{\color[rgb]{0.0,0.0001,0.0}{{which}}}
{\color[rgb]{0.0002,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0001,0.0}{{easily}}}
{\color[rgb]{0.383,0.0,0.0}{{blocked}}}
{\color[rgb]{0.4129,0.0,0.0}{{by}}}
{\color[rgb]{0.4039,0.0,0.0}{{the}}}
{\color[rgb]{0.3333,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0006,0.0,0.0}{{induced}}}
{\color[rgb]{0.2812,0.0,0.0}{{by}}}
{\color[rgb]{0.5497,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.3732,0.0,0.0}{{;}}}
{\color[rgb]{0.1866,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.4848,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.3605,0.0,0.0}{{can}}}
{\color[rgb]{0.2056,0.0,0.0}{{easily}}}
{\color[rgb]{0.2286,0.0,0.0}{{cause}}}
{\color[rgb]{0.6359,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.3584,0.0,0.0}{{in}}}
{\color[rgb]{0.3448,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0009,0.0,0.0}{{subject}}}
{\color[rgb]{0.0002,0.0,0.0}{{to}}}
{\color[rgb]{0.0003,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0002,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.6918,0.0}{{asthma}}}
{\color[rgb]{0.0,0.0005,0.0}{{,}}}
{\color[rgb]{0.0,0.0002,0.0}{{or}}}
{\color[rgb]{0.0,0.0004,0.0}{{heart}}}
{\color[rgb]{0.0,0.9091,0.0}{{disease}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0002,0.0}{{9}}}
{\color[rgb]{0.0004,0.0,0.0}{{.}}}
{\color[rgb]{0.0012,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.5012,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.2823,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.5232,0.0,0.0}{{MS}}}
{\color[rgb]{0.1655,0.0,0.0}{{...}}}
{\color[rgb]{0.37,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.4898,0.0,0.0}{{bases}}}
{\color[rgb]{0.3027,0.0,0.0}{{his}}}
{\color[rgb]{0.2251,0.0,0.0}{{interpretation}}}
{\color[rgb]{0.2767,0.0,0.0}{{on}}}
{\color[rgb]{0.5849,0.0,0.0}{{linguistics}}}
{\color[rgb]{0.2444,0.0,0.0}{{and}}}
{\color[rgb]{0.2895,0.0,0.0}{{the}}}
{\color[rgb]{0.212,0.0,0.0}{{historical}}}
{\color[rgb]{0.53,0.0,0.0}{{setting}}}
{\color[rgb]{0.186,0.0,0.0}{{.}}}
{\color[rgb]{0.5099,0.0,0.0}{{I}}}
{\color[rgb]{0.261,0.0,0.0}{{am}}}
{\color[rgb]{0.3882,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.2866,0.0,0.0}{{willing}}}
{\color[rgb]{0.3053,0.0,0.0}{{to}}}
{\color[rgb]{0.3654,0.0,0.0}{{grant}}}
{\color[rgb]{0.3063,0.0,0.0}{{that}}}
{\color[rgb]{0.3554,0.0,0.0}{{I}}}
{\color[rgb]{0.2994,0.0,0.0}{{could}}}
{\color[rgb]{0.3526,0.0,0.0}{{be}}}
{\color[rgb]{0.3396,0.0,0.0}{{blind}}}
{\color[rgb]{0.2812,0.0,0.0}{{to}}}
{\color[rgb]{0.2647,0.0,0.0}{{my}}}
{\color[rgb]{0.5471,0.0,0.0}{{own}}}
{\color[rgb]{0.1218,0.0,0.0}{{sin}}}
{\color[rgb]{0.4769,0.0,0.0}{{.}}}
{\color[rgb]{0.4757,0.0,0.0}{{Any}}}
{\color[rgb]{0.22,0.0,0.0}{{other}}}
{\color[rgb]{0.3476,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.2715,0.0,0.0}{{?}}}
{\color[rgb]{0.4072,0.0,0.0}{{Heck}}}
{\color[rgb]{0.281,0.0,0.0}{{,}}}
{\color[rgb]{0.3532,0.0,0.0}{{those}}}
{\color[rgb]{0.3106,0.0,0.0}{{miles}}}
{\color[rgb]{0.2171,0.0,0.0}{{go}}}
{\color[rgb]{0.5925,0.0,0.0}{{by}}}
{\color[rgb]{0.2021,0.0,0.0}{{fast}}}
{\color[rgb]{0.3772,0.0,0.0}{{,}}}
{\color[rgb]{0.2241,0.0,0.0}{{and}}}
{\color[rgb]{0.5394,0.0,0.0}{{it}}}
{\color[rgb]{0.2454,0.0,0.0}{{'s}}}
{\color[rgb]{0.322,0.0,0.0}{{worth}}}
{\color[rgb]{0.3428,0.0,0.0}{{it}}}
{\color[rgb]{0.3042,0.0,0.0}{{to}}}
{\color[rgb]{0.2954,0.0,0.0}{{know}}}
{\color[rgb]{0.2385,0.0,0.0}{{you}}}
{\color[rgb]{0.4846,0.0,0.0}{{have}}}
{\color[rgb]{0.4011,0.0,0.0}{{n't}}}
{\color[rgb]{0.409,0.0,0.0}{{possibly}}}
{\color[rgb]{0.2155,0.0,0.0}{{screwed}}}
{\color[rgb]{0.2148,0.0,0.0}{{up}}}
{\color[rgb]{0.4425,0.0,0.0}{{your}}}
{\color[rgb]{0.4339,0.0,0.0}{{engine}}}
{\color[rgb]{0.3321,0.0,0.0}{{.}}}
{\color[rgb]{0.251,0.0,0.0}{{If}}}
{\color[rgb]{0.2897,0.0,0.0}{{these}}}
{\color[rgb]{0.4525,0.0,0.0}{{people}}}
{\color[rgb]{0.2776,0.0,0.0}{{are}}}
{\color[rgb]{0.2338,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.4574,0.0,0.0}{{,}}}
{\color[rgb]{0.2608,0.0,0.0}{{does}}}
{\color[rgb]{0.4237,0.0,0.0}{{it}}}
{\color[rgb]{0.4222,0.0,0.0}{{mean}}}
{\color[rgb]{0.3472,0.0,0.0}{{that}}}
{\color[rgb]{0.285,0.0,0.0}{{they}}}
{\color[rgb]{0.2455,0.0,0.0}{{are}}}
{\color[rgb]{0.0863,0.0,0.0}{{less}}}
{\color[rgb]{0.0004,0.0,0.0}{{valuable}}}
{\color[rgb]{0.0001,0.0,0.0}{{?}}}

==> examples/CNN_newsgroup_lime_prob_3737.tex <==
{\color[rgb]{0.0,0.0,0.0}{{settings}}}
{\color[rgb]{0.0001,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Children}}}
{\color[rgb]{0.0,0.0003,0.0}{{have}}}
{\color[rgb]{0.0,0.0233,0.0}{{tiny}}}
{\color[rgb]{0.0,0.9091,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.084,0.0}{{passages}}}
{\color[rgb]{0.0001,0.0,0.0}{{which}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0003,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0002,0.0}{{by}}}
{\color[rgb]{0.0,0.0002,0.0}{{the}}}
{\color[rgb]{0.0001,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0001,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0002,0.0}{{by}}}
{\color[rgb]{0.0,0.0001,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0002,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0001,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0001,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0001,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0003,0.0}{{in}}}
{\color[rgb]{0.0,0.0001,0.0}{{anyone}}}
{\color[rgb]{0.0002,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0002,0.0}{{to}}}
{\color[rgb]{0.0002,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.0003,0.0}{{,}}}
{\color[rgb]{0.0,0.9051,0.0}{{asthma}}}
{\color[rgb]{0.0,0.0589,0.0}{{,}}}
{\color[rgb]{0.0,0.0001,0.0}{{or}}}
{\color[rgb]{0.0,0.0943,0.0}{{heart}}}
{\color[rgb]{0.0,0.3235,0.0}{{disease}}}
{\color[rgb]{0.0,0.0004,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0002,0.0}{{.}}}
{\color[rgb]{0.0,0.0003,0.0}{\underline{J}}}
{\color[rgb]{0.0001,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.0001,0.0,0.0}{{MS}}}
{\color[rgb]{0.0002,0.0,0.0}{{...}}}
{\color[rgb]{0.0001,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0001,0.0,0.0}{{bases}}}
{\color[rgb]{0.0,0.0002,0.0}{{his}}}
{\color[rgb]{0.0,0.0002,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.0004,0.0}{{on}}}
{\color[rgb]{0.0,0.0005,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0001,0.0}{{and}}}
{\color[rgb]{0.0,0.0002,0.0}{{the}}}
{\color[rgb]{0.0,0.0001,0.0}{{historical}}}
{\color[rgb]{0.0,0.0003,0.0}{{setting}}}
{\color[rgb]{0.0002,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0003,0.0}{{I}}}
{\color[rgb]{0.0,0.0001,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0001,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0001,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0004,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0001,0.0}{{could}}}
{\color[rgb]{0.0001,0.0,0.0}{{be}}}
{\color[rgb]{0.0,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0003,0.0}{{to}}}
{\color[rgb]{0.0,0.0003,0.0}{{my}}}
{\color[rgb]{0.0,0.0,0.0}{{own}}}
{\color[rgb]{0.0,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0002,0.0}{{.}}}
{\color[rgb]{0.0,0.0002,0.0}{{Any}}}
{\color[rgb]{0.0002,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0002,0.0}{{suggestions}}}
{\color[rgb]{0.0001,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0001,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0002,0.0}{{go}}}
{\color[rgb]{0.0001,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0004,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0001,0.0}{{and}}}
{\color[rgb]{0.0,0.0001,0.0}{{it}}}
{\color[rgb]{0.0,0.0002,0.0}{{'s}}}
{\color[rgb]{0.0,0.0003,0.0}{{worth}}}
{\color[rgb]{0.0002,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0003,0.0,0.0}{{know}}}
{\color[rgb]{0.0002,0.0,0.0}{{you}}}
{\color[rgb]{0.0001,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0002,0.0}{{n't}}}
{\color[rgb]{0.0002,0.0,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0003,0.0}{{screwed}}}
{\color[rgb]{0.0001,0.0,0.0}{{up}}}
{\color[rgb]{0.0001,0.0,0.0}{{your}}}
{\color[rgb]{0.0,0.0002,0.0}{{engine}}}
{\color[rgb]{0.0,0.0004,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{If}}}
{\color[rgb]{0.0001,0.0,0.0}{{these}}}
{\color[rgb]{0.0001,0.0,0.0}{{people}}}
{\color[rgb]{0.0002,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0001,0.0}{{Muslims}}}
{\color[rgb]{0.0001,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0003,0.0}{{does}}}
{\color[rgb]{0.0001,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0001,0.0}{{mean}}}
{\color[rgb]{0.0,0.0001,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0002,0.0,0.0}{{are}}}
{\color[rgb]{0.0002,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0001,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0001,0.0}{{?}}}

==> examples/CNN_newsgroup_lime_raw_3737.tex <==
{\color[rgb]{0.1775,0.0,0.0}{{settings}}}
{\color[rgb]{0.0375,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Children}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0953,0.0}{{tiny}}}
{\color[rgb]{0.0,0.6481,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.1813,0.0}{{passages}}}
{\color[rgb]{0.0,0.0,0.0}{{which}}}
{\color[rgb]{0.0812,0.0,0.0}{{are}}}
{\color[rgb]{0.0142,0.0,0.0}{{easily}}}
{\color[rgb]{0.038,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0001,0.0,0.0}{{by}}}
{\color[rgb]{0.0007,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0065,0.0,0.0}{{;}}}
{\color[rgb]{0.0018,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0057,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0036,0.0,0.0}{{can}}}
{\color[rgb]{0.0134,0.0,0.0}{{easily}}}
{\color[rgb]{0.0002,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0129,0.0,0.0}{{subject}}}
{\color[rgb]{0.0612,0.0,0.0}{{to}}}
{\color[rgb]{0.0491,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0272,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.0359,0.0}{{,}}}
{\color[rgb]{0.0,0.0367,0.0}{{or}}}
{\color[rgb]{0.0,0.0944,0.0}{{heart}}}
{\color[rgb]{0.0,0.3331,0.0}{{disease}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0418,0.0,0.0}{{9}}}
{\color[rgb]{0.028,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0121,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.0337,0.0,0.0}{{MS}}}
{\color[rgb]{0.0173,0.0,0.0}{{...}}}
{\color[rgb]{0.0021,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0,0.0}{{bases}}}
{\color[rgb]{0.0,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.0442,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.0059,0.0}{{on}}}
{\color[rgb]{0.0,0.0132,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0392,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0065,0.0,0.0}{{I}}}
{\color[rgb]{0.0007,0.0,0.0}{{am}}}
{\color[rgb]{0.0101,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0059,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0152,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0225,0.0,0.0}{{could}}}
{\color[rgb]{0.0072,0.0,0.0}{{be}}}
{\color[rgb]{0.0079,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0324,0.0,0.0}{{my}}}
{\color[rgb]{0.0429,0.0,0.0}{{own}}}
{\color[rgb]{0.1734,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0001,0.0,0.0}{{?}}}
{\color[rgb]{0.0173,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0007,0.0,0.0}{{,}}}
{\color[rgb]{0.0034,0.0,0.0}{{those}}}
{\color[rgb]{0.0043,0.0,0.0}{{miles}}}
{\color[rgb]{0.001,0.0,0.0}{{go}}}
{\color[rgb]{0.0073,0.0,0.0}{{by}}}
{\color[rgb]{0.0034,0.0,0.0}{{fast}}}
{\color[rgb]{0.0045,0.0,0.0}{{,}}}
{\color[rgb]{0.0027,0.0,0.0}{{and}}}
{\color[rgb]{0.005,0.0,0.0}{{it}}}
{\color[rgb]{0.0037,0.0,0.0}{{'s}}}
{\color[rgb]{0.0064,0.0,0.0}{{worth}}}
{\color[rgb]{0.002,0.0,0.0}{{it}}}
{\color[rgb]{0.003,0.0,0.0}{{to}}}
{\color[rgb]{0.0095,0.0,0.0}{{know}}}
{\color[rgb]{0.0033,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0,0.0}{{n't}}}
{\color[rgb]{0.0,0.0,0.0}{{possibly}}}
{\color[rgb]{0.0536,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0,0.0}{{up}}}
{\color[rgb]{0.0249,0.0,0.0}{{your}}}
{\color[rgb]{0.1466,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{If}}}
{\color[rgb]{0.0,0.0,0.0}{{these}}}
{\color[rgb]{0.0802,0.0,0.0}{{people}}}
{\color[rgb]{0.0436,0.0,0.0}{{are}}}
{\color[rgb]{0.1695,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0162,0.0,0.0}{{they}}}
{\color[rgb]{0.0001,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}

==> examples/CNN_newsgroup_lrp_3737.tex <==
{\color[rgb]{0.2134,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.0598,0.0}{{.}}}
{\color[rgb]{0.0,0.0466,0.0}{{Children}}}
{\color[rgb]{0.0538,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0261,0.0}{{tiny}}}
{\color[rgb]{0.0,0.1612,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.09,0.0}{{passages}}}
{\color[rgb]{0.0105,0.0,0.0}{{which}}}
{\color[rgb]{0.0212,0.0,0.0}{{are}}}
{\color[rgb]{0.0002,0.0,0.0}{{easily}}}
{\color[rgb]{0.0054,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0186,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.2277,0.0,0.0}{{,}}}
{\color[rgb]{0.2246,0.0,0.0}{{or}}}
{\color[rgb]{0.0301,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.237,0.0}{{disease}}}
{\color[rgb]{0.0122,0.0,0.0}{{.}}}
{\color[rgb]{0.0132,0.0,0.0}{{9}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0035,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.006,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0023,0.0}{{Thanks}}}
{\color[rgb]{0.0185,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0034,0.0}{{...}}}
{\color[rgb]{0.0057,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0115,0.0}{{bases}}}
{\color[rgb]{0.0145,0.0,0.0}{{his}}}
{\color[rgb]{0.0,0.0287,0.0}{{interpretation}}}
{\color[rgb]{0.0195,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.0836,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0109,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.0321,0.0}{{to}}}
{\color[rgb]{0.0,0.0363,0.0}{{my}}}
{\color[rgb]{0.0,0.014,0.0}{{own}}}
{\color[rgb]{0.1812,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Any}}}
{\color[rgb]{0.0,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.006,0.0}{{n't}}}
{\color[rgb]{0.0,0.0286,0.0}{{possibly}}}
{\color[rgb]{0.0371,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0282,0.0}{{up}}}
{\color[rgb]{0.0,0.0148,0.0}{{your}}}
{\color[rgb]{0.1576,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.0192,0.0}{{.}}}
{\color[rgb]{0.0,0.0564,0.0}{{If}}}
{\color[rgb]{0.0,0.0312,0.0}{{these}}}
{\color[rgb]{0.0,0.0398,0.0}{{people}}}
{\color[rgb]{0.0,0.0149,0.0}{{are}}}
{\color[rgb]{0.2662,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0002,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0001,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0,0.0}{{are}}}
{\color[rgb]{0.0144,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.0241,0.0}{{valuable}}}
{\color[rgb]{0.0016,0.0,0.0}{{?}}}

==> examples/CNN_newsgroup_omission-3_3737.tex <==
{\color[rgb]{0.0656,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.1248,0.0}{{.}}}
{\color[rgb]{0.0,0.1313,0.0}{{Children}}}
{\color[rgb]{0.0,0.387,0.0}{{have}}}
{\color[rgb]{0.0,0.3593,0.0}{{tiny}}}
{\color[rgb]{0.0,0.5078,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.2153,0.0}{{passages}}}
{\color[rgb]{0.0668,0.0,0.0}{{which}}}
{\color[rgb]{0.2658,0.0,0.0}{{are}}}
{\color[rgb]{0.1643,0.0,0.0}{{easily}}}
{\color[rgb]{0.0614,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0012,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0038,0.0}{{the}}}
{\color[rgb]{0.0,0.0203,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0041,0.0}{{induced}}}
{\color[rgb]{0.0216,0.0,0.0}{{by}}}
{\color[rgb]{0.0216,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0217,0.0,0.0}{{;}}}
{\color[rgb]{0.0012,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0012,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0012,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0183,0.0}{{cause}}}
{\color[rgb]{0.0,0.0258,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0299,0.0}{{in}}}
{\color[rgb]{0.011,0.0,0.0}{{anyone}}}
{\color[rgb]{0.1467,0.0,0.0}{{subject}}}
{\color[rgb]{0.4953,0.0,0.0}{{to}}}
{\color[rgb]{0.1334,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.3195,0.0}{{,}}}
{\color[rgb]{0.0,0.8348,0.0}{{asthma}}}
{\color[rgb]{0.3802,0.0,0.0}{{,}}}
{\color[rgb]{0.828,0.0,0.0}{{or}}}
{\color[rgb]{0.9091,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.131,0.0}{{disease}}}
{\color[rgb]{0.0,0.0888,0.0}{{.}}}
{\color[rgb]{0.0469,0.0,0.0}{{9}}}
{\color[rgb]{0.1923,0.0,0.0}{{.}}}
{\color[rgb]{0.0022,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0615,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0588,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0287,0.0}{{MS}}}
{\color[rgb]{0.0,0.0432,0.0}{{...}}}
{\color[rgb]{0.0,0.0045,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0091,0.0}{{bases}}}
{\color[rgb]{0.0,0.0039,0.0}{{his}}}
{\color[rgb]{0.0,0.0816,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.1234,0.0}{{on}}}
{\color[rgb]{0.0,0.1541,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.1634,0.0}{{and}}}
{\color[rgb]{0.0,0.1222,0.0}{{the}}}
{\color[rgb]{0.0,0.0644,0.0}{{historical}}}
{\color[rgb]{0.0,0.0088,0.0}{{setting}}}
{\color[rgb]{0.0,0.0343,0.0}{{.}}}
{\color[rgb]{0.0,0.0443,0.0}{{I}}}
{\color[rgb]{0.0,0.0391,0.0}{{am}}}
{\color[rgb]{0.0,0.0409,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0309,0.0}{{willing}}}
{\color[rgb]{0.0,0.039,0.0}{{to}}}
{\color[rgb]{0.0,0.0167,0.0}{{grant}}}
{\color[rgb]{0.0,0.0504,0.0}{{that}}}
{\color[rgb]{0.0,0.0509,0.0}{{I}}}
{\color[rgb]{0.0,0.0371,0.0}{{could}}}
{\color[rgb]{0.0,0.0469,0.0}{{be}}}
{\color[rgb]{0.0,0.2114,0.0}{{blind}}}
{\color[rgb]{0.0,0.5514,0.0}{{to}}}
{\color[rgb]{0.0,0.4331,0.0}{{my}}}
{\color[rgb]{0.0,0.1809,0.0}{{own}}}
{\color[rgb]{0.2327,0.0,0.0}{{sin}}}
{\color[rgb]{0.0076,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.1658,0.0}{{Any}}}
{\color[rgb]{0.0,0.2628,0.0}{{other}}}
{\color[rgb]{0.0,0.1124,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0144,0.0}{{?}}}
{\color[rgb]{0.0001,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0236,0.0}{{,}}}
{\color[rgb]{0.0,0.0236,0.0}{{those}}}
{\color[rgb]{0.0,0.0236,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0074,0.0}{{by}}}
{\color[rgb]{0.0,0.0074,0.0}{{fast}}}
{\color[rgb]{0.0,0.0115,0.0}{{,}}}
{\color[rgb]{0.0,0.0041,0.0}{{and}}}
{\color[rgb]{0.0,0.0041,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0007,0.0}{{worth}}}
{\color[rgb]{0.0,0.0085,0.0}{{it}}}
{\color[rgb]{0.0,0.0085,0.0}{{to}}}
{\color[rgb]{0.0,0.02,0.0}{{know}}}
{\color[rgb]{0.0,0.0607,0.0}{{you}}}
{\color[rgb]{0.0,0.2242,0.0}{{have}}}
{\color[rgb]{0.0,0.2141,0.0}{{n't}}}
{\color[rgb]{0.0,0.2294,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0938,0.0}{{screwed}}}
{\color[rgb]{0.0,0.0787,0.0}{{up}}}
{\color[rgb]{0.0,0.0094,0.0}{{your}}}
{\color[rgb]{0.0,0.0155,0.0}{{engine}}}
{\color[rgb]{0.0,0.1524,0.0}{{.}}}
{\color[rgb]{0.0,0.3504,0.0}{{If}}}
{\color[rgb]{0.0,0.5033,0.0}{{these}}}
{\color[rgb]{0.0,0.2914,0.0}{{people}}}
{\color[rgb]{0.0,0.0133,0.0}{{are}}}
{\color[rgb]{0.2626,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.1411,0.0,0.0}{{,}}}
{\color[rgb]{0.0485,0.0,0.0}{{does}}}
{\color[rgb]{0.0,0.0499,0.0}{{it}}}
{\color[rgb]{0.0,0.0061,0.0}{{mean}}}
{\color[rgb]{0.0154,0.0,0.0}{{that}}}
{\color[rgb]{0.0399,0.0,0.0}{{they}}}
{\color[rgb]{0.0076,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0125,0.0}{{less}}}
{\color[rgb]{0.0,0.0276,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0056,0.0}{{?}}}

==> examples/CNN_newsgroup_omission-5_3737.tex <==
{\color[rgb]{0.1243,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.1845,0.0}{{.}}}
{\color[rgb]{0.0,0.353,0.0}{{Children}}}
{\color[rgb]{0.0,0.4866,0.0}{{have}}}
{\color[rgb]{0.0,0.613,0.0}{{tiny}}}
{\color[rgb]{0.0,0.8442,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.4402,0.0}{{passages}}}
{\color[rgb]{0.0,0.1818,0.0}{{which}}}
{\color[rgb]{0.0,0.0089,0.0}{{are}}}
{\color[rgb]{0.1425,0.0,0.0}{{easily}}}
{\color[rgb]{0.2377,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0945,0.0,0.0}{{by}}}
{\color[rgb]{0.0019,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0375,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0624,0.0}{{induced}}}
{\color[rgb]{0.0,0.0242,0.0}{{by}}}
{\color[rgb]{0.0216,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0243,0.0,0.0}{{;}}}
{\color[rgb]{0.0243,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0243,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0024,0.0}{{can}}}
{\color[rgb]{0.0,0.0002,0.0}{{easily}}}
{\color[rgb]{0.0,0.0087,0.0}{{cause}}}
{\color[rgb]{0.0,0.0001,0.0}\textit{{fatalities}}}
{\color[rgb]{0.081,0.0,0.0}{{in}}}
{\color[rgb]{0.329,0.0,0.0}{{anyone}}}
{\color[rgb]{0.1117,0.0,0.0}{{subject}}}
{\color[rgb]{0.0,0.0925,0.0}{{to}}}
{\color[rgb]{0.0,0.2145,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.4067,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.3492,0.0}{{,}}}
{\color[rgb]{0.0,0.0561,0.0}{{or}}}
{\color[rgb]{0.0011,0.0,0.0}{{heart}}}
{\color[rgb]{0.0071,0.0,0.0}{{disease}}}
{\color[rgb]{0.3337,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0208,0.0}{{9}}}
{\color[rgb]{0.0,0.1009,0.0}{{.}}}
{\color[rgb]{0.0,0.0544,0.0}{\underline{J}}}
{\color[rgb]{0.0175,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0664,0.0}{{Thanks}}}
{\color[rgb]{0.0,0.0449,0.0}{{MS}}}
{\color[rgb]{0.0,0.0996,0.0}{{...}}}
{\color[rgb]{0.0,0.0928,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0908,0.0}{{bases}}}
{\color[rgb]{0.0,0.1695,0.0}{{his}}}
{\color[rgb]{0.0,0.2244,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.2459,0.0}{{on}}}
{\color[rgb]{0.0,0.2744,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.2785,0.0}{{and}}}
{\color[rgb]{0.0,0.189,0.0}{{the}}}
{\color[rgb]{0.0,0.1438,0.0}{{historical}}}
{\color[rgb]{0.0,0.076,0.0}{{setting}}}
{\color[rgb]{0.0,0.1197,0.0}{{.}}}
{\color[rgb]{0.0,0.1369,0.0}{{I}}}
{\color[rgb]{0.0,0.1359,0.0}{{am}}}
{\color[rgb]{0.0,0.1412,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.1371,0.0}{{willing}}}
{\color[rgb]{0.0,0.0812,0.0}{{to}}}
{\color[rgb]{0.0,0.0619,0.0}{{grant}}}
{\color[rgb]{0.0,0.0953,0.0}{{that}}}
{\color[rgb]{0.0,0.1245,0.0}{{I}}}
{\color[rgb]{0.0,0.2339,0.0}{{could}}}
{\color[rgb]{0.0,0.3918,0.0}{{be}}}
{\color[rgb]{0.0,0.307,0.0}{{blind}}}
{\color[rgb]{0.0,0.2518,0.0}{{to}}}
{\color[rgb]{0.0,0.168,0.0}{{my}}}
{\color[rgb]{0.0,0.0093,0.0}{{own}}}
{\color[rgb]{0.2038,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.008,0.0}{{.}}}
{\color[rgb]{0.0,0.0757,0.0}{{Any}}}
{\color[rgb]{0.0,0.131,0.0}{{other}}}
{\color[rgb]{0.0,0.1784,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.2171,0.0}{{?}}}
{\color[rgb]{0.0,0.0603,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0511,0.0}{{,}}}
{\color[rgb]{0.0,0.0447,0.0}{{those}}}
{\color[rgb]{0.0,0.0428,0.0}{{miles}}}
{\color[rgb]{0.0,0.0458,0.0}{{go}}}
{\color[rgb]{0.0,0.0591,0.0}{{by}}}
{\color[rgb]{0.0,0.0231,0.0}{{fast}}}
{\color[rgb]{0.0,0.0258,0.0}{{,}}}
{\color[rgb]{0.0,0.0258,0.0}{{and}}}
{\color[rgb]{0.0,0.0215,0.0}{{it}}}
{\color[rgb]{0.0,0.0049,0.0}{{'s}}}
{\color[rgb]{0.0,0.0075,0.0}{{worth}}}
{\color[rgb]{0.0,0.0178,0.0}{{it}}}
{\color[rgb]{0.0,0.0511,0.0}{{to}}}
{\color[rgb]{0.0,0.2446,0.0}{{know}}}
{\color[rgb]{0.0,0.2445,0.0}{{you}}}
{\color[rgb]{0.0,0.286,0.0}{{have}}}
{\color[rgb]{0.0,0.3206,0.0}{{n't}}}
{\color[rgb]{0.0,0.2496,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0171,0.0}{{screwed}}}
{\color[rgb]{0.0,0.113,0.0}{{up}}}
{\color[rgb]{0.0,0.1191,0.0}{{your}}}
{\color[rgb]{0.0,0.1863,0.0}{{engine}}}
{\color[rgb]{0.0,0.4507,0.0}{{.}}}
{\color[rgb]{0.0,0.438,0.0}{{If}}}
{\color[rgb]{0.0,0.2876,0.0}{{these}}}
{\color[rgb]{0.0,0.1808,0.0}{{people}}}
{\color[rgb]{0.0,0.0109,0.0}{{are}}}
{\color[rgb]{0.2736,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.1575,0.0,0.0}{{,}}}
{\color[rgb]{0.0985,0.0,0.0}{{does}}}
{\color[rgb]{0.0543,0.0,0.0}{{it}}}
{\color[rgb]{0.0166,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0587,0.0}{{that}}}
{\color[rgb]{0.0038,0.0,0.0}{{they}}}
{\color[rgb]{0.0083,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0035,0.0}{{less}}}
{\color[rgb]{0.0,0.0208,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0034,0.0}{{?}}}

==> examples/CNN_newsgroup_omission-7_3737.tex <==
{\color[rgb]{0.0,0.0306,0.0}{{settings}}}
{\color[rgb]{0.0,0.2436,0.0}{{.}}}
{\color[rgb]{0.0,0.3647,0.0}{{Children}}}
{\color[rgb]{0.0,0.4577,0.0}{{have}}}
{\color[rgb]{0.0,0.5283,0.0}{{tiny}}}
{\color[rgb]{0.0,0.5819,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.5171,0.0}{{passages}}}
{\color[rgb]{0.0,0.4278,0.0}{{which}}}
{\color[rgb]{0.0,0.1986,0.0}{{are}}}
{\color[rgb]{0.0,0.0773,0.0}{{easily}}}
{\color[rgb]{0.0104,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0502,0.0,0.0}{{by}}}
{\color[rgb]{0.1021,0.0,0.0}{{the}}}
{\color[rgb]{0.0373,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0227,0.0}{{induced}}}
{\color[rgb]{0.0,0.022,0.0}{{by}}}
{\color[rgb]{0.0,0.0222,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0169,0.0}{{;}}}
{\color[rgb]{0.0137,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0154,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0154,0.0,0.0}{{can}}}
{\color[rgb]{0.0263,0.0,0.0}{{easily}}}
{\color[rgb]{0.0569,0.0,0.0}{{cause}}}
{\color[rgb]{0.2103,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0663,0.0,0.0}{{in}}}
{\color[rgb]{0.0,0.0669,0.0}{{anyone}}}
{\color[rgb]{0.0,0.1374,0.0}{{subject}}}
{\color[rgb]{0.0,0.2089,0.0}{{to}}}
{\color[rgb]{0.0,0.3816,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.0,0.5924,0.0}{{,}}}
{\color[rgb]{0.0,0.9091,0.0}{{asthma}}}
{\color[rgb]{0.0,0.5464,0.0}{{,}}}
{\color[rgb]{0.0,0.3599,0.0}{{or}}}
{\color[rgb]{0.0,0.346,0.0}{{heart}}}
{\color[rgb]{0.0,0.3615,0.0}{{disease}}}
{\color[rgb]{0.0,0.1348,0.0}{{.}}}
{\color[rgb]{0.04,0.0,0.0}{{9}}}
{\color[rgb]{0.1939,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0317,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0908,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0327,0.0}{{Thanks}}}
{\color[rgb]{0.0602,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0578,0.0}{{...}}}
{\color[rgb]{0.0,0.0921,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.1064,0.0}{{bases}}}
{\color[rgb]{0.0,0.1844,0.0}{{his}}}
{\color[rgb]{0.0,0.202,0.0}{{interpretation}}}
{\color[rgb]{0.0,0.2236,0.0}{{on}}}
{\color[rgb]{0.0,0.2504,0.0}{{linguistics}}}
{\color[rgb]{0.0,0.2167,0.0}{{and}}}
{\color[rgb]{0.0,0.1955,0.0}{{the}}}
{\color[rgb]{0.0,0.1733,0.0}{{historical}}}
{\color[rgb]{0.0,0.1227,0.0}{{setting}}}
{\color[rgb]{0.0,0.1456,0.0}{{.}}}
{\color[rgb]{0.0,0.1285,0.0}{{I}}}
{\color[rgb]{0.0,0.1098,0.0}{{am}}}
{\color[rgb]{0.0,0.0956,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.1159,0.0}{{willing}}}
{\color[rgb]{0.0,0.1192,0.0}{{to}}}
{\color[rgb]{0.0,0.1044,0.0}{{grant}}}
{\color[rgb]{0.0,0.1513,0.0}{{that}}}
{\color[rgb]{0.0,0.2645,0.0}{{I}}}
{\color[rgb]{0.0,0.2277,0.0}{{could}}}
{\color[rgb]{0.0,0.1871,0.0}{{be}}}
{\color[rgb]{0.0,0.1324,0.0}{{blind}}}
{\color[rgb]{0.0,0.1154,0.0}{{to}}}
{\color[rgb]{0.0,0.0762,0.0}{{my}}}
{\color[rgb]{0.0279,0.0,0.0}{{own}}}
{\color[rgb]{0.1787,0.0,0.0}{{sin}}}
{\color[rgb]{0.0619,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0027,0.0}{{Any}}}
{\color[rgb]{0.0,0.0416,0.0}{{other}}}
{\color[rgb]{0.0,0.0559,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0756,0.0}{{?}}}
{\color[rgb]{0.0,0.0861,0.0}{{Heck}}}
{\color[rgb]{0.0,0.1444,0.0}{{,}}}
{\color[rgb]{0.0,0.063,0.0}{{those}}}
{\color[rgb]{0.0,0.0392,0.0}{{miles}}}
{\color[rgb]{0.0,0.0367,0.0}{{go}}}
{\color[rgb]{0.0,0.039,0.0}{{by}}}
{\color[rgb]{0.0,0.039,0.0}{{fast}}}
{\color[rgb]{0.0,0.0408,0.0}{{,}}}
{\color[rgb]{0.0,0.0173,0.0}{{and}}}
{\color[rgb]{0.0,0.0182,0.0}{{it}}}
{\color[rgb]{0.0,0.0165,0.0}{{'s}}}
{\color[rgb]{0.0,0.0345,0.0}{{worth}}}
{\color[rgb]{0.0,0.1583,0.0}{{it}}}
{\color[rgb]{0.0,0.1593,0.0}{{to}}}
{\color[rgb]{0.0,0.1863,0.0}{{know}}}
{\color[rgb]{0.0,0.2157,0.0}{{you}}}
{\color[rgb]{0.0,0.1897,0.0}{{have}}}
{\color[rgb]{0.0,0.1606,0.0}{{n't}}}
{\color[rgb]{0.0,0.1334,0.0}{{possibly}}}
{\color[rgb]{0.0,0.0162,0.0}{{screwed}}}
{\color[rgb]{0.0,0.1256,0.0}{{up}}}
{\color[rgb]{0.0,0.208,0.0}{{your}}}
{\color[rgb]{0.0,0.1398,0.0}{{engine}}}
{\color[rgb]{0.0,0.1475,0.0}{{.}}}
{\color[rgb]{0.0,0.14,0.0}{{If}}}
{\color[rgb]{0.0,0.1115,0.0}{{these}}}
{\color[rgb]{0.0,0.0639,0.0}{{people}}}
{\color[rgb]{0.0785,0.0,0.0}{{are}}}
{\color[rgb]{0.2268,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.1552,0.0,0.0}{{,}}}
{\color[rgb]{0.1434,0.0,0.0}{{does}}}
{\color[rgb]{0.1061,0.0,0.0}{{it}}}
{\color[rgb]{0.0737,0.0,0.0}{{mean}}}
{\color[rgb]{0.037,0.0,0.0}{{that}}}
{\color[rgb]{0.0051,0.0,0.0}{{they}}}
{\color[rgb]{0.0,0.0321,0.0}{{are}}}
{\color[rgb]{0.0007,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.004,0.0}{{valuable}}}
{\color[rgb]{0.002,0.0,0.0}{{?}}}

==> examples/CNN_newsgroup_omission_3737.tex <==
{\color[rgb]{0.218,0.0,0.0}{{settings}}}
{\color[rgb]{0.0,0.3212,0.0}{{.}}}
{\color[rgb]{0.0,0.1013,0.0}{{Children}}}
{\color[rgb]{0.1876,0.0,0.0}{{have}}}
{\color[rgb]{0.0,0.0816,0.0}{{tiny}}}
{\color[rgb]{0.0,0.3171,0.0}{{respiratory}}}
{\color[rgb]{0.0,0.1296,0.0}{{passages}}}
{\color[rgb]{0.1608,0.0,0.0}{{which}}}
{\color[rgb]{0.1229,0.0,0.0}{{are}}}
{\color[rgb]{0.0,0.0094,0.0}{{easily}}}
{\color[rgb]{0.0023,0.0,0.0}{{blocked}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0066,0.0,0.0}\textit{{secretions}}}
{\color[rgb]{0.0,0.0,0.0}{{induced}}}
{\color[rgb]{0.0189,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{;}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{moreover}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{teargas}}}
{\color[rgb]{0.0,0.0,0.0}{{can}}}
{\color[rgb]{0.0,0.0,0.0}{{easily}}}
{\color[rgb]{0.0,0.0,0.0}{{cause}}}
{\color[rgb]{0.0,0.0,0.0}\textit{{fatalities}}}
{\color[rgb]{0.0,0.0276,0.0}{{in}}}
{\color[rgb]{0.0,0.0,0.0}{{anyone}}}
{\color[rgb]{0.0,0.0,0.0}{{subject}}}
{\color[rgb]{0.0356,0.0,0.0}{{to}}}
{\color[rgb]{0.115,0.0,0.0}\textit{{laryngospasms}}}
{\color[rgb]{0.3973,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.9085,0.0}{{asthma}}}
{\color[rgb]{0.9091,0.0,0.0}{{,}}}
{\color[rgb]{0.7359,0.0,0.0}{{or}}}
{\color[rgb]{0.1373,0.0,0.0}{{heart}}}
{\color[rgb]{0.0,0.4017,0.0}{{disease}}}
{\color[rgb]{0.0719,0.0,0.0}{{.}}}
{\color[rgb]{0.0513,0.0,0.0}{{9}}}
{\color[rgb]{0.0246,0.0,0.0}{{.}}}
{\color[rgb]{0.0094,0.0,0.0}{\underline{J}}}
{\color[rgb]{0.0,0.0292,0.0}{\underline{.}}}
{\color[rgb]{0.0023,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.0135,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0043,0.0}{{...}}}
{\color[rgb]{0.0735,0.0,0.0}\textit{{Boswell}}}
{\color[rgb]{0.0,0.0232,0.0}{{bases}}}
{\color[rgb]{0.0,0.031,0.0}{{his}}}
{\color[rgb]{0.0,0.0603,0.0}{{interpretation}}}
{\color[rgb]{0.0371,0.0,0.0}{{on}}}
{\color[rgb]{0.0,0.1358,0.0}{{linguistics}}}
{\color[rgb]{0.0195,0.0,0.0}{{and}}}
{\color[rgb]{0.0007,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{historical}}}
{\color[rgb]{0.0,0.0,0.0}{{setting}}}
{\color[rgb]{0.0,0.0275,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{am}}}
{\color[rgb]{0.0,0.0239,0.0}{{perfectly}}}
{\color[rgb]{0.0,0.0,0.0}{{willing}}}
{\color[rgb]{0.0,0.0074,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{grant}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{I}}}
{\color[rgb]{0.0,0.0,0.0}{{could}}}
{\color[rgb]{0.0,0.0,0.0}{{be}}}
{\color[rgb]{0.0237,0.0,0.0}{{blind}}}
{\color[rgb]{0.0,0.1446,0.0}{{to}}}
{\color[rgb]{0.0,0.2119,0.0}{{my}}}
{\color[rgb]{0.0,0.1654,0.0}{{own}}}
{\color[rgb]{0.2208,0.0,0.0}{{sin}}}
{\color[rgb]{0.0,0.0829,0.0}{{.}}}
{\color[rgb]{0.0,0.0581,0.0}{{Any}}}
{\color[rgb]{0.0,0.015,0.0}{{other}}}
{\color[rgb]{0.0,0.0,0.0}{{suggestions}}}
{\color[rgb]{0.0,0.0,0.0}{{?}}}
{\color[rgb]{0.0,0.0,0.0}{{Heck}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{those}}}
{\color[rgb]{0.0,0.0,0.0}{{miles}}}
{\color[rgb]{0.0,0.0,0.0}{{go}}}
{\color[rgb]{0.0,0.0,0.0}{{by}}}
{\color[rgb]{0.0,0.0,0.0}{{fast}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{and}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{'s}}}
{\color[rgb]{0.0,0.0,0.0}{{worth}}}
{\color[rgb]{0.0,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.0,0.0}{{know}}}
{\color[rgb]{0.0,0.0,0.0}{{you}}}
{\color[rgb]{0.0,0.0172,0.0}{{have}}}
{\color[rgb]{0.0,0.0255,0.0}{{n't}}}
{\color[rgb]{0.0,0.1888,0.0}{{possibly}}}
{\color[rgb]{0.0491,0.0,0.0}{{screwed}}}
{\color[rgb]{0.0,0.2062,0.0}{{up}}}
{\color[rgb]{0.0,0.0915,0.0}{{your}}}
{\color[rgb]{0.1316,0.0,0.0}{{engine}}}
{\color[rgb]{0.0,0.072,0.0}{{.}}}
{\color[rgb]{0.0,0.1519,0.0}{{If}}}
{\color[rgb]{0.0,0.0954,0.0}{{these}}}
{\color[rgb]{0.0,0.1623,0.0}{{people}}}
{\color[rgb]{0.0,0.1051,0.0}{{are}}}
{\color[rgb]{0.2382,0.0,0.0}{{Muslims}}}
{\color[rgb]{0.0,0.0311,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{does}}}
{\color[rgb]{0.0018,0.0,0.0}{{it}}}
{\color[rgb]{0.0,0.0,0.0}{{mean}}}
{\color[rgb]{0.0,0.0,0.0}{{that}}}
{\color[rgb]{0.0057,0.0,0.0}{{they}}}
{\color[rgb]{0.0053,0.0,0.0}{{are}}}
{\color[rgb]{0.0274,0.0,0.0}{{less}}}
{\color[rgb]{0.0,0.038,0.0}{{valuable}}}
{\color[rgb]{0.0,0.0151,0.0}{{?}}}

==> examples/GRU_deeplift_2167.tex <==
{\color[rgb]{0.015,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.278,0.0}{{a}}}
{\color[rgb]{0.0,0.086,0.0}{{pagan}}}
{\color[rgb]{0.0,0.097,0.0}{{culture}}}
{\color[rgb]{0.0,0.107,0.0}{{,}}}
{\color[rgb]{0.0,0.252,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.244,0.0}{{about}}}
{\color[rgb]{0.0,0.077,0.0}{{the}}}
{\color[rgb]{0.0,0.246,0.0}{{return}}}
{\color[rgb]{0.003,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.047,0.0}{{the}}}
{\color[rgb]{0.0,0.097,0.0}{{christian}}}
{\color[rgb]{0.0,0.294,0.0}{{religion}}}
{\color[rgb]{0.0,0.119,0.0}{{to}}}
{\color[rgb]{0.0,0.014,0.0}{{the}}}
{\color[rgb]{0.117,0.0,0.0}{{islands}}}
{\color[rgb]{0.045,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.022,0.0}{{the}}}
{\color[rgb]{0.0,0.232,0.0}{{\textit{norse-era}}}}


==> examples/GRU_gamma_2167.tex <==
{\color[rgb]{0.103,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.15,0.0}{{a}}}
{\color[rgb]{0.0,0.066,0.0}{{pagan}}}
{\color[rgb]{0.0,0.061,0.0}{{culture}}}
{\color[rgb]{0.0,0.018,0.0}{{,}}}
{\color[rgb]{0.0,0.197,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.767,0.0}{{about}}}
{\color[rgb]{0.015,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.277,0.0}{{return}}}
{\color[rgb]{0.0,0.064,0.0}{{of}}}
{\color[rgb]{0.018,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.053,0.0}{{christian}}}
{\color[rgb]{0.0,0.331,0.0}{{religion}}}
{\color[rgb]{0.0,0.076,0.0}{{to}}}
{\color[rgb]{0.0,0.001,0.0}{{the}}}
{\color[rgb]{0.177,0.0,0.0}{{islands}}}
{\color[rgb]{0.304,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.016,0.0}{{the}}}
{\color[rgb]{0.0,0.617,0.0}{{\textit{norse-era}}}}


==> examples/GRU_l2_prob_2167.tex <==
{\color[rgb]{0.0,0.848,0.0}{{initially}}}
{\color[rgb]{0.0,0.194,0.0}{{a}}}
{\color[rgb]{0.0,0.143,0.0}{{pagan}}}
{\color[rgb]{0.0,0.187,0.0}{{culture}}}
{\color[rgb]{0.0,0.397,0.0}{{,}}}
{\color[rgb]{0.0,0.394,0.0}{{detailed}}}
{\color[rgb]{0.0,0.23,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.681,0.0}{{about}}}
{\color[rgb]{0.0,0.256,0.0}{{the}}}
{\color[rgb]{0.0,0.226,0.0}{{return}}}
{\color[rgb]{0.0,0.142,0.0}{{of}}}
{\color[rgb]{0.0,0.056,0.0}{{the}}}
{\color[rgb]{0.0,0.224,0.0}{{christian}}}
{\color[rgb]{0.0,0.372,0.0}{{religion}}}
{\color[rgb]{0.0,0.524,0.0}{{to}}}
{\color[rgb]{0.0,0.352,0.0}{{the}}}
{\color[rgb]{0.0,0.458,0.0}{{islands}}}
{\color[rgb]{0.0,0.494,0.0}{{during}}}
{\color[rgb]{0.0,0.299,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/GRU_l2_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.565,0.0}{{initially}}}
{\color[rgb]{0.0,0.313,0.0}{{a}}}
{\color[rgb]{0.0,0.222,0.0}{{pagan}}}
{\color[rgb]{0.0,0.125,0.0}{{culture}}}
{\color[rgb]{0.0,0.11,0.0}{{,}}}
{\color[rgb]{0.0,0.113,0.0}{{detailed}}}
{\color[rgb]{0.0,0.11,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.183,0.0}{{about}}}
{\color[rgb]{0.0,0.059,0.0}{{the}}}
{\color[rgb]{0.0,0.071,0.0}{{return}}}
{\color[rgb]{0.0,0.073,0.0}{{of}}}
{\color[rgb]{0.0,0.037,0.0}{{the}}}
{\color[rgb]{0.0,0.066,0.0}{{christian}}}
{\color[rgb]{0.0,0.127,0.0}{{religion}}}
{\color[rgb]{0.0,0.214,0.0}{{to}}}
{\color[rgb]{0.0,0.173,0.0}{{the}}}
{\color[rgb]{0.0,0.19,0.0}{{islands}}}
{\color[rgb]{0.0,0.231,0.0}{{during}}}
{\color[rgb]{0.0,0.305,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/GRU_l2_raw_2167.tex <==
{\color[rgb]{0.0,0.909,0.0}\textbf{{initially}}}
{\color[rgb]{0.0,0.235,0.0}{{a}}}
{\color[rgb]{0.0,0.177,0.0}{{pagan}}}
{\color[rgb]{0.0,0.211,0.0}{{culture}}}
{\color[rgb]{0.0,0.463,0.0}{{,}}}
{\color[rgb]{0.0,0.437,0.0}{{detailed}}}
{\color[rgb]{0.0,0.3,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.819,0.0}{{about}}}
{\color[rgb]{0.0,0.35,0.0}{{the}}}
{\color[rgb]{0.0,0.325,0.0}{{return}}}
{\color[rgb]{0.0,0.206,0.0}{{of}}}
{\color[rgb]{0.0,0.09,0.0}{{the}}}
{\color[rgb]{0.0,0.299,0.0}{{christian}}}
{\color[rgb]{0.0,0.523,0.0}{{religion}}}
{\color[rgb]{0.0,0.658,0.0}{{to}}}
{\color[rgb]{0.0,0.419,0.0}{{the}}}
{\color[rgb]{0.0,0.571,0.0}{{islands}}}
{\color[rgb]{0.0,0.553,0.0}{{during}}}
{\color[rgb]{0.0,0.317,0.0}{{the}}}
{\color[rgb]{0.0,0.89,0.0}{{\textit{norse-era}}}}


==> examples/GRU_l2_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.564,0.0}{{initially}}}
{\color[rgb]{0.0,0.288,0.0}{{a}}}
{\color[rgb]{0.0,0.224,0.0}{{pagan}}}
{\color[rgb]{0.0,0.173,0.0}{{culture}}}
{\color[rgb]{0.0,0.268,0.0}{{,}}}
{\color[rgb]{0.0,0.241,0.0}{{detailed}}}
{\color[rgb]{0.0,0.194,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.387,0.0}{{about}}}
{\color[rgb]{0.0,0.14,0.0}{{the}}}
{\color[rgb]{0.0,0.15,0.0}{{return}}}
{\color[rgb]{0.0,0.117,0.0}{{of}}}
{\color[rgb]{0.0,0.047,0.0}{{the}}}
{\color[rgb]{0.0,0.117,0.0}{{christian}}}
{\color[rgb]{0.0,0.22,0.0}{{religion}}}
{\color[rgb]{0.0,0.398,0.0}{{to}}}
{\color[rgb]{0.0,0.29,0.0}{{the}}}
{\color[rgb]{0.0,0.308,0.0}{{islands}}}
{\color[rgb]{0.0,0.315,0.0}{{during}}}
{\color[rgb]{0.0,0.305,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/GRU_lime_class_2167.tex <==
{\color[rgb]{0.0,0.399,0.0}{{initially}}}
{\color[rgb]{0.0,0.122,0.0}{{a}}}
{\color[rgb]{0.0,0.429,0.0}{{pagan}}}
{\color[rgb]{0.0,0.744,0.0}{{culture}}}
{\color[rgb]{0.0,0.867,0.0}{{,}}}
{\color[rgb]{0.0,0.303,0.0}{{detailed}}}
{\color[rgb]{0.0,0.478,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.352,0.0}{{the}}}
{\color[rgb]{0.0,0.443,0.0}{{return}}}
{\color[rgb]{0.0,0.429,0.0}{{of}}}
{\color[rgb]{0.0,0.348,0.0}{{the}}}
{\color[rgb]{0.0,0.517,0.0}{{christian}}}
{\color[rgb]{0.0,0.83,0.0}{{religion}}}
{\color[rgb]{0.0,0.203,0.0}{{to}}}
{\color[rgb]{0.0,0.165,0.0}{{the}}}
{\color[rgb]{0.349,0.0,0.0}{{islands}}}
{\color[rgb]{0.108,0.0,0.0}{{during}}}
{\color[rgb]{0.121,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.437,0.0}{{\textit{norse-era}}}}


==> examples/GRU_lime_prob_2167.tex <==
{\color[rgb]{0.0,0.593,0.0}{{initially}}}
{\color[rgb]{0.0,0.315,0.0}{{a}}}
{\color[rgb]{0.0,0.509,0.0}{{pagan}}}
{\color[rgb]{0.0,0.496,0.0}{{culture}}}
{\color[rgb]{0.0,0.541,0.0}{{,}}}
{\color[rgb]{0.0,0.183,0.0}{{detailed}}}
{\color[rgb]{0.0,0.382,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.586,0.0}{{about}}}
{\color[rgb]{0.0,0.244,0.0}{{the}}}
{\color[rgb]{0.0,0.577,0.0}{{return}}}
{\color[rgb]{0.0,0.245,0.0}{{of}}}
{\color[rgb]{0.0,0.184,0.0}{{the}}}
{\color[rgb]{0.0,0.461,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.247,0.0}{{to}}}
{\color[rgb]{0.0,0.293,0.0}{{the}}}
{\color[rgb]{0.15,0.0,0.0}{{islands}}}
{\color[rgb]{0.009,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.085,0.0}{{the}}}
{\color[rgb]{0.0,0.698,0.0}{{\textit{norse-era}}}}


==> examples/GRU_lime_raw_2167.tex <==
{\color[rgb]{0.0,0.593,0.0}{{initially}}}
{\color[rgb]{0.0,0.315,0.0}{{a}}}
{\color[rgb]{0.0,0.509,0.0}{{pagan}}}
{\color[rgb]{0.0,0.496,0.0}{{culture}}}
{\color[rgb]{0.0,0.541,0.0}{{,}}}
{\color[rgb]{0.0,0.183,0.0}{{detailed}}}
{\color[rgb]{0.0,0.382,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.586,0.0}{{about}}}
{\color[rgb]{0.0,0.244,0.0}{{the}}}
{\color[rgb]{0.0,0.577,0.0}{{return}}}
{\color[rgb]{0.0,0.245,0.0}{{of}}}
{\color[rgb]{0.0,0.184,0.0}{{the}}}
{\color[rgb]{0.0,0.461,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.247,0.0}{{to}}}
{\color[rgb]{0.0,0.293,0.0}{{the}}}
{\color[rgb]{0.15,0.0,0.0}{{islands}}}
{\color[rgb]{0.009,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.085,0.0}{{the}}}
{\color[rgb]{0.0,0.698,0.0}{{\textit{norse-era}}}}


==> examples/GRU_lrp_2167.tex <==
{\color[rgb]{0.036,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.244,0.0}{{a}}}
{\color[rgb]{0.0,0.084,0.0}{{pagan}}}
{\color[rgb]{0.0,0.084,0.0}{{culture}}}
{\color[rgb]{0.0,0.109,0.0}{{,}}}
{\color[rgb]{0.0,0.268,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.222,0.0}{{about}}}
{\color[rgb]{0.0,0.093,0.0}{{the}}}
{\color[rgb]{0.0,0.25,0.0}{{return}}}
{\color[rgb]{0.004,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.057,0.0}{{the}}}
{\color[rgb]{0.0,0.107,0.0}{{christian}}}
{\color[rgb]{0.0,0.312,0.0}{{religion}}}
{\color[rgb]{0.0,0.144,0.0}{{to}}}
{\color[rgb]{0.0,0.017,0.0}{{the}}}
{\color[rgb]{0.129,0.0,0.0}{{islands}}}
{\color[rgb]{0.063,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.033,0.0}{{the}}}
{\color[rgb]{0.0,0.274,0.0}{{\textit{norse-era}}}}


==> examples/GRU_occlusion-3_2167.tex <==
{\color[rgb]{0.0,0.046,0.0}{{initially}}}
{\color[rgb]{0.0,0.098,0.0}{{a}}}
{\color[rgb]{0.0,0.244,0.0}{{pagan}}}
{\color[rgb]{0.0,0.417,0.0}{{culture}}}
{\color[rgb]{0.0,0.767,0.0}{{,}}}
{\color[rgb]{0.0,0.844,0.0}{{detailed}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.806,0.0}{{about}}}
{\color[rgb]{0.0,0.621,0.0}{{the}}}
{\color[rgb]{0.0,0.405,0.0}{{return}}}
{\color[rgb]{0.0,0.248,0.0}{{of}}}
{\color[rgb]{0.0,0.305,0.0}{{the}}}
{\color[rgb]{0.0,0.545,0.0}{{christian}}}
{\color[rgb]{0.0,0.648,0.0}{{religion}}}
{\color[rgb]{0.0,0.729,0.0}{{to}}}
{\color[rgb]{0.0,0.508,0.0}{{the}}}
{\color[rgb]{0.0,0.326,0.0}{{islands}}}
{\color[rgb]{0.0,0.321,0.0}{{during}}}
{\color[rgb]{0.0,0.256,0.0}{{the}}}
{\color[rgb]{0.0,0.23,0.0}{{NNP}}}


==> examples/GRU_occlusion-7_2167.tex <==
{\color[rgb]{0.0,0.224,0.0}{{initially}}}
{\color[rgb]{0.0,0.313,0.0}{{a}}}
{\color[rgb]{0.0,0.436,0.0}{{pagan}}}
{\color[rgb]{0.0,0.614,0.0}{{culture}}}
{\color[rgb]{0.0,0.654,0.0}{{,}}}
{\color[rgb]{0.0,0.749,0.0}{{detailed}}}
{\color[rgb]{0.0,0.898,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.818,0.0}{{about}}}
{\color[rgb]{0.0,0.899,0.0}{{the}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{return}}}
{\color[rgb]{0.0,0.839,0.0}{{of}}}
{\color[rgb]{0.0,0.873,0.0}{{the}}}
{\color[rgb]{0.0,0.852,0.0}{{christian}}}
{\color[rgb]{0.0,0.798,0.0}{{religion}}}
{\color[rgb]{0.0,0.762,0.0}{{to}}}
{\color[rgb]{0.0,0.657,0.0}{{the}}}
{\color[rgb]{0.0,0.567,0.0}{{islands}}}
{\color[rgb]{0.0,0.516,0.0}{{during}}}
{\color[rgb]{0.0,0.449,0.0}{{the}}}
{\color[rgb]{0.0,0.387,0.0}{{NNP}}}


==> examples/GRU_occlusion_2167.tex <==
{\color[rgb]{0.25,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.121,0.0}{{a}}}
{\color[rgb]{0.0,0.018,0.0}{{pagan}}}
{\color[rgb]{0.023,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.325,0.0}{{,}}}
{\color[rgb]{0.0,0.246,0.0}{{detailed}}}
{\color[rgb]{0.0,0.891,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.175,0.0}{{about}}}
{\color[rgb]{0.0,0.023,0.0}{{the}}}
{\color[rgb]{0.0,0.165,0.0}{{return}}}
{\color[rgb]{0.0,0.099,0.0}{{of}}}
{\color[rgb]{0.0,0.056,0.0}{{the}}}
{\color[rgb]{0.0,0.051,0.0}{{christian}}}
{\color[rgb]{0.0,0.102,0.0}{{religion}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{to}}}
{\color[rgb]{0.0,0.123,0.0}{{the}}}
{\color[rgb]{0.111,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.206,0.0}{{during}}}
{\color[rgb]{0.002,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.093,0.0}{{NNP}}}


==> examples/GRU_omission-3_2167.tex <==
{\color[rgb]{0.239,0.0,0.0}{{initially}}}
{\color[rgb]{0.216,0.0,0.0}{{a}}}
{\color[rgb]{0.066,0.0,0.0}{{pagan}}}
{\color[rgb]{0.0,0.421,0.0}{{culture}}}
\textbf{\color[rgb]{0.0,0.873,0.0}{{,}}}
{\color[rgb]{0.0,0.582,0.0}{{detailed}}}
{\color[rgb]{0.0,0.193,0.0}{\underline {information}}}
{\color[rgb]{0.582,0.0,0.0}{{about}}}
{\color[rgb]{0.484,0.0,0.0}{{the}}}
{\color[rgb]{0.386,0.0,0.0}{{return}}}
{\color[rgb]{0.107,0.0,0.0}{{of}}}
{\color[rgb]{0.19,0.0,0.0}{{the}}}
{\color[rgb]{0.237,0.0,0.0}{{christian}}}
{\color[rgb]{0.177,0.0,0.0}{{religion}}}
{\color[rgb]{0.311,0.0,0.0}{{to}}}
{\color[rgb]{0.546,0.0,0.0}{{the}}}
{\color[rgb]{0.909,0.0,0.0}\textbf{{islands}}}
{\color[rgb]{0.721,0.0,0.0}{{during}}}
{\color[rgb]{0.237,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.285,0.0}{{\textit{norse-era}}}}


==> examples/GRU_omission-7_2167.tex <==
{\color[rgb]{0.0,0.156,0.0}{{initially}}}
{\color[rgb]{0.0,0.242,0.0}{{a}}}
{\color[rgb]{0.0,0.333,0.0}{{pagan}}}
{\color[rgb]{0.0,0.491,0.0}{{culture}}}
\textbf{\color[rgb]{0.0,0.558,0.0}{{,}}}
{\color[rgb]{0.0,0.537,0.0}{{detailed}}}
{\color[rgb]{0.0,0.527,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.276,0.0}{{about}}}
{\color[rgb]{0.0,0.21,0.0}{{the}}}
{\color[rgb]{0.0,0.138,0.0}{{return}}}
{\color[rgb]{0.134,0.0,0.0}{{of}}}
{\color[rgb]{0.34,0.0,0.0}{{the}}}
{\color[rgb]{0.458,0.0,0.0}{{christian}}}
{\color[rgb]{0.585,0.0,0.0}{{religion}}}
{\color[rgb]{0.707,0.0,0.0}{{to}}}
{\color[rgb]{0.824,0.0,0.0}{{the}}}
{\color[rgb]{0.909,0.0,0.0}\textbf{{islands}}}
{\color[rgb]{0.815,0.0,0.0}{{during}}}
{\color[rgb]{0.63,0.0,0.0}{{the}}}
{\color[rgb]{0.433,0.0,0.0}{{\textit{norse-era}}}}


==> examples/GRU_omission_2167.tex <==
{\color[rgb]{0.614,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.128,0.0}{{a}}}
{\color[rgb]{0.037,0.0,0.0}{{pagan}}}
{\color[rgb]{0.083,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.364,0.0}{{,}}}
{\color[rgb]{0.0,0.166,0.0}{{detailed}}}
{\color[rgb]{0.0,0.596,0.0}{\underline{information}}}
{\color[rgb]{0.39,0.0,0.0}{{about}}}
{\color[rgb]{0.154,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.074,0.0}{{return}}}
{\color[rgb]{0.0,0.026,0.0}{{of}}}
{\color[rgb]{0.0,0.005,0.0}{{the}}}
{\color[rgb]{0.033,0.0,0.0}{{christian}}}
{\color[rgb]{0.105,0.0,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.124,0.0,0.0}{{the}}}
{\color[rgb]{0.318,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.053,0.0}{{during}}}
{\color[rgb]{0.054,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.332,0.0}{{\textit{norse-era}}}}


==> examples/GRU_salience_prob_2167.tex <==
{\color[rgb]{0.551,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.335,0.0}{{a}}}
{\color[rgb]{0.0,0.068,0.0}{{pagan}}}
{\color[rgb]{0.06,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.336,0.0}{{,}}}
{\color[rgb]{0.0,0.212,0.0}{{detailed}}}
{\color[rgb]{0.0,0.56,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.542,0.0}{{about}}}
{\color[rgb]{0.0,0.101,0.0}{{the}}}
{\color[rgb]{0.0,0.156,0.0}{{return}}}
{\color[rgb]{0.0,0.02,0.0}{{of}}}
{\color[rgb]{0.0,0.065,0.0}{{the}}}
{\color[rgb]{0.0,0.084,0.0}{{christian}}}
{\color[rgb]{0.0,0.098,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.118,0.0}{{the}}}
{\color[rgb]{0.344,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.247,0.0}{{during}}}
{\color[rgb]{0.191,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.154,0.0}{{\textit{norse-era}}}}


==> examples/GRU_salience_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.522,0.0}{{initially}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{a}}}
{\color[rgb]{0.0,0.272,0.0}{{pagan}}}
{\color[rgb]{0.0,0.279,0.0}{{culture}}}
{\color[rgb]{0.0,0.208,0.0}{{,}}}
{\color[rgb]{0.0,0.249,0.0}{{detailed}}}
{\color[rgb]{0.0,0.591,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.231,0.0}{{about}}}
{\color[rgb]{0.0,0.055,0.0}{{the}}}
{\color[rgb]{0.0,0.213,0.0}{{return}}}
{\color[rgb]{0.0,0.166,0.0}{{of}}}
{\color[rgb]{0.0,0.069,0.0}{{the}}}
{\color[rgb]{0.0,0.16,0.0}{{christian}}}
{\color[rgb]{0.0,0.324,0.0}{{religion}}}
{\color[rgb]{0.0,0.646,0.0}{{to}}}
{\color[rgb]{0.0,0.009,0.0}{{the}}}
{\color[rgb]{0.332,0.0,0.0}{{islands}}}
{\color[rgb]{0.246,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.224,0.0}{{the}}}
{\color[rgb]{0.0,0.696,0.0}{{\textit{norse-era}}}}


==> examples/GRU_salience_raw_2167.tex <==
{\color[rgb]{0.529,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.324,0.0}{{a}}}
{\color[rgb]{0.0,0.074,0.0}{{pagan}}}
{\color[rgb]{0.03,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.336,0.0}{{,}}}
{\color[rgb]{0.0,0.178,0.0}{{detailed}}}
{\color[rgb]{0.0,0.554,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.451,0.0}{{about}}}
{\color[rgb]{0.0,0.091,0.0}{{the}}}
{\color[rgb]{0.0,0.224,0.0}{{return}}}
{\color[rgb]{0.079,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.072,0.0}{{the}}}
{\color[rgb]{0.0,0.107,0.0}{{christian}}}
{\color[rgb]{0.0,0.128,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.09,0.0}{{the}}}
{\color[rgb]{0.317,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.245,0.0}{{during}}}
{\color[rgb]{0.082,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.182,0.0}{{\textit{norse-era}}}}


==> examples/GRU_salience_raw_integrated_2167.tex <==
{\color[rgb]{0.018,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.671,0.0}{{a}}}
{\color[rgb]{0.0,0.19,0.0}{{pagan}}}
{\color[rgb]{0.0,0.163,0.0}{{culture}}}
{\color[rgb]{0.0,0.386,0.0}{{,}}}
{\color[rgb]{0.0,0.316,0.0}{{detailed}}}
{\color[rgb]{0.0,0.74,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.358,0.0}{{about}}}
{\color[rgb]{0.0,0.054,0.0}{{the}}}
{\color[rgb]{0.0,0.262,0.0}{{return}}}
{\color[rgb]{0.0,0.145,0.0}{{of}}}
{\color[rgb]{0.0,0.065,0.0}{{the}}}
{\color[rgb]{0.0,0.142,0.0}{{christian}}}
{\color[rgb]{0.0,0.214,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.059,0.0}{{the}}}
{\color[rgb]{0.332,0.0,0.0}{{islands}}}
{\color[rgb]{0.023,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.103,0.0}{{the}}}
{\color[rgb]{0.0,0.475,0.0}{{\textit{norse-era}}}}


==> examples/GRU_yelp_omission-5_3707.tex <==
{\color[rgb]{0.0458,0.0,0.0}{{That}}}
{\color[rgb]{0.1813,0.0,0.0}{{should}}}
{\color[rgb]{0.2234,0.0,0.0}{{have}}}
{\color[rgb]{0.271,0.0,0.0}{{been}}}
{\color[rgb]{0.3299,0.0,0.0}{{a}}}
{\color[rgb]{0.3298,0.0,0.0}{{flag}}}
{\color[rgb]{0.2197,0.0,0.0}{{for}}}
{\color[rgb]{0.1848,0.0,0.0}{{me}}}
{\color[rgb]{0.1291,0.0,0.0}{{for}}}
{\color[rgb]{0.0554,0.0,0.0}{{when}}}
{\color[rgb]{0.04,0.0,0.0}{{I}}}
{\color[rgb]{0.0372,0.0,0.0}{{came}}}
{\color[rgb]{0.0,0.0441,0.0}{{in}}}
{\color[rgb]{0.0,0.1221,0.0}{{.}}}
{\color[rgb]{0.0,0.1625,0.0}{\underline {Service}}}
{\color[rgb]{0.0,0.3019,0.0}{\underline {was}}}
{\color[rgb]{0.0,0.4871,0.0}{\underline {excellent}}}
{\color[rgb]{0.0,0.4818,0.0}{\underline {and}}}
{\color[rgb]{0.0,0.478,0.0}{\underline {food}}}
{\color[rgb]{0.0,0.4898,0.0}{\underline {very}}}
{\color[rgb]{0.0,0.4406,0.0}{\underline {good}}}
{\color[rgb]{0.0,0.2746,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.2001,0.0}{{This}}}
{\color[rgb]{0.0,0.1028,0.0}{{was}}}
{\color[rgb]{0.0,0.0274,0.0}{{a}}}
{\color[rgb]{0.0457,0.0,0.0}{{disaster}}}
{\color[rgb]{0.0,0.025,0.0}{{,}}}
{\color[rgb]{0.0,0.0377,0.0}{{and}}}
{\color[rgb]{0.0,0.0649,0.0}{{Penn}}}
{\color[rgb]{0.0,0.0807,0.0}{{Avenue}}}
{\color[rgb]{0.0,0.1015,0.0}{{Fish}}}
{\color[rgb]{0.0,0.0413,0.0}{{Company}}}
{\color[rgb]{0.0,0.0603,0.0}{{was}}}
{\color[rgb]{0.0,0.0757,0.0}{{responsible}}}
{\color[rgb]{0.0,0.1166,0.0}{{.}}}
{\color[rgb]{0.0,0.1151,0.0}{\underline {Very}}}
{\color[rgb]{0.0,0.1255,0.0}{\underline {clean}}}
{\color[rgb]{0.0,0.0894,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.0582,0.0}{{Did}}}
{\color[rgb]{0.0,0.0032,0.0}{{n't}}}
{\color[rgb]{0.0,0.0174,0.0}{{see}}}
{\color[rgb]{0.0,0.0055,0.0}{{that}}}
{\color[rgb]{0.0,0.0328,0.0}{{coming}}}
{\color[rgb]{0.0,0.0453,0.0}{{.}}}
{\color[rgb]{0.0,0.0671,0.0}{\underline {Always}}}
{\color[rgb]{0.0,0.0591,0.0}{\underline {a}}}
{\color[rgb]{0.0,0.069,0.0}{\underline {pleasure}}}
{\color[rgb]{0.0,0.0392,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.0398,0.0}{{I}}}
{\color[rgb]{0.0,0.0218,0.0}{{really}}}
{\color[rgb]{0.0637,0.0,0.0}{{felt}}}
{\color[rgb]{0.1582,0.0,0.0}{{like}}}
{\color[rgb]{0.2182,0.0,0.0}{{I}}}
{\color[rgb]{0.2595,0.0,0.0}{{had}}}
{\color[rgb]{0.2559,0.0,0.0}{{wasted}}}
{\color[rgb]{0.016,0.0,0.0}{{\$}}}
{\color[rgb]{0.0,0.2573,0.0}{{25}}}
{\color[rgb]{0.0,0.5123,0.0}{{.}}}
{\color[rgb]{0.0,0.6907,0.0}{\underline {Will}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {always}}}
{\color[rgb]{0.0,0.8091,0.0}{\underline {go}}}
{\color[rgb]{0.0,0.6149,0.0}{\underline {back}}}
{\color[rgb]{0.0,0.403,0.0}{\underline {Check}}}
{\color[rgb]{0.0,0.2492,0.0}{\underline {them}}}
{\color[rgb]{0.0,0.0398,0.0}{\underline {out}}}
{\color[rgb]{0.0,0.0182,0.0}{\underline {on}}}
{\color[rgb]{0.0,0.0821,0.0}{\underline {Beer}}}
{\color[rgb]{0.0,0.3414,0.0}{\underline {Advocate}}}
{\color[rgb]{0.0,0.3486,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.3391,0.0}{\underline {Friendly}}}
{\color[rgb]{0.0,0.294,0.0}{\underline {staff}}}
{\color[rgb]{0.0,0.2298,0.0}{\underline {.}}}

==> examples/LSTM_l2_prob_2167.tex <==
{\color[rgb]{0.0,0.106,0.0}{{initially}}}
{\color[rgb]{0.0,0.074,0.0}{{a}}}
{\color[rgb]{0.0,0.113,0.0}{{pagan}}}
{\color[rgb]{0.0,0.082,0.0}{{culture}}}
{\color[rgb]{0.0,0.096,0.0}{{,}}}
{\color[rgb]{0.0,0.135,0.0}{{detailed}}}
{\color[rgb]{0.0,0.465,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.617,0.0}{{about}}}
{\color[rgb]{0.0,0.364,0.0}{{the}}}
{\color[rgb]{0.0,0.226,0.0}{{return}}}
{\color[rgb]{0.0,0.282,0.0}{{of}}}
{\color[rgb]{0.0,0.147,0.0}{{the}}}
{\color[rgb]{0.0,0.296,0.0}{{christian}}}
{\color[rgb]{0.0,0.459,0.0}{{religion}}}
{\color[rgb]{0.0,0.18,0.0}{{to}}}
{\color[rgb]{0.0,0.233,0.0}{{the}}}
{\color[rgb]{0.0,0.439,0.0}{{islands}}}
{\color[rgb]{0.0,0.256,0.0}{{during}}}
{\color[rgb]{0.0,0.284,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/LSTM_l2_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.805,0.0}{{initially}}}
{\color[rgb]{0.0,0.514,0.0}{{a}}}
{\color[rgb]{0.0,0.256,0.0}{{pagan}}}
{\color[rgb]{0.0,0.249,0.0}{{culture}}}
{\color[rgb]{0.0,0.312,0.0}{{,}}}
{\color[rgb]{0.0,0.518,0.0}{{detailed}}}
{\color[rgb]{0.0,0.806,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.658,0.0}{{about}}}
{\color[rgb]{0.0,0.148,0.0}{{the}}}
{\color[rgb]{0.0,0.174,0.0}{{return}}}
{\color[rgb]{0.0,0.16,0.0}{{of}}}
{\color[rgb]{0.0,0.148,0.0}{{the}}}
{\color[rgb]{0.0,0.159,0.0}{{christian}}}
{\color[rgb]{0.0,0.241,0.0}{{religion}}}
{\color[rgb]{0.0,0.239,0.0}{{to}}}
{\color[rgb]{0.0,0.211,0.0}{{the}}}
{\color[rgb]{0.0,0.321,0.0}{{islands}}}
{\color[rgb]{0.0,0.539,0.0}{{during}}}
{\color[rgb]{0.0,0.595,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/LSTM_l2_raw_2167.tex <==
{\color[rgb]{0.0,0.099,0.0}{{initially}}}
{\color[rgb]{0.0,0.077,0.0}{{a}}}
{\color[rgb]{0.0,0.118,0.0}{{pagan}}}
{\color[rgb]{0.0,0.087,0.0}{{culture}}}
{\color[rgb]{0.0,0.101,0.0}{{,}}}
{\color[rgb]{0.0,0.134,0.0}{{detailed}}}
{\color[rgb]{0.0,0.466,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.618,0.0}{{about}}}
{\color[rgb]{0.0,0.348,0.0}{{the}}}
{\color[rgb]{0.0,0.213,0.0}{{return}}}
{\color[rgb]{0.0,0.285,0.0}{{of}}}
{\color[rgb]{0.0,0.139,0.0}{{the}}}
{\color[rgb]{0.0,0.282,0.0}{{christian}}}
{\color[rgb]{0.0,0.45,0.0}{{religion}}}
{\color[rgb]{0.0,0.174,0.0}{{to}}}
{\color[rgb]{0.0,0.232,0.0}{{the}}}
{\color[rgb]{0.0,0.425,0.0}{{islands}}}
{\color[rgb]{0.0,0.273,0.0}{{during}}}
{\color[rgb]{0.0,0.311,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/LSTM_l2_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.355,0.0}{{initially}}}
{\color[rgb]{0.0,0.237,0.0}{{a}}}
{\color[rgb]{0.0,0.119,0.0}{{pagan}}}
{\color[rgb]{0.0,0.302,0.0}{{culture}}}
{\color[rgb]{0.0,0.351,0.0}{{,}}}
{\color[rgb]{0.0,0.419,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.544,0.0}{{about}}}
{\color[rgb]{0.0,0.209,0.0}{{the}}}
{\color[rgb]{0.0,0.156,0.0}{{return}}}
{\color[rgb]{0.0,0.188,0.0}{{of}}}
{\color[rgb]{0.0,0.127,0.0}{{the}}}
{\color[rgb]{0.0,0.124,0.0}{{christian}}}
{\color[rgb]{0.0,0.172,0.0}{{religion}}}
{\color[rgb]{0.0,0.174,0.0}{{to}}}
{\color[rgb]{0.0,0.157,0.0}{{the}}}
{\color[rgb]{0.0,0.275,0.0}{{islands}}}
{\color[rgb]{0.0,0.217,0.0}{{during}}}
{\color[rgb]{0.0,0.352,0.0}{{the}}}
{\color[rgb]{0.0,0.817,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_lime_class_2167.tex <==
{\color[rgb]{0.0,0.284,0.0}{{initially}}}
{\color[rgb]{0.0,0.128,0.0}{{a}}}
{\color[rgb]{0.0,0.435,0.0}{{pagan}}}
{\color[rgb]{0.0,0.748,0.0}{{culture}}}
{\color[rgb]{0.0,0.756,0.0}{{,}}}
{\color[rgb]{0.0,0.309,0.0}{{detailed}}}
{\color[rgb]{0.0,0.48,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.359,0.0}{{the}}}
{\color[rgb]{0.0,0.457,0.0}{{return}}}
{\color[rgb]{0.0,0.341,0.0}{{of}}}
{\color[rgb]{0.0,0.273,0.0}{{the}}}
{\color[rgb]{0.0,0.439,0.0}{{christian}}}
{\color[rgb]{0.0,0.863,0.0}{{religion}}}
{\color[rgb]{0.0,0.139,0.0}{{to}}}
{\color[rgb]{0.0,0.098,0.0}{{the}}}
{\color[rgb]{0.415,0.0,0.0}{{islands}}}
{\color[rgb]{0.159,0.0,0.0}{{during}}}
{\color[rgb]{0.207,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.334,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_lime_raw_2167.tex <==
{\color[rgb]{0.0,0.347,0.0}{{initially}}}
{\color[rgb]{0.0,0.322,0.0}{{a}}}
{\color[rgb]{0.0,0.427,0.0}{{pagan}}}
{\color[rgb]{0.0,0.51,0.0}{{culture}}}
{\color[rgb]{0.0,0.365,0.0}{{,}}}
{\color[rgb]{0.0,0.146,0.0}{{detailed}}}
{\color[rgb]{0.0,0.392,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.439,0.0}{{about}}}
{\color[rgb]{0.0,0.239,0.0}{{the}}}
{\color[rgb]{0.0,0.551,0.0}{{return}}}
{\color[rgb]{0.0,0.145,0.0}{{of}}}
{\color[rgb]{0.0,0.143,0.0}{{the}}}
{\color[rgb]{0.0,0.385,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.099,0.0}{{to}}}
{\color[rgb]{0.0,0.204,0.0}{{the}}}
{\color[rgb]{0.168,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.05,0.0}{{during}}}
{\color[rgb]{0.0,0.078,0.0}{{the}}}
{\color[rgb]{0.0,0.527,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_lrp_2167.tex <==
{\color[rgb]{0.0,0.749,0.0}{{initially}}}
{\color[rgb]{0.0,0.203,0.0}{{a}}}
{\color[rgb]{0.2,0.0,0.0}{{pagan}}}
{\color[rgb]{0.0,0.513,0.0}{{culture}}}
{\color[rgb]{0.0,0.252,0.0}{{,}}}
{\color[rgb]{0.006,0.0,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.006,0.0,0.0}{{about}}}
{\color[rgb]{0.097,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.12,0.0}{{return}}}
{\color[rgb]{0.0,0.104,0.0}{{of}}}
{\color[rgb]{0.0,0.005,0.0}{{the}}}
{\color[rgb]{0.0,0.031,0.0}{{christian}}}
{\color[rgb]{0.0,0.068,0.0}{{religion}}}
{\color[rgb]{0.0,0.047,0.0}{{to}}}
{\color[rgb]{0.0,0.025,0.0}{{the}}}
{\color[rgb]{0.096,0.0,0.0}{{islands}}}
{\color[rgb]{0.079,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.063,0.0}{{the}}}
{\color[rgb]{0.0,0.158,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_newsgroup_omission-5_1028.tex <==
{\color[rgb]{0.0,0.013,0.0}{{Fair}}}
{\color[rgb]{0.0,0.0007,0.0}{{enough}}}
{\color[rgb]{0.0,0.0199,0.0}{{.}}}
{\color[rgb]{0.0,0.0343,0.0}{{2}}}
{\color[rgb]{0.0,0.0791,0.0}{{.}}}
{\color[rgb]{0.0,0.111,0.0}{{H.}}}
{\color[rgb]{0.0,0.147,0.0}\textit{{Rahmi}}}
{\color[rgb]{0.0,0.1483,0.0}{{,}}}
{\color[rgb]{0.0,0.1434,0.0}{{ed}}}
{\color[rgb]{0.0318,0.0,0.0}{{.}}}
{\color[rgb]{0.2098,0.0,0.0}{{There}}}
{\color[rgb]{0.4219,0.0,0.0}{{'s}}}
{\color[rgb]{0.6293,0.0,0.0}{{nothing}}}
{\color[rgb]{0.8193,0.0,0.0}{{punitive}}}
{\color[rgb]{0.787,0.0,0.0}{{or}}}
{\color[rgb]{0.7041,0.0,0.0}{{unjust}}}
{\color[rgb]{0.52,0.0,0.0}{{about}}}
{\color[rgb]{0.4745,0.0,0.0}{{it}}}
{\color[rgb]{0.4387,0.0,0.0}{{.}}}
{\color[rgb]{0.481,0.0,0.0}{{Thanks}}}
{\color[rgb]{0.5696,0.0,0.0}{{(}}}
{\color[rgb]{0.7041,0.0,0.0}{{Deletion}}}
{\color[rgb]{0.5879,0.0,0.0}{{)}}}
{\color[rgb]{0.4324,0.0,0.0}{{It}}}
{\color[rgb]{0.2901,0.0,0.0}{{is}}}
{\color[rgb]{0.1503,0.0,0.0}{{not}}}
{\color[rgb]{0.0106,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.0154,0.0}{{question}}}
{\color[rgb]{0.0,0.0038,0.0}{{of}}}
{\color[rgb]{0.0,0.0013,0.0}{{grammar}}}
{\color[rgb]{0.0,0.0023,0.0}{{,}}}
{\color[rgb]{0.0,0.0074,0.0}{{it}}}
{\color[rgb]{0.0233,0.0,0.0}{{is}}}
{\color[rgb]{0.0562,0.0,0.0}{{a}}}
{\color[rgb]{0.0914,0.0,0.0}{{question}}}
{\color[rgb]{0.1334,0.0,0.0}{{of}}}
{\color[rgb]{0.1815,0.0,0.0}{{modelling}}}
{\color[rgb]{0.1612,0.0,0.0}{{.}}}
{\color[rgb]{0.1253,0.0,0.0}{{So}}}
{\color[rgb]{0.0909,0.0,0.0}{{far}}}
{\color[rgb]{0.0501,0.0,0.0}{{only}}}
{\color[rgb]{0.003,0.0,0.0}{{two}}}
{\color[rgb]{0.0,0.0081,0.0}{{things}}}
{\color[rgb]{0.0,0.0062,0.0}{{seem}}}
{\color[rgb]{0.0128,0.0,0.0}{{to}}}
{\color[rgb]{0.0329,0.0,0.0}{{work}}}
{\color[rgb]{0.0726,0.0,0.0}{{:}}}
{\color[rgb]{0.1098,0.0,0.0}{{To}}}
{\color[rgb]{0.1449,0.0,0.0}{{kill}}}
{\color[rgb]{0.1276,0.0,0.0}{{it}}}
{\color[rgb]{0.1162,0.0,0.0}{{dead}}}
{\color[rgb]{0.0772,0.0,0.0}{{or}}}
{\color[rgb]{0.0499,0.0,0.0}{{to}}}
{\color[rgb]{0.0223,0.0,0.0}{{run}}}
{\color[rgb]{0.0267,0.0,0.0}{{into}}}
{\color[rgb]{0.0232,0.0,0.0}{{the}}}
{\color[rgb]{0.0594,0.0,0.0}{{house}}}
{\color[rgb]{0.0658,0.0,0.0}{{and}}}
{\color[rgb]{0.0787,0.0,0.0}{{close}}}
{\color[rgb]{0.0986,0.0,0.0}{{all}}}
{\color[rgb]{0.1219,0.0,0.0}{{doors}}}
{\color[rgb]{0.1085,0.0,0.0}{{and}}}
{\color[rgb]{0.0816,0.0,0.0}{{windows}}}
{\color[rgb]{0.0476,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0026,0.0}{{FTP}}}
{\color[rgb]{0.0,0.0408,0.0}{{to}}}
{\color[rgb]{0.0,0.0787,0.0}{{ftp.uu.net}}}
{\color[rgb]{0.0,0.0617,0.0}{{:}}}
{\color[rgb]{0.0,0.0447,0.0}\textit{{graphics/jpeg/jpegsrc.v}}}
{\color[rgb]{0.0,0.0172,0.0}{{?}}}
{\color[rgb]{0.0,0.0023,0.0}{{.tar.Z}}}
{\color[rgb]{0.011,0.0,0.0}{{Do}}}
{\color[rgb]{0.0,0.0272,0.0}{{n't}}}
{\color[rgb]{0.0,0.0776,0.0}{{forget}}}
{\color[rgb]{0.0,0.1291,0.0}{{to}}}
{\color[rgb]{0.0,0.1832,0.0}{{set}}}
{\color[rgb]{0.0,0.2212,0.0}{{binary}}}
{\color[rgb]{0.0,0.221,0.0}{{mode}}}
{\color[rgb]{0.0,0.1966,0.0}{{when}}}
{\color[rgb]{0.0,0.1737,0.0}{{you}}}
{\color[rgb]{0.0,0.0722,0.0}{{FTP}}}
{\color[rgb]{0.0475,0.0,0.0}{{tar}}}
{\color[rgb]{0.1668,0.0,0.0}{{files}}}
{\color[rgb]{0.2681,0.0,0.0}{{.}}}
{\color[rgb]{0.3293,0.0,0.0}{{Interplanetary}}}
{\color[rgb]{0.1742,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0613,0.0}{\underline {:}}}
{\color[rgb]{0.0,0.3444,0.0}{\underline {+49}}}
{\color[rgb]{0.0,0.5884,0.0}{\underline {231}}}
{\color[rgb]{0.0,0.7822,0.0}{\underline {755-4663}}}
{\color[rgb]{0.0,0.7987,0.0}{\underline {D-W4600}}}
{\color[rgb]{0.0,0.7305,0.0}{\underline {Dortmund}}}
{\color[rgb]{0.0,0.6311,0.0}{\underline {50}}}
{\color[rgb]{0.0,0.6738,0.0}{\underline {||}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {Fax}}}
{\color[rgb]{0.0,0.7893,0.0}{\underline {:}}}
{\color[rgb]{0.0,0.6978,0.0}{\underline {+49}}}
{\color[rgb]{0.0,0.6,0.0}{\underline {231}}}
{\color[rgb]{0.0,0.3919,0.0}{\underline {755-2386}}}


==> examples/LSTM_occlusion-3_2167.tex <==
{\color[rgb]{0.0,0.028,0.0}{{initially}}}
{\color[rgb]{0.0,0.048,0.0}{{a}}}
{\color[rgb]{0.0,0.092,0.0}{{pagan}}}
{\color[rgb]{0.0,0.198,0.0}{{culture}}}
{\color[rgb]{0.0,0.468,0.0}{{,}}}
{\color[rgb]{0.0,0.676,0.0}{{detailed}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.87,0.0}{{about}}}
{\color[rgb]{0.0,0.619,0.0}{{the}}}
{\color[rgb]{0.0,0.287,0.0}{{return}}}
{\color[rgb]{0.0,0.071,0.0}{{of}}}
{\color[rgb]{0.0,0.087,0.0}{{the}}}
{\color[rgb]{0.0,0.103,0.0}{{christian}}}
{\color[rgb]{0.0,0.083,0.0}{{religion}}}
{\color[rgb]{0.0,0.088,0.0}{{to}}}
{\color[rgb]{0.0,0.073,0.0}{{the}}}
{\color[rgb]{0.0,0.074,0.0}{{islands}}}
{\color[rgb]{0.0,0.226,0.0}{{during}}}
{\color[rgb]{0.0,0.327,0.0}{{the}}}
{\color[rgb]{0.0,0.421,0.0}{{NNP}}}


==> examples/LSTM_occlusion-7_2167.tex <==
{\color[rgb]{0.0,0.145,0.0}{{initially}}}
{\color[rgb]{0.0,0.23,0.0}{{a}}}
{\color[rgb]{0.0,0.373,0.0}{{pagan}}}
{\color[rgb]{0.0,0.555,0.0}{{culture}}}
{\color[rgb]{0.0,0.6,0.0}{{,}}}
{\color[rgb]{0.0,0.722,0.0}{{detailed}}}
{\color[rgb]{0.0,0.902,0.0}{\underline {information}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{about}}}
{\color[rgb]{0.0,0.876,0.0}{{the}}}
{\color[rgb]{0.0,0.771,0.0}{{return}}}
{\color[rgb]{0.0,0.624,0.0}{{of}}}
{\color[rgb]{0.0,0.617,0.0}{{the}}}
{\color[rgb]{0.0,0.546,0.0}{{christian}}}
{\color[rgb]{0.0,0.458,0.0}{{religion}}}
{\color[rgb]{0.0,0.395,0.0}{{to}}}
{\color[rgb]{0.0,0.427,0.0}{{the}}}
{\color[rgb]{0.0,0.474,0.0}{{islands}}}
{\color[rgb]{0.0,0.518,0.0}{{during}}}
{\color[rgb]{0.0,0.544,0.0}{{the}}}
{\color[rgb]{0.0,0.542,0.0}{{NNP}}}


==> examples/LSTM_occlusion_2167.tex <==
{\color[rgb]{0.0,0.034,0.0}{{initially}}}
{\color[rgb]{0.0,0.009,0.0}{{a}}}
{\color[rgb]{0.0,0.016,0.0}{{pagan}}}
{\color[rgb]{0.0,0.034,0.0}{{culture}}}
{\color[rgb]{0.0,0.134,0.0}{{,}}}
{\color[rgb]{0.0,0.144,0.0}{{detailed}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.439,0.0}{{about}}}
{\color[rgb]{0.019,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.001,0.0}{{return}}}
{\color[rgb]{0.0,0.06,0.0}{{of}}}
{\color[rgb]{0.044,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.04,0.0}{{christian}}}
{\color[rgb]{0.006,0.0,0.0}{{religion}}}
{\color[rgb]{0.0,0.101,0.0}{{to}}}
{\color[rgb]{0.004,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.123,0.0}{{islands}}}
{\color[rgb]{0.04,0.0,0.0}{{during}}}
{\color[rgb]{0.033,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.262,0.0}{{NNP}}}


==> examples/LSTM_omission-3_2167.tex <==
{\color[rgb]{0.0,0.024,0.0}{{initially}}}
{\color[rgb]{0.0,0.041,0.0}{{a}}}
{\color[rgb]{0.0,0.106,0.0}{{pagan}}}
{\color[rgb]{0.0,0.148,0.0}{{culture}}}
{\color[rgb]{0.0,0.191,0.0}{{,}}}
{\color[rgb]{0.0,0.319,0.0}{{detailed}}}
{\color[rgb]{0.0,0.428,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.484,0.0}{{about}}}
{\color[rgb]{0.0,0.235,0.0}{{the}}}
{\color[rgb]{0.0,0.003,0.0}{{return}}}
{\color[rgb]{0.104,0.0,0.0}{{of}}}
{\color[rgb]{0.156,0.0,0.0}{{the}}}
{\color[rgb]{0.037,0.0,0.0}{{christian}}}
{\color[rgb]{0.057,0.0,0.0}{{religion}}}
{\color[rgb]{0.0,0.12,0.0}{{to}}}
{\color[rgb]{0.0,0.123,0.0}{{the}}}
{\color[rgb]{0.0,0.199,0.0}{{islands}}}
{\color[rgb]{0.092,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.274,0.0}{{the}}}
{\color[rgb]{0.0,0.686,0.0}\textbf{{\textit{norse-era}}}}


==> examples/LSTM_omission-7_2167.tex <==
{\color[rgb]{0.0,0.189,0.0}{{initially}}}
{\color[rgb]{0.0,0.287,0.0}{{a}}}
{\color[rgb]{0.0,0.376,0.0}{{pagan}}}
{\color[rgb]{0.0,0.749,0.0}{{culture}}}
{\color[rgb]{0.0,0.815,0.0}{{,}}}
{\color[rgb]{0.0,0.87,0.0}{{detailed}}}
{\color[rgb]{0.0,0.887,0.0}\textbf{\underline {information}}}
{\color[rgb]{0.0,0.606,0.0}{{about}}}
{\color[rgb]{0.0,0.416,0.0}{{the}}}
{\color[rgb]{0.0,0.234,0.0}{{return}}}
{\color[rgb]{0.08,0.0,0.0}{{of}}}
{\color[rgb]{0.084,0.0,0.0}{{the}}}
{\color[rgb]{0.075,0.0,0.0}{{christian}}}
{\color[rgb]{0.083,0.0,0.0}{{religion}}}
{\color[rgb]{0.115,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.042,0.0}{{the}}}
{\color[rgb]{0.0,0.48,0.0}{{islands}}}
{\color[rgb]{0.0,0.26,0.0}{{during}}}
{\color[rgb]{0.0,0.511,0.0}{{the}}}
{\color[rgb]{0.0,0.795,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_omission_2167.tex <==
{\color[rgb]{0.0,0.027,0.0}{{initially}}}
{\color[rgb]{0.0,0.015,0.0}{{a}}}
{\color[rgb]{0.0,0.027,0.0}{{pagan}}}
{\color[rgb]{0.0,0.035,0.0}{{culture}}}
{\color[rgb]{0.0,0.102,0.0}{{,}}}
{\color[rgb]{0.0,0.135,0.0}{{detailed}}}
{\color[rgb]{0.0,0.132,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.055,0.0}{{about}}}
{\color[rgb]{0.098,0.0,0.0}{{the}}}
{\color[rgb]{0.019,0.0,0.0}{{return}}}
{\color[rgb]{0.0,0.075,0.0}{{of}}}
{\color[rgb]{0.062,0.0,0.0}{{the}}}
{\color[rgb]{0.032,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.02,0.0}{{religion}}}
{\color[rgb]{0.0,0.074,0.0}{{to}}}
{\color[rgb]{0.097,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.021,0.0}{{islands}}}
{\color[rgb]{0.0,0.035,0.0}{{during}}}
{\color[rgb]{0.036,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/LSTM_salience_prob_2167.tex <==
{\color[rgb]{0.0,0.077,0.0}{{initially}}}
{\color[rgb]{0.085,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.053,0.0}{{pagan}}}
{\color[rgb]{0.053,0.0,0.0}{{culture}}}
{\color[rgb]{0.035,0.0,0.0}{{,}}}
{\color[rgb]{0.082,0.0,0.0}{{detailed}}}
{\color[rgb]{0.377,0.0,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.335,0.0}{{the}}}
{\color[rgb]{0.0,0.009,0.0}{{return}}}
{\color[rgb]{0.029,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.156,0.0}{{the}}}
{\color[rgb]{0.0,0.28,0.0}{{christian}}}
{\color[rgb]{0.0,0.3,0.0}{{religion}}}
{\color[rgb]{0.0,0.312,0.0}{{to}}}
{\color[rgb]{0.436,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.172,0.0}{{islands}}}
{\color[rgb]{0.0,0.338,0.0}{{during}}}
{\color[rgb]{0.517,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.399,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_salience_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.438,0.0}{{initially}}}
{\color[rgb]{0.0,0.157,0.0}{{a}}}
{\color[rgb]{0.048,0.0,0.0}{{pagan}}}
{\color[rgb]{0.0,0.03,0.0}{{culture}}}
{\color[rgb]{0.0,0.29,0.0}{{,}}}
{\color[rgb]{0.0,0.377,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.499,0.0}{{about}}}
{\color[rgb]{0.004,0.0,0.0}{{the}}}
{\color[rgb]{0.011,0.0,0.0}{{return}}}
{\color[rgb]{0.0,0.088,0.0}{{of}}}
{\color[rgb]{0.0,0.018,0.0}{{the}}}
{\color[rgb]{0.0,0.048,0.0}{{christian}}}
{\color[rgb]{0.0,0.093,0.0}{{religion}}}
{\color[rgb]{0.0,0.153,0.0}{{to}}}
{\color[rgb]{0.0,0.044,0.0}{{the}}}
{\color[rgb]{0.224,0.0,0.0}{{islands}}}
{\color[rgb]{0.107,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.431,0.0}{{the}}}
{\color[rgb]{0.0,0.109,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_salience_raw_2167.tex <==
{\color[rgb]{0.0,0.076,0.0}{{initially}}}
{\color[rgb]{0.086,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.053,0.0}{{pagan}}}
{\color[rgb]{0.061,0.0,0.0}{{culture}}}
{\color[rgb]{0.042,0.0,0.0}{{,}}}
{\color[rgb]{0.08,0.0,0.0}{{detailed}}}
{\color[rgb]{0.388,0.0,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.357,0.0}{{the}}}
{\color[rgb]{0.0,0.007,0.0}{{return}}}
{\color[rgb]{0.022,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.137,0.0}{{the}}}
{\color[rgb]{0.0,0.238,0.0}{{christian}}}
{\color[rgb]{0.0,0.338,0.0}{{religion}}}
{\color[rgb]{0.0,0.296,0.0}{{to}}}
{\color[rgb]{0.404,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.187,0.0}{{islands}}}
{\color[rgb]{0.0,0.326,0.0}{{during}}}
{\color[rgb]{0.537,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.365,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_salience_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.223,0.0}{{initially}}}
{\color[rgb]{0.0,0.02,0.0}{{a}}}
{\color[rgb]{0.023,0.0,0.0}{{pagan}}}
{\color[rgb]{0.06,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.52,0.0}{{,}}}
{\color[rgb]{0.0,0.329,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.651,0.0}{{about}}}
{\color[rgb]{0.0,0.112,0.0}{{the}}}
{\color[rgb]{0.0,0.067,0.0}{{return}}}
{\color[rgb]{0.0,0.178,0.0}{{of}}}
{\color[rgb]{0.0,0.057,0.0}{{the}}}
{\color[rgb]{0.0,0.111,0.0}{{christian}}}
{\color[rgb]{0.0,0.01,0.0}{{religion}}}
{\color[rgb]{0.0,0.2,0.0}{{to}}}
{\color[rgb]{0.0,0.035,0.0}{{the}}}
{\color[rgb]{0.088,0.0,0.0}{{islands}}}
{\color[rgb]{0.078,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.227,0.0}{{the}}}
{\color[rgb]{0.0,0.314,0.0}{{\textit{norse-era}}}}


==> examples/LSTM_yelp_omission-5_5667.tex <==
{\color[rgb]{0.0523,0.0,0.0}{\underline {When}}}
{\color[rgb]{0.064,0.0,0.0}{\underline {we}}}
{\color[rgb]{0.0425,0.0,0.0}{\underline {went}}}
{\color[rgb]{0.0313,0.0,0.0}{\underline {to}}}
{\color[rgb]{0.0223,0.0,0.0}{\underline {pay}}}
{\color[rgb]{0.0,0.0357,0.0}{\underline {we}}}
{\color[rgb]{0.0,0.0566,0.0}{\underline {handing}}}
{\color[rgb]{0.0,0.0378,0.0}{\underline {the}}}
{\color[rgb]{0.0,0.0248,0.0}{\underline {guy}}}
{\color[rgb]{0.0,0.0267,0.0}{\underline {the}}}
{\color[rgb]{0.0,0.0355,0.0}{\underline {card}}}
{\color[rgb]{0.0,0.0389,0.0}{\underline {and}}}
{\color[rgb]{0.0,0.0481,0.0}{\underline {our}}}
{\color[rgb]{0.0,0.061,0.0}{\underline {payment}}}
{\color[rgb]{0.0,0.0484,0.0}{\underline {,}}}
{\color[rgb]{0.0,0.0322,0.0}{\underline {he}}}
{\color[rgb]{0.0,0.085,0.0}{\underline {checked}}}
{\color[rgb]{0.0,0.1374,0.0}{\underline {us}}}
{\color[rgb]{0.0,0.1926,0.0}{\underline {out}}}
{\color[rgb]{0.0,0.2769,0.0}{\underline {and}}}
{\color[rgb]{0.0,0.3492,0.0}{\underline {handed}}}
{\color[rgb]{0.0,0.3511,0.0}{\underline {back}}}
{\color[rgb]{0.0,0.3002,0.0}{\underline {our}}}
{\color[rgb]{0.0,0.2452,0.0}{\underline {payment}}}
{\color[rgb]{0.0,0.1652,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.096,0.0}{\underline {After}}}
{\color[rgb]{0.0,0.0288,0.0}{\underline {we}}}
{\color[rgb]{0.0,0.0191,0.0}{\underline {got}}}
{\color[rgb]{0.0,0.0111,0.0}{\underline {our}}}
{\color[rgb]{0.0,0.0111,0.0}{\underline {food}}}
{\color[rgb]{0.0,0.0197,0.0}{\underline {our}}}
{\color[rgb]{0.0,0.0445,0.0}{\underline {waitress}}}
{\color[rgb]{0.0,0.0239,0.0}{\underline {went}}}
{\color[rgb]{0.0,0.0008,0.0}\textit{\underline {M.I.A}}}
{\color[rgb]{0.0257,0.0,0.0}{\underline {.}}}
{\color[rgb]{0.0593,0.0,0.0}{{The}}}
{\color[rgb]{0.1104,0.0,0.0}{{room}}}
{\color[rgb]{0.1196,0.0,0.0}{{was}}}
{\color[rgb]{0.1287,0.0,0.0}{{good}}}
{\color[rgb]{0.1186,0.0,0.0}{{size}}}
{\color[rgb]{0.0949,0.0,0.0}{{.}}}
{\color[rgb]{0.0294,0.0,0.0}{{:}}}
{\color[rgb]{0.0,0.0439,0.0}{{)}}}
{\color[rgb]{0.0,0.1201,0.0}{{The}}}
{\color[rgb]{0.0,0.1819,0.0}{{waitresses}}}
{\color[rgb]{0.0,0.2203,0.0}{{need}}}
{\color[rgb]{0.0,0.1828,0.0}{{to}}}
{\color[rgb]{0.0,0.1362,0.0}{{work}}}
{\color[rgb]{0.0,0.0894,0.0}{{on}}}
{\color[rgb]{0.0,0.0475,0.0}{{their}}}
{\color[rgb]{0.0,0.0863,0.0}{{skills}}}
{\color[rgb]{0.0,0.135,0.0}{{a}}}
{\color[rgb]{0.0,0.1875,0.0}{{little}}}
{\color[rgb]{0.0,0.2553,0.0}{{more}}}
{\color[rgb]{0.0,0.3563,0.0}{{.}}}
{\color[rgb]{0.0,0.3864,0.0}{\underline {This}}}
{\color[rgb]{0.0,0.4575,0.0}{\underline {place}}}
{\color[rgb]{0.0,0.5239,0.0}{\underline {is}}}
{\color[rgb]{0.0,0.6422,0.0}{\underline {terrible}}}
{\color[rgb]{0.0,0.6208,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.675,0.0}{\underline {!}}}
{\color[rgb]{0.0,0.7121,0.0}{\underline {We}}}
{\color[rgb]{0.0,0.7505,0.0}{\underline {will}}}
{\color[rgb]{0.0,0.8494,0.0}{\underline {not}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {be}}}
{\color[rgb]{0.0,0.8519,0.0}{\underline {back}}}
{\color[rgb]{0.0,0.7436,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.6626,0.0}{\underline {Luckily}}}
{\color[rgb]{0.0,0.3594,0.0}{\underline {I}}}
{\color[rgb]{0.0,0.2001,0.0}{\underline {do}}}
{\color[rgb]{0.0,0.0773,0.0}{\underline {eat}}}
{\color[rgb]{0.0,0.0093,0.0}{\underline {salmon}}}
{\color[rgb]{0.0783,0.0,0.0}{\underline {,}}}
{\color[rgb]{0.0731,0.0,0.0}{\underline {so}}}
{\color[rgb]{0.0519,0.0,0.0}{\underline {I}}}
{\color[rgb]{0.0256,0.0,0.0}{\underline {headed}}}
{\color[rgb]{0.0121,0.0,0.0}{\underline {to}}}
{\color[rgb]{0.0054,0.0,0.0}{\underline {the}}}
{\color[rgb]{0.0,0.005,0.0}{\underline {smoked}}}
{\color[rgb]{0.0062,0.0,0.0}{\underline {salmon}}}
{\color[rgb]{0.0173,0.0,0.0}{\underline {station}}}
{\color[rgb]{0.0157,0.0,0.0}{\underline {.}}}
{\color[rgb]{0.0096,0.0,0.0}{{One}}}
{\color[rgb]{0.0046,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.0252,0.0}{{the}}}
{\color[rgb]{0.0,0.0715,0.0}{{few}}}
{\color[rgb]{0.0,0.0719,0.0}{{places}}}
{\color[rgb]{0.0,0.0672,0.0}{{where}}}
{\color[rgb]{0.0,0.0648,0.0}{{you}}}
{\color[rgb]{0.0,0.0036,0.0}{{can}}}
{\color[rgb]{0.0,0.0458,0.0}{{find}}}
{\color[rgb]{0.0,0.048,0.0}{{good}}}
{\color[rgb]{0.0,0.0504,0.0}{{Italian}}}
{\color[rgb]{0.0,0.0499,0.0}{{food}}}
{\color[rgb]{0.0,0.0851,0.0}{{.}}}

==> examples/QGRU_deeplift_2167.tex <==
{\color[rgb]{0.0,0.012,0.0}{{initially}}}
{\color[rgb]{0.0,0.054,0.0}{{a}}}
{\color[rgb]{0.0,0.106,0.0}{{pagan}}}
{\color[rgb]{0.0,0.048,0.0}{{culture}}}
{\color[rgb]{0.049,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.023,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.004,0.0}{{about}}}
{\color[rgb]{0.002,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.064,0.0}{{return}}}
{\color[rgb]{0.058,0.0,0.0}{{of}}}
{\color[rgb]{0.003,0.0,0.0}{{the}}}
{\color[rgb]{0.007,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.266,0.0}{{religion}}}
{\color[rgb]{0.0,0.147,0.0}{{to}}}
{\color[rgb]{0.0,0.017,0.0}{{the}}}
{\color[rgb]{0.096,0.0,0.0}{{islands}}}
{\color[rgb]{0.117,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.001,0.0}{{the}}}
{\color[rgb]{0.0,0.044,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_deeplift_233.tex <==
{\color[rgb]{0.0,0.082,0.0}{{the}}}
{\color[rgb]{0.0,0.039,0.0}{{most}}}
{\color[rgb]{0.0,0.043,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.091,0.0,0.0}{{to}}}
{\color[rgb]{0.005,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.274,0.0}{{village}}}


==> examples/QGRU_deeplift_970.tex <==
{\color[rgb]{0.165,0.0,0.0}{{the}}}
{\color[rgb]{0.186,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.067,0.0}{{in}}}
{\color[rgb]{0.019,0.0,0.0}{{the}}}
{\color[rgb]{0.026,0.0,0.0}{{series}}}


==> examples/QGRU_gamma_2167.tex <==
{\color[rgb]{0.081,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.012,0.0}{{a}}}
{\color[rgb]{0.0,0.013,0.0}{{pagan}}}
{\color[rgb]{0.0,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.045,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.073,0.0}{{about}}}
{\color[rgb]{0.001,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.126,0.0}{{return}}}
{\color[rgb]{0.0,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.049,0.0}{{christian}}}
{\color[rgb]{0.0,0.521,0.0}{{religion}}}
{\color[rgb]{0.0,0.175,0.0}{{to}}}
{\color[rgb]{0.0,0.124,0.0}{{the}}}
{\color[rgb]{0.282,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.02,0.0}{{during}}}
{\color[rgb]{0.0,0.07,0.0}{{the}}}
{\color[rgb]{0.0,0.313,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_gamma_233.tex <==
{\color[rgb]{0.0,0.001,0.0}{{the}}}
{\color[rgb]{0.004,0.0,0.0}{{most}}}
{\color[rgb]{0.097,0.0,0.0}{{recent}}}
{\color[rgb]{0.0,0.399,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.037,0.0}{{to}}}
{\color[rgb]{0.0,0.01,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}{{village}}}


==> examples/QGRU_gamma_970.tex <==
{\color[rgb]{0.095,0.0,0.0}{{the}}}
{\color[rgb]{0.036,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.063,0.0}{{in}}}
{\color[rgb]{0.016,0.0,0.0}{{the}}}
{\color[rgb]{0.043,0.0,0.0}{{series}}}


==> examples/QGRU_l2_prob_2167.tex <==
{\color[rgb]{0.0,0.237,0.0}{{initially}}}
{\color[rgb]{0.0,0.173,0.0}{{a}}}
{\color[rgb]{0.0,0.546,0.0}{{pagan}}}
{\color[rgb]{0.0,0.401,0.0}{{culture}}}
{\color[rgb]{0.0,0.436,0.0}{{,}}}
{\color[rgb]{0.0,0.54,0.0}{{detailed}}}
{\color[rgb]{0.0,0.407,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.192,0.0}{{about}}}
{\color[rgb]{0.0,0.059,0.0}{{the}}}
{\color[rgb]{0.0,0.068,0.0}{{return}}}
{\color[rgb]{0.0,0.074,0.0}{{of}}}
{\color[rgb]{0.0,0.099,0.0}{{the}}}
{\color[rgb]{0.0,0.45,0.0}{{christian}}}
{\color[rgb]{0.0,0.648,0.0}{{religion}}}
{\color[rgb]{0.0,0.81,0.0}{{to}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{the}}}
{\color[rgb]{0.0,0.624,0.0}{{islands}}}
{\color[rgb]{0.0,0.572,0.0}{{during}}}
{\color[rgb]{0.0,0.116,0.0}{{the}}}
{\color[rgb]{0.0,0.161,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_l2_prob_233.tex <==
{\color[rgb]{0.0,0.515,0.0}{{the}}}
{\color[rgb]{0.0,0.581,0.0}{{most}}}
{\color[rgb]{0.0,0.638,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.323,0.0}{{to}}}
{\color[rgb]{0.0,0.263,0.0}{{the}}}
{\color[rgb]{0.0,0.256,0.0}{{village}}}


==> examples/QGRU_l2_prob_970.tex <==
{\color[rgb]{0.0,0.6,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}{{other}}}
{\color[rgb]{0.0,0.558,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.27,0.0}{{in}}}
{\color[rgb]{0.0,0.24,0.0}{{the}}}
{\color[rgb]{0.0,0.275,0.0}{{series}}}


==> examples/QGRU_l2_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.342,0.0}{{initially}}}
{\color[rgb]{0.0,0.174,0.0}{{a}}}
{\color[rgb]{0.0,0.346,0.0}{{pagan}}}
{\color[rgb]{0.0,0.328,0.0}{{culture}}}
{\color[rgb]{0.0,0.293,0.0}{{,}}}
{\color[rgb]{0.0,0.261,0.0}{{detailed}}}
{\color[rgb]{0.0,0.493,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.327,0.0}{{about}}}
{\color[rgb]{0.0,0.164,0.0}{{the}}}
{\color[rgb]{0.0,0.286,0.0}{{return}}}
{\color[rgb]{0.0,0.171,0.0}{{of}}}
{\color[rgb]{0.0,0.169,0.0}{{the}}}
{\color[rgb]{0.0,0.358,0.0}{{christian}}}
{\color[rgb]{0.0,0.617,0.0}{{religion}}}
{\color[rgb]{0.0,0.722,0.0}{{to}}}
{\color[rgb]{0.0,0.776,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{islands}}}
{\color[rgb]{0.0,0.632,0.0}{{during}}}
{\color[rgb]{0.0,0.392,0.0}{{the}}}
{\color[rgb]{0.0,0.582,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_l2_prob_integrated_233.tex <==
{\color[rgb]{0.0,0.708,0.0}{{the}}}
{\color[rgb]{0.0,0.707,0.0}{{most}}}
{\color[rgb]{0.0,0.705,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.524,0.0}{{to}}}
{\color[rgb]{0.0,0.56,0.0}{{the}}}
{\color[rgb]{0.0,0.881,0.0}{{village}}}


==> examples/QGRU_l2_prob_integrated_970.tex <==
{\color[rgb]{0.0,0.614,0.0}{{the}}}
{\color[rgb]{0.0,0.775,0.0}{{other}}}
{\color[rgb]{0.0,0.848,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.504,0.0}{{in}}}
{\color[rgb]{0.0,0.368,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}{{series}}}


==> examples/QGRU_l2_raw_2167.tex <==
{\color[rgb]{0.0,0.248,0.0}{{initially}}}
{\color[rgb]{0.0,0.207,0.0}{{a}}}
{\color[rgb]{0.0,0.598,0.0}{{pagan}}}
{\color[rgb]{0.0,0.454,0.0}{{culture}}}
{\color[rgb]{0.0,0.492,0.0}{{,}}}
{\color[rgb]{0.0,0.576,0.0}{{detailed}}}
{\color[rgb]{0.0,0.418,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.163,0.0}{{about}}}
{\color[rgb]{0.0,0.066,0.0}{{the}}}
{\color[rgb]{0.0,0.1,0.0}{{return}}}
{\color[rgb]{0.0,0.105,0.0}{{of}}}
{\color[rgb]{0.0,0.134,0.0}{{the}}}
{\color[rgb]{0.0,0.453,0.0}{{christian}}}
{\color[rgb]{0.0,0.687,0.0}{{religion}}}
{\color[rgb]{0.0,0.806,0.0}{{to}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{the}}}
{\color[rgb]{0.0,0.669,0.0}{{islands}}}
{\color[rgb]{0.0,0.575,0.0}{{during}}}
{\color[rgb]{0.0,0.123,0.0}{{the}}}
{\color[rgb]{0.0,0.169,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_l2_raw_233.tex <==
{\color[rgb]{0.0,0.565,0.0}{{the}}}
{\color[rgb]{0.0,0.617,0.0}{{most}}}
{\color[rgb]{0.0,0.643,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.317,0.0}{{to}}}
{\color[rgb]{0.0,0.32,0.0}{{the}}}
{\color[rgb]{0.0,0.316,0.0}{{village}}}


==> examples/QGRU_l2_raw_970.tex <==
{\color[rgb]{0.0,0.588,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}{{other}}}
{\color[rgb]{0.0,0.537,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.286,0.0}{{in}}}
{\color[rgb]{0.0,0.251,0.0}{{the}}}
{\color[rgb]{0.0,0.273,0.0}{{series}}}


==> examples/QGRU_l2_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.253,0.0}{{initially}}}
{\color[rgb]{0.0,0.187,0.0}{{a}}}
{\color[rgb]{0.0,0.435,0.0}{{pagan}}}
{\color[rgb]{0.0,0.31,0.0}{{culture}}}
{\color[rgb]{0.0,0.288,0.0}{{,}}}
{\color[rgb]{0.0,0.363,0.0}{{detailed}}}
{\color[rgb]{0.0,0.481,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.24,0.0}{{about}}}
{\color[rgb]{0.0,0.114,0.0}{{the}}}
{\color[rgb]{0.0,0.197,0.0}{{return}}}
{\color[rgb]{0.0,0.146,0.0}{{of}}}
{\color[rgb]{0.0,0.161,0.0}{{the}}}
{\color[rgb]{0.0,0.407,0.0}{{christian}}}
{\color[rgb]{0.0,0.7,0.0}{{religion}}}
{\color[rgb]{0.0,0.822,0.0}{{to}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{the}}}
{\color[rgb]{0.0,0.882,0.0}{{islands}}}
{\color[rgb]{0.0,0.669,0.0}{{during}}}
{\color[rgb]{0.0,0.346,0.0}{{the}}}
{\color[rgb]{0.0,0.561,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_l2_raw_integrated_233.tex <==
{\color[rgb]{0.0,0.686,0.0}{{the}}}
{\color[rgb]{0.0,0.68,0.0}{{most}}}
{\color[rgb]{0.0,0.686,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.407,0.0}{{to}}}
{\color[rgb]{0.0,0.408,0.0}{{the}}}
{\color[rgb]{0.0,0.651,0.0}{{village}}}


==> examples/QGRU_l2_raw_integrated_970.tex <==
{\color[rgb]{0.0,0.656,0.0}{{the}}}
{\color[rgb]{0.0,0.847,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.485,0.0}{{in}}}
{\color[rgb]{0.0,0.386,0.0}{{the}}}
{\color[rgb]{0.0,0.766,0.0}{{series}}}


==> examples/QGRU_lime_class_2167.tex <==
{\color[rgb]{0.0,0.362,0.0}{{initially}}}
{\color[rgb]{0.0,0.111,0.0}{{a}}}
{\color[rgb]{0.0,0.391,0.0}{{pagan}}}
{\color[rgb]{0.0,0.674,0.0}{{culture}}}
{\color[rgb]{0.0,0.784,0.0}{{,}}}
{\color[rgb]{0.0,0.268,0.0}{{detailed}}}
{\color[rgb]{0.0,0.42,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.39,0.0}{{the}}}
{\color[rgb]{0.0,0.37,0.0}{{return}}}
{\color[rgb]{0.0,0.557,0.0}{{of}}}
{\color[rgb]{0.0,0.384,0.0}{{the}}}
{\color[rgb]{0.0,0.447,0.0}{{christian}}}
{\color[rgb]{0.0,0.742,0.0}{{religion}}}
{\color[rgb]{0.0,0.284,0.0}{{to}}}
{\color[rgb]{0.0,0.169,0.0}{{the}}}
{\color[rgb]{0.386,0.0,0.0}{{islands}}}
{\color[rgb]{0.225,0.0,0.0}{{during}}}
{\color[rgb]{0.282,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.208,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_lime_class_233.tex <==
{\color[rgb]{0.0,0.44,0.0}{{the}}}
{\color[rgb]{0.0,0.432,0.0}{{most}}}
{\color[rgb]{0.0,0.545,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.538,0.0}{{to}}}
{\color[rgb]{0.0,0.789,0.0}{{the}}}
{\color[rgb]{0.0,0.189,0.0}{{village}}}


==> examples/QGRU_lime_class_970.tex <==
{\color[rgb]{0.0,0.016,0.0}{{the}}}
{\color[rgb]{0.0,0.312,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.317,0.0}{{in}}}
{\color[rgb]{0.279,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0,0.0}{{series}}}


==> examples/QGRU_lime_prob_2167.tex <==
{\color[rgb]{0.0,0.666,0.0}{{initially}}}
{\color[rgb]{0.0,0.361,0.0}{{a}}}
{\color[rgb]{0.0,0.578,0.0}{{pagan}}}
{\color[rgb]{0.0,0.563,0.0}{{culture}}}
{\color[rgb]{0.0,0.621,0.0}{{,}}}
{\color[rgb]{0.0,0.208,0.0}{{detailed}}}
{\color[rgb]{0.0,0.411,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.679,0.0}{{about}}}
{\color[rgb]{0.0,0.331,0.0}{{the}}}
{\color[rgb]{0.0,0.528,0.0}{{return}}}
{\color[rgb]{0.0,0.427,0.0}{{of}}}
{\color[rgb]{0.0,0.291,0.0}{{the}}}
{\color[rgb]{0.0,0.428,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.461,0.0}{{to}}}
{\color[rgb]{0.0,0.418,0.0}{{the}}}
{\color[rgb]{0.241,0.0,0.0}{{islands}}}
{\color[rgb]{0.014,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.114,0.0}{{the}}}
{\color[rgb]{0.0,0.617,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_lime_prob_233.tex <==
{\color[rgb]{0.0,0.909,0.0}{{the}}}
{\color[rgb]{0.0,0.626,0.0}{{most}}}
{\color[rgb]{0.0,0.302,0.0}{{recent}}}
{\color[rgb]{0.0,0.869,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.43,0.0}{{to}}}
{\color[rgb]{0.0,0.735,0.0}{{the}}}
{\color[rgb]{0.0,0.758,0.0}{{village}}}


==> examples/QGRU_lime_prob_970.tex <==
{\color[rgb]{0.059,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.379,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.317,0.0}{{in}}}
{\color[rgb]{0.089,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.293,0.0}{{series}}}


==> examples/QGRU_lime_raw_2167.tex <==
{\color[rgb]{0.0,0.666,0.0}{{initially}}}
{\color[rgb]{0.0,0.361,0.0}{{a}}}
{\color[rgb]{0.0,0.578,0.0}{{pagan}}}
{\color[rgb]{0.0,0.563,0.0}{{culture}}}
{\color[rgb]{0.0,0.621,0.0}{{,}}}
{\color[rgb]{0.0,0.208,0.0}{{detailed}}}
{\color[rgb]{0.0,0.411,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.679,0.0}{{about}}}
{\color[rgb]{0.0,0.331,0.0}{{the}}}
{\color[rgb]{0.0,0.528,0.0}{{return}}}
{\color[rgb]{0.0,0.427,0.0}{{of}}}
{\color[rgb]{0.0,0.291,0.0}{{the}}}
{\color[rgb]{0.0,0.428,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.461,0.0}{{to}}}
{\color[rgb]{0.0,0.418,0.0}{{the}}}
{\color[rgb]{0.241,0.0,0.0}{{islands}}}
{\color[rgb]{0.014,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.114,0.0}{{the}}}
{\color[rgb]{0.0,0.617,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_lime_raw_233.tex <==
{\color[rgb]{0.0,0.909,0.0}{{the}}}
{\color[rgb]{0.0,0.626,0.0}{{most}}}
{\color[rgb]{0.0,0.302,0.0}{{recent}}}
{\color[rgb]{0.0,0.869,0.0}{\underline{addition}}}
{\color[rgb]{0.0,0.43,0.0}{{to}}}
{\color[rgb]{0.0,0.735,0.0}{{the}}}
{\color[rgb]{0.0,0.758,0.0}{{village}}}


==> examples/QGRU_lime_raw_970.tex <==
{\color[rgb]{0.059,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.379,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.317,0.0}{{in}}}
{\color[rgb]{0.089,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.293,0.0}{{series}}}


==> examples/QGRU_lrp_2167.tex <==
{\color[rgb]{0.0,0.018,0.0}{{initially}}}
{\color[rgb]{0.0,0.058,0.0}{{a}}}
{\color[rgb]{0.0,0.11,0.0}{{pagan}}}
{\color[rgb]{0.0,0.055,0.0}{{culture}}}
{\color[rgb]{0.024,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.025,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.012,0.0}{{about}}}
{\color[rgb]{0.011,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.172,0.0}{{return}}}
{\color[rgb]{0.158,0.0,0.0}{{of}}}
{\color[rgb]{0.01,0.0,0.0}{{the}}}
{\color[rgb]{0.03,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.532,0.0}{{religion}}}
{\color[rgb]{0.0,0.204,0.0}{{to}}}
{\color[rgb]{0.0,0.077,0.0}{{the}}}
{\color[rgb]{0.223,0.0,0.0}{{islands}}}
{\color[rgb]{0.204,0.0,0.0}{{during}}}
{\color[rgb]{0.001,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.121,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_lrp_233.tex <==
{\color[rgb]{0.079,0.0,0.0}{{the}}}
{\color[rgb]{0.092,0.0,0.0}{{most}}}
{\color[rgb]{0.0,0.004,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.026,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.025,0.0}{{the}}}
{\color[rgb]{0.0,0.551,0.0}{{village}}}


==> examples/QGRU_lrp_970.tex <==
{\color[rgb]{0.026,0.0,0.0}{{the}}}
{\color[rgb]{0.075,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.064,0.0}{{in}}}
{\color[rgb]{0.028,0.0,0.0}{{the}}}
{\color[rgb]{0.026,0.0,0.0}{{series}}}


==> examples/QGRU_newsgroup_grad_raw_dot_2297_short.tex <==
[...]
{\color[rgb]{0.0,0.0737,0.0}{\underline{I}}}
{\color[rgb]{0.0,0.0312,0.0}{\underline{am}}}
{\color[rgb]{0.0,0.0004,0.0}{\underline{considering}}}
{\color[rgb]{0.0,0.0003,0.0}{\underline{the}}}
{\color[rgb]{0.0267,0.0,0.0}\textit{\underline{purchse}}}
{\color[rgb]{0.1612,0.0,0.0}{\underline{of}}}
{\color[rgb]{0.1517,0.0,0.0}{\underline{a}}}
{\color[rgb]{0.1611,0.0,0.0}{\underline{1987}}}
{\color[rgb]{0.0,0.9091,0.0}{\underline{VW}}}
{\color[rgb]{0.0,0.4673,0.0}{\underline{Jetta}}}
{\color[rgb]{0.2619,0.0,0.0}\textit{\underline{GLI}}}
{\color[rgb]{0.2213,0.0,0.0}{\underline{with}}}
{\color[rgb]{0.172,0.0,0.0}\textit{\underline{87k}}}
{\color[rgb]{0.0699,0.0,0.0}{\underline{miles}}}
{\color[rgb]{0.0051,0.0,0.0}{\underline{on}}}
{\color[rgb]{0.0,0.0067,0.0}{\underline{it}}}
{\color[rgb]{0.0085,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.002,0.0,0.0}{{It}}}
{\color[rgb]{0.0,0.0012,0.0}{{has}}}
{\color[rgb]{0.0,0.0063,0.0}{{a}}}
{\color[rgb]{0.0,0.0046,0.0}{{very}}}
{\color[rgb]{0.0,0.0097,0.0}{{limited}}}
{\color[rgb]{0.011,0.0,0.0}{{(}}}
{\color[rgb]{0.0,0.0022,0.0}{{but}}}
{\color[rgb]{0.0,0.0,0.0}{{very}}}
{\color[rgb]{0.0003,0.0,0.0}{{important}}}
{\color[rgb]{0.0118,0.0,0.0}{{)}}}
{\color[rgb]{0.0084,0.0,0.0}{{role}}}
{\color[rgb]{0.0,0.0325,0.0}{{in}}}
{\color[rgb]{0.0,0.0223,0.0}{{the}}}
{\color[rgb]{0.0,0.0279,0.0}{{body}}}
{\color[rgb]{0.0,0.002,0.0}{{.}}}
{\color[rgb]{0.0079,0.0,0.0}{{That}}}
{\color[rgb]{0.0194,0.0,0.0}{{probably}}}
{\color[rgb]{0.0,0.0027,0.0}{{is}}}
{\color[rgb]{0.0,0.009,0.0}{{not}}}
{\color[rgb]{0.0,0.0232,0.0}{{true}}}
{\color[rgb]{0.0,0.1106,0.0}{{.}}}
{\color[rgb]{0.0521,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.3391,0.0}{{$>$}}}
{\color[rgb]{0.2213,0.0,0.0}{{Subsequent}}}
{\color[rgb]{0.2137,0.0,0.0}{{reads}}}
{\color[rgb]{0.0,0.2565,0.0}{{of}}}
{\color[rgb]{0.0,0.0858,0.0}{{the}}}
{\color[rgb]{0.0,0.0876,0.0}{{time}}}
{\color[rgb]{0.0163,0.0,0.0}{{add}}}
{\color[rgb]{0.0,0.0636,0.0}{{one}}}
{\color[rgb]{0.0,0.1291,0.0}{{.}}}
{\color[rgb]{0.0444,0.0,0.0}{{Bill}}}
{\color[rgb]{0.3967,0.0,0.0}{{Conner}}}
{\color[rgb]{0.0,0.401,0.0}{{,}}}
{\color[rgb]{0.0,0.2926,0.0}{{meet}}}
{\color[rgb]{0.0,0.268,0.0}{{Bill}}}
{\color[rgb]{0.4702,0.0,0.0}{{Conner}}}
{\color[rgb]{0.0183,0.0,0.0}{{.}}}


==> examples/QGRU_newsgroup_grad_raw_l2_2297_short.tex <==
[...]
{\color[rgb]{0.0,0.0925,0.0}{\underline{I}}}
{\color[rgb]{0.0,0.0629,0.0}{\underline{am}}}
{\color[rgb]{0.0,0.0219,0.0}{\underline{considering}}}
{\color[rgb]{0.0,0.0454,0.0}{\underline{the}}}
{\color[rgb]{0.0,0.1061,0.0}\textit{\underline{purchse}}}
{\color[rgb]{0.0,0.2529,0.0}{\underline{of}}}
{\color[rgb]{0.0,0.2914,0.0}{\underline{a}}}
{\color[rgb]{0.0,0.4368,0.0}{\underline{1987}}}
{\color[rgb]{0.0,0.6909,0.0}{\underline{VW}}}
{\color[rgb]{0.0,0.6041,0.0}{\underline{Jetta}}}
{\color[rgb]{0.0,0.3941,0.0}\textit{\underline{GLI}}}
{\color[rgb]{0.0,0.3551,0.0}{\underline{with}}}
{\color[rgb]{0.0,0.2691,0.0}\textit{\underline{87k}}}
{\color[rgb]{0.0,0.154,0.0}{\underline{miles}}}
{\color[rgb]{0.0,0.0758,0.0}{\underline{on}}}
{\color[rgb]{0.0,0.0821,0.0}{\underline{it}}}
{\color[rgb]{0.0,0.0573,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0191,0.0}{{It}}}
{\color[rgb]{0.0,0.0192,0.0}{{has}}}
{\color[rgb]{0.0,0.0227,0.0}{{a}}}
{\color[rgb]{0.0,0.0216,0.0}{{very}}}
{\color[rgb]{0.0,0.022,0.0}{{limited}}}
{\color[rgb]{0.0,0.0224,0.0}{{(}}}
{\color[rgb]{0.0,0.0251,0.0}{{but}}}
{\color[rgb]{0.0,0.0004,0.0}{{very}}}
{\color[rgb]{0.0,0.0011,0.0}{{important}}}
{\color[rgb]{0.0,0.0216,0.0}{{)}}}
{\color[rgb]{0.0,0.0863,0.0}{{role}}}
{\color[rgb]{0.0,0.082,0.0}{{in}}}
{\color[rgb]{0.0,0.0731,0.0}{{the}}}
{\color[rgb]{0.0,0.0888,0.0}{{body}}}
{\color[rgb]{0.0,0.0851,0.0}{{.}}}
{\color[rgb]{0.0,0.0145,0.0}{{That}}}
{\color[rgb]{0.0,0.0289,0.0}{{probably}}}
{\color[rgb]{0.0,0.0309,0.0}{{is}}}
{\color[rgb]{0.0,0.0309,0.0}{{not}}}
{\color[rgb]{0.0,0.0575,0.0}{{true}}}
{\color[rgb]{0.0,0.1787,0.0}{{.}}}
{\color[rgb]{0.0,0.4376,0.0}{{MS}}}
{\color[rgb]{0.0,0.3442,0.0}{{$>$}}}
{\color[rgb]{0.0,0.5873,0.0}{{Subsequent}}}
{\color[rgb]{0.0,0.559,0.0}{{reads}}}
{\color[rgb]{0.0,0.447,0.0}{{of}}}
{\color[rgb]{0.0,0.2992,0.0}{{the}}}
{\color[rgb]{0.0,0.2676,0.0}{{time}}}
{\color[rgb]{0.0,0.1744,0.0}{{add}}}
{\color[rgb]{0.0,0.2203,0.0}{{one}}}
{\color[rgb]{0.0,0.2695,0.0}{{.}}}
{\color[rgb]{0.0,0.2903,0.0}{{Bill}}}
{\color[rgb]{0.0,0.9054,0.0}{{Conner}}}
{\color[rgb]{0.0,0.72,0.0}{{,}}}
{\color[rgb]{0.0,0.7634,0.0}{{meet}}}
{\color[rgb]{0.0,0.7455,0.0}{{Bill}}}
{\color[rgb]{0.0,0.9091,0.0}{\textbf{Conner}}}
{\color[rgb]{0.0,0.2914,0.0}{{.}}}


==> examples/QGRU_newsgroup_grad_raw_l2_short_2297.tex <==
[...]
{\color[rgb]{0.0,0.1069,0.0}{{It}}}
{\color[rgb]{0.0,0.2209,0.0}{{states}}}
{\color[rgb]{0.0,0.2193,0.0}{{clearly}}}
{\color[rgb]{0.0,0.2473,0.0}{{that}}}
{\color[rgb]{0.0,0.4797,0.0}{{the}}}
{\color[rgb]{0.0,0.5243,0.0}{{visitors}}}
{\color[rgb]{0.0,0.3683,0.0}{{were}}}
{\color[rgb]{0.0,0.549,0.0}{{angels}}}
{\color[rgb]{0.0,0.4078,0.0}{{.}}}
{\color[rgb]{0.0,0.0925,0.0}{\underline{I}}}
{\color[rgb]{0.0,0.0629,0.0}{\underline{am}}}
{\color[rgb]{0.0,0.0219,0.0}{\underline{considering}}}
{\color[rgb]{0.0,0.0454,0.0}{\underline{the}}}
{\color[rgb]{0.0,0.1061,0.0}\textit{\underline{purchse}}}
{\color[rgb]{0.0,0.2529,0.0}{\underline{of}}}
{\color[rgb]{0.0,0.2914,0.0}{\underline{a}}}
{\color[rgb]{0.0,0.4368,0.0}{\underline{1987}}}
{\color[rgb]{0.0,0.6909,0.0}{\underline{VW}}}
{\color[rgb]{0.0,0.6041,0.0}{\underline{Jetta}}}
{\color[rgb]{0.0,0.3941,0.0}\textit{\underline{GLI}}}
{\color[rgb]{0.0,0.3551,0.0}{\underline{with}}}
{\color[rgb]{0.0,0.2691,0.0}\textit{\underline{87k}}}
{\color[rgb]{0.0,0.154,0.0}{\underline{miles}}}
{\color[rgb]{0.0,0.0758,0.0}{\underline{on}}}
{\color[rgb]{0.0,0.0821,0.0}{\underline{it}}}
{\color[rgb]{0.0,0.0573,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0191,0.0}{{It}}}
{\color[rgb]{0.0,0.0192,0.0}{{has}}}
{\color[rgb]{0.0,0.0227,0.0}{{a}}}
{\color[rgb]{0.0,0.0216,0.0}{{very}}}
{\color[rgb]{0.0,0.022,0.0}{{limited}}}
{\color[rgb]{0.0,0.0224,0.0}{{(}}}
{\color[rgb]{0.0,0.0251,0.0}{{but}}}
{\color[rgb]{0.0,0.0004,0.0}{{very}}}
{\color[rgb]{0.0,0.0011,0.0}{{important}}}
{\color[rgb]{0.0,0.0216,0.0}{{)}}}
{\color[rgb]{0.0,0.0863,0.0}{{role}}}
{\color[rgb]{0.0,0.082,0.0}{{in}}}
{\color[rgb]{0.0,0.0731,0.0}{{the}}}
{\color[rgb]{0.0,0.0888,0.0}{{body}}}
{\color[rgb]{0.0,0.0851,0.0}{{.}}}
{\color[rgb]{0.0,0.0145,0.0}{{That}}}
{\color[rgb]{0.0,0.0289,0.0}{{probably}}}
{\color[rgb]{0.0,0.0309,0.0}{{is}}}
{\color[rgb]{0.0,0.0309,0.0}{{not}}}
{\color[rgb]{0.0,0.0575,0.0}{{true}}}
{\color[rgb]{0.0,0.1787,0.0}{{.}}}
{\color[rgb]{0.0,0.4376,0.0}{{MS}}}
{\color[rgb]{0.0,0.3442,0.0}{{$>$}}}
{\color[rgb]{0.0,0.5873,0.0}{{Subsequent}}}
{\color[rgb]{0.0,0.559,0.0}{{reads}}}
{\color[rgb]{0.0,0.447,0.0}{{of}}}
{\color[rgb]{0.0,0.2992,0.0}{{the}}}
{\color[rgb]{0.0,0.2676,0.0}{{time}}}
{\color[rgb]{0.0,0.1744,0.0}{{add}}}
{\color[rgb]{0.0,0.2203,0.0}{{one}}}
{\color[rgb]{0.0,0.2695,0.0}{{.}}}
{\color[rgb]{0.0,0.2903,0.0}{{Bill}}}
{\color[rgb]{0.0,0.9054,0.0}{{Conner}}}
{\color[rgb]{0.0,0.72,0.0}{{,}}}
{\color[rgb]{0.0,0.7634,0.0}{{meet}}}
{\color[rgb]{0.0,0.7455,0.0}{{Bill}}}
{\color[rgb]{0.0,0.9091,0.0}{\textbf{Conner}}}
{\color[rgb]{0.0,0.2914,0.0}{{.}}}


==> examples/QGRU_newsgroup_lime_raw_short_2297.tex <==
[...]
{\color[rgb]{0.0,0.0,0.0}{{It}}}
{\color[rgb]{0.0,0.0,0.0}{{states}}}
{\color[rgb]{0.0225,0.0,0.0}{{clearly}}}
{\color[rgb]{0.0227,0.0,0.0}{{that}}}
{\color[rgb]{0.0,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0253,0.0}{{visitors}}}
{\color[rgb]{0.0,0.0625,0.0}{{were}}}
{\color[rgb]{0.046,0.0,0.0}{{angels}}}
{\color[rgb]{0.0167,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{\underline {I}}}
{\color[rgb]{0.0,0.0,0.0}{\underline {am}}}
{\color[rgb]{0.0,0.0,0.0}{\underline {considering}}}
{\color[rgb]{0.0,0.0367,0.0}{\underline {the}}}
{\color[rgb]{0.0,0.0,0.0}\textit{\underline {purchse}}}
{\color[rgb]{0.0607,0.0,0.0}{\underline {of}}}
{\color[rgb]{0.0528,0.0,0.0}{\underline {a}}}
{\color[rgb]{0.0545,0.0,0.0}{\underline {1987}}}
{\color[rgb]{0.0,0.6647,0.0}{\underline {VW}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {Jetta}}}
{\color[rgb]{0.0,0.1912,0.0}\textit{\underline {GLI}}}
{\color[rgb]{0.0,0.0445,0.0}{\underline {with}}}
{\color[rgb]{0.0,0.0032,0.0}\textit{\underline {87k}}}
{\color[rgb]{0.0,0.1015,0.0}{\underline {miles}}}
{\color[rgb]{0.0,0.0461,0.0}{\underline {on}}}
{\color[rgb]{0.0,0.0,0.0}{\underline {it}}}
{\color[rgb]{0.0,0.0142,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.0,0.0}{{It}}}
{\color[rgb]{0.0202,0.0,0.0}{{has}}}
{\color[rgb]{0.0133,0.0,0.0}{{a}}}
{\color[rgb]{0.0115,0.0,0.0}{{very}}}
{\color[rgb]{0.0,0.0393,0.0}{{limited}}}
{\color[rgb]{0.0,0.0,0.0}{{(}}}
{\color[rgb]{0.0,0.0,0.0}{{but}}}
{\color[rgb]{0.0,0.005,0.0}{{very}}}
{\color[rgb]{0.0,0.0505,0.0}{{important}}}
{\color[rgb]{0.0,0.0,0.0}{{)}}}
{\color[rgb]{0.0876,0.0,0.0}{{role}}}
{\color[rgb]{0.0251,0.0,0.0}{{in}}}
{\color[rgb]{0.007,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.0691,0.0}{{body}}}
{\color[rgb]{0.0,0.013,0.0}{{.}}}
{\color[rgb]{0.0,0.0201,0.0}{{That}}}
{\color[rgb]{0.0,0.0093,0.0}{{probably}}}
{\color[rgb]{0.0,0.0,0.0}{{is}}}
{\color[rgb]{0.0136,0.0,0.0}{{not}}}
{\color[rgb]{0.0,0.0,0.0}{{true}}}
{\color[rgb]{0.0,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{MS}}}
{\color[rgb]{0.0,0.0,0.0}{{$>$}}}
{\color[rgb]{0.0,0.0,0.0}{{Subsequent}}}
{\color[rgb]{0.0179,0.0,0.0}{{reads}}}
{\color[rgb]{0.0276,0.0,0.0}{{of}}}
{\color[rgb]{0.0031,0.0,0.0}{{the}}}
{\color[rgb]{0.0028,0.0,0.0}{{time}}}
{\color[rgb]{0.0,0.0,0.0}{{add}}}
{\color[rgb]{0.0,0.0122,0.0}{{one}}}
{\color[rgb]{0.0,0.0262,0.0}{{.}}}
{\color[rgb]{0.0,0.0,0.0}{{Bill}}}
{\color[rgb]{0.0635,0.0,0.0}{{Conner}}}
{\color[rgb]{0.0,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.0,0.0}{{meet}}}
{\color[rgb]{0.0,0.0,0.0}{{Bill}}}
{\color[rgb]{0.0536,0.0,0.0}{{Conner}}}
{\color[rgb]{0.0055,0.0,0.0}{{.}}}


==> examples/QGRU_newsgroup_lrp_2297_short.tex <==
[...]
{\color[rgb]{0.0,0.001,0.0}{\underline{I}}}
{\color[rgb]{0.0,0.0014,0.0}{\underline{am}}}
{\color[rgb]{0.0,0.0075,0.0}{\underline{considering}}}
{\color[rgb]{0.0,0.0011,0.0}{\underline{the}}}
{\color[rgb]{0.0,0.0152,0.0}\textit{\underline{purchse}}}
{\color[rgb]{0.0216,0.0,0.0}{\underline{of}}}
{\color[rgb]{0.0,0.0094,0.0}{\underline{a}}}
{\color[rgb]{0.0454,0.0,0.0}{\underline{1987}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {VW}}}
{\color[rgb]{0.0,0.6319,0.0}{\underline{Jetta}}}
{\color[rgb]{0.0,0.0209,0.0}\textit{\underline{GLI}}}
{\color[rgb]{0.0,0.0198,0.0}{\underline{with}}}
{\color[rgb]{0.002,0.0,0.0}\textit{\underline{87k}}}
{\color[rgb]{0.0,0.0326,0.0}{\underline{miles}}}
{\color[rgb]{0.0,0.0051,0.0}{\underline{on}}}
{\color[rgb]{0.0,0.001,0.0}{\underline{it}}}
{\color[rgb]{0.0118,0.0,0.0}{\underline{.}}}
{\color[rgb]{0.0,0.0006,0.0}{{It}}}
{\color[rgb]{0.0027,0.0,0.0}{{has}}}
{\color[rgb]{0.0015,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.0018,0.0}{{very}}}
{\color[rgb]{0.0,0.0018,0.0}{{limited}}}
{\color[rgb]{0.0004,0.0,0.0}{{(}}}
{\color[rgb]{0.0012,0.0,0.0}{{but}}}
{\color[rgb]{0.0,0.001,0.0}{{very}}}
{\color[rgb]{0.0,0.0011,0.0}{{important}}}
{\color[rgb]{0.0007,0.0,0.0}{{)}}}
{\color[rgb]{0.0107,0.0,0.0}{{role}}}
{\color[rgb]{0.0,0.0104,0.0}{{in}}}
{\color[rgb]{0.0,0.0003,0.0}{{the}}}
{\color[rgb]{0.0,0.0304,0.0}{{body}}}
{\color[rgb]{0.0097,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0095,0.0}{{That}}}
{\color[rgb]{0.0,0.0097,0.0}{{probably}}}
{\color[rgb]{0.0,0.0034,0.0}{{is}}}
{\color[rgb]{0.0,0.0034,0.0}{{not}}}
{\color[rgb]{0.0,0.0019,0.0}{{true}}}
{\color[rgb]{0.0,0.0009,0.0}{{.}}}
{\color[rgb]{0.0,0.0252,0.0}{{MS}}}
{\color[rgb]{0.0,0.0336,0.0}{{$>$}}}
{\color[rgb]{0.0,0.0005,0.0}{{Subsequent}}}
{\color[rgb]{0.0472,0.0,0.0}{{reads}}}
{\color[rgb]{0.0,0.0252,0.0}{{of}}}
{\color[rgb]{0.0059,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.013,0.0}{{time}}}
{\color[rgb]{0.0206,0.0,0.0}{{add}}}
{\color[rgb]{0.0099,0.0,0.0}{{one}}}
{\color[rgb]{0.0,0.0286,0.0}{{.}}}
{\color[rgb]{0.051,0.0,0.0}{{Bill}}}
{\color[rgb]{0.0361,0.0,0.0}{{Conner}}}
{\color[rgb]{0.0,0.0135,0.0}{{,}}}
{\color[rgb]{0.026,0.0,0.0}{{meet}}}
{\color[rgb]{0.0,0.0689,0.0}{{Bill}}}
{\color[rgb]{0.0512,0.0,0.0}{{Conner}}}
{\color[rgb]{0.026,0.0,0.0}{{.}}}


==> examples/QGRU_newsgroup_omission-5_630.tex <==
{\color[rgb]{0.0,0.0255,0.0}{{If}}}
{\color[rgb]{0.0,0.0544,0.0}{{you}}}
{\color[rgb]{0.0,0.0673,0.0}{{find}}}
{\color[rgb]{0.0,0.0732,0.0}{{faith}}}
{\color[rgb]{0.0,0.0677,0.0}{{to}}}
{\color[rgb]{0.0,0.0445,0.0}{{be}}}
{\color[rgb]{0.0,0.0568,0.0}{{honest}}}
{\color[rgb]{0.0,0.0373,0.0}{{,}}}
{\color[rgb]{0.0,0.0285,0.0}{{show}}}
{\color[rgb]{0.0,0.0797,0.0}{{me}}}
{\color[rgb]{0.0,0.15,0.0}{{how}}}
{\color[rgb]{0.0,0.1552,0.0}{{.}}}
{\color[rgb]{0.0,0.1583,0.0}{{David}}}
{\color[rgb]{0.0,0.1589,0.0}{{The}}}
{\color[rgb]{0.0,0.1294,0.0}{{whole}}}
{\color[rgb]{0.0,0.0618,0.0}{{denominational}}}
{\color[rgb]{0.0,0.039,0.0}{{mindset}}}
{\color[rgb]{0.0,0.0954,0.0}{{only}}}
{\color[rgb]{0.0,0.1295,0.0}{{causes}}}
{\color[rgb]{0.0,0.0984,0.0}{{more}}}
{\color[rgb]{0.0,0.0926,0.0}{{problems}}}
{\color[rgb]{0.0,0.1157,0.0}{{,}}}
{\color[rgb]{0.0,0.1164,0.0}{{sadly}}}
{\color[rgb]{0.0,0.1251,0.0}{{.}}}
{\color[rgb]{0.0,0.1654,0.0}{{(}}}
{\color[rgb]{0.0,0.208,0.0}{{See}}}
{\color[rgb]{0.0,0.1631,0.0}{{section}}}
{\color[rgb]{0.0,0.1176,0.0}{{7}}}
{\color[rgb]{0.0,0.1016,0.0}{{for}}}
{\color[rgb]{0.0,0.132,0.0}{{details}}}
{\color[rgb]{0.0,0.131,0.0}{{.}}}
{\color[rgb]{0.0,0.1129,0.0}{{)}}}
{\color[rgb]{0.0,0.2844,0.0}{{Thank}}}
{\color[rgb]{0.0,0.4476,0.0}{{you}}}
{\color[rgb]{0.0,0.5782,0.0}{{.}}}
{\color[rgb]{0.0,0.7185,0.0}{\underline {'The}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {Armenians}}}
{\color[rgb]{0.0,0.8287,0.0}{\underline {just}}}
{\color[rgb]{0.0,0.7192,0.0}{\underline {shot}}}
{\color[rgb]{0.0,0.5895,0.0}{\underline {and}}}
{\color[rgb]{0.0,0.4369,0.0}{\underline {shot}}}
{\color[rgb]{0.0,0.3032,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.2535,0.0}{{Maybe}}}
{\color[rgb]{0.0,0.1917,0.0}\textit{{coz}}}
{\color[rgb]{0.0,0.1401,0.0}{{they}}}
{\color[rgb]{0.0,0.1208,0.0}{{'re}}}
{\color[rgb]{0.0,0.1075,0.0}\textit{{'quality'}}}
{\color[rgb]{0.0,0.0787,0.0}{{cars}}}
{\color[rgb]{0.0,0.0836,0.0}{{;}}}
{\color[rgb]{0.0,0.0991,0.0}{{-}}}
{\color[rgb]{0.0,0.0991,0.0}{{)}}}
{\color[rgb]{0.0,0.0889,0.0}{{200}}}
{\color[rgb]{0.0,0.0828,0.0}\textit{{posts/day}}}
{\color[rgb]{0.0,0.0832,0.0}{{.}}}
{\color[rgb]{0.0,0.0927,0.0}{{can}}}
{\color[rgb]{0.0,0.109,0.0}{{you}}}
{\color[rgb]{0.0,0.1195,0.0}{{explain}}}
{\color[rgb]{0.0,0.1217,0.0}{{this}}}
{\color[rgb]{0.0,0.1203,0.0}{{or}}}
{\color[rgb]{0.0,0.1046,0.0}{{is}}}
{\color[rgb]{0.0,0.1002,0.0}{{it}}}
{\color[rgb]{0.0,0.097,0.0}{{that}}}
{\color[rgb]{0.0,0.1105,0.0}{{they}}}
{\color[rgb]{0.0,0.1384,0.0}{{usually}}}
{\color[rgb]{0.0,0.177,0.0}{{talk}}}
{\color[rgb]{0.0,0.231,0.0}{{to}}}
{\color[rgb]{0.0,0.2232,0.0}{{stars}}}
{\color[rgb]{0.0,0.2216,0.0}{{more}}}
{\color[rgb]{0.0,0.1736,0.0}{{than}}}
{\color[rgb]{0.0,0.1266,0.0}{{regular}}}
{\color[rgb]{0.0,0.0689,0.0}{{players}}}
{\color[rgb]{0.0,0.0528,0.0}{{which}}}
{\color[rgb]{0.0,0.0534,0.0}{{explains}}}
{\color[rgb]{0.0,0.0848,0.0}{{the}}}
{\color[rgb]{0.0,0.1002,0.0}\textit{{hight}}}
{\color[rgb]{0.0,0.1053,0.0}{{percentage}}}
{\color[rgb]{0.0,0.1344,0.0}{{of}}}
{\color[rgb]{0.0,0.13,0.0}{{results}}}
{\color[rgb]{0.0,0.1355,0.0}{{after}}}
{\color[rgb]{0.0,0.1469,0.0}{{.}}}
{\color[rgb]{0.0,0.1388,0.0}{{It}}}
{\color[rgb]{0.0,0.1267,0.0}{{was}}}
{\color[rgb]{0.0,0.1305,0.0}{{produced}}}
{\color[rgb]{0.0,0.1468,0.0}{{in}}}
{\color[rgb]{0.0,0.1171,0.0}{{collaboration}}}
{\color[rgb]{0.0,0.1109,0.0}{{with}}}
{\color[rgb]{0.0,0.102,0.0}{{the}}}
{\color[rgb]{0.0,0.0921,0.0}{{American}}}
{\color[rgb]{0.0,0.0629,0.0}{{College}}}
{\color[rgb]{0.0,0.0538,0.0}{{of}}}
{\color[rgb]{0.0,0.0276,0.0}\textit{{Surgeons}}}
{\color[rgb]{0.0,0.0191,0.0}{{Commission}}}
{\color[rgb]{0.0,0.0003,0.0}{{on}}}
{\color[rgb]{0.0238,0.0,0.0}{{Cancer}}}
{\color[rgb]{0.0179,0.0,0.0}{{.}}}

==> examples/QGRU_occlusion-3_2167.tex <==
{\color[rgb]{0.0,0.086,0.0}{{initially}}}
{\color[rgb]{0.0,0.109,0.0}{{a}}}
{\color[rgb]{0.0,0.097,0.0}{{pagan}}}
{\color[rgb]{0.0,0.003,0.0}{{culture}}}
{\color[rgb]{0.0,0.146,0.0}{{,}}}
{\color[rgb]{0.0,0.209,0.0}{{detailed}}}
{\color[rgb]{0.0,0.34,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.279,0.0}{{about}}}
{\color[rgb]{0.0,0.153,0.0}{{the}}}
{\color[rgb]{0.0,0.008,0.0}{{return}}}
{\color[rgb]{0.096,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.007,0.0}{{the}}}
{\color[rgb]{0.0,0.46,0.0}{{christian}}}
{\color[rgb]{0.0,0.87,0.0}{{religion}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{to}}}
{\color[rgb]{0.0,0.469,0.0}{{the}}}
{\color[rgb]{0.0,0.025,0.0}{{islands}}}
{\color[rgb]{0.0,0.098,0.0}{{during}}}
{\color[rgb]{0.0,0.12,0.0}{{the}}}
{\color[rgb]{0.0,0.164,0.0}{{NNP}}}


==> examples/QGRU_occlusion-7_2167.tex <==
{\color[rgb]{0.0,0.129,0.0}{{initially}}}
{\color[rgb]{0.0,0.178,0.0}{{a}}}
{\color[rgb]{0.0,0.253,0.0}{{pagan}}}
{\color[rgb]{0.0,0.374,0.0}{{culture}}}
{\color[rgb]{0.0,0.39,0.0}{{,}}}
{\color[rgb]{0.0,0.429,0.0}{{detailed}}}
{\color[rgb]{0.0,0.511,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.508,0.0}{{about}}}
{\color[rgb]{0.0,0.633,0.0}{{the}}}
{\color[rgb]{0.0,0.724,0.0}{{return}}}
{\color[rgb]{0.0,0.729,0.0}{{of}}}
{\color[rgb]{0.0,0.793,0.0}{{the}}}
{\color[rgb]{0.0,0.866,0.0}{{christian}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{religion}}}
{\color[rgb]{0.0,0.881,0.0}{{to}}}
{\color[rgb]{0.0,0.754,0.0}{{the}}}
{\color[rgb]{0.0,0.606,0.0}{{islands}}}
{\color[rgb]{0.0,0.53,0.0}{{during}}}
{\color[rgb]{0.0,0.454,0.0}{{the}}}
{\color[rgb]{0.0,0.346,0.0}{{NNP}}}


==> examples/QGRU_occlusion_2167.tex <==
{\color[rgb]{0.0,0.013,0.0}{{initially}}}
{\color[rgb]{0.0,0.045,0.0}{{a}}}
{\color[rgb]{0.0,0.017,0.0}{{pagan}}}
{\color[rgb]{0.037,0.0,0.0}{{culture}}}
{\color[rgb]{0.047,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.004,0.0}{{detailed}}}
{\color[rgb]{0.0,0.474,0.0}{\underline {information}}}
{\color[rgb]{0.014,0.0,0.0}{{about}}}
{\color[rgb]{0.0,0.007,0.0}{{the}}}
{\color[rgb]{0.0,0.039,0.0}{{return}}}
{\color[rgb]{0.097,0.0,0.0}{{of}}}
{\color[rgb]{0.008,0.0,0.0}{{the}}}
{\color[rgb]{0.053,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.24,0.0}{{religion}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{to}}}
{\color[rgb]{0.068,0.0,0.0}{{the}}}
{\color[rgb]{0.1,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.095,0.0}{{during}}}
{\color[rgb]{0.0,0.01,0.0}{{the}}}
{\color[rgb]{0.0,0.037,0.0}{{NNP}}}


==> examples/QGRU_omission-3_2167.tex <==
{\color[rgb]{0.017,0.0,0.0}{{initially}}}
{\color[rgb]{0.032,0.0,0.0}{{a}}}
{\color[rgb]{0.054,0.0,0.0}{{pagan}}}
{\color[rgb]{0.059,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.087,0.0}{{,}}}
{\color[rgb]{0.0,0.125,0.0}{{detailed}}}
{\color[rgb]{0.0,0.197,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.079,0.0}{{about}}}
{\color[rgb]{0.022,0.0,0.0}{{the}}}
{\color[rgb]{0.111,0.0,0.0}{{return}}}
{\color[rgb]{0.158,0.0,0.0}{{of}}}
{\color[rgb]{0.044,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.46,0.0}{{christian}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{religion}}}
{\color[rgb]{0.0,0.856,0.0}{{to}}}
{\color[rgb]{0.0,0.355,0.0}{{the}}}
{\color[rgb]{0.138,0.0,0.0}{{islands}}}
{\color[rgb]{0.062,0.0,0.0}{{during}}}
{\color[rgb]{0.004,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.085,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_omission-7_2167.tex <==
{\color[rgb]{0.0,0.159,0.0}{{initially}}}
{\color[rgb]{0.0,0.178,0.0}{{a}}}
{\color[rgb]{0.0,0.24,0.0}{{pagan}}}
{\color[rgb]{0.0,0.388,0.0}{{culture}}}
{\color[rgb]{0.0,0.341,0.0}{{,}}}
{\color[rgb]{0.0,0.329,0.0}{{detailed}}}
{\color[rgb]{0.0,0.348,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.22,0.0}{{about}}}
{\color[rgb]{0.0,0.623,0.0}{{the}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{return}}}
{\color[rgb]{0.0,0.784,0.0}{{of}}}
{\color[rgb]{0.0,0.834,0.0}{{the}}}
{\color[rgb]{0.0,0.813,0.0}{{christian}}}
{\color[rgb]{0.0,0.718,0.0}{{religion}}}
{\color[rgb]{0.0,0.584,0.0}{{to}}}
{\color[rgb]{0.0,0.074,0.0}{{the}}}
{\color[rgb]{0.349,0.0,0.0}{{islands}}}
{\color[rgb]{0.324,0.0,0.0}{{during}}}
{\color[rgb]{0.309,0.0,0.0}{{the}}}
{\color[rgb]{0.265,0.0,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_omission_2167.tex <==
{\color[rgb]{0.137,0.0,0.0}{{initially}}}
{\color[rgb]{0.003,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.007,0.0}{{pagan}}}
{\color[rgb]{0.049,0.0,0.0}{{culture}}}
{\color[rgb]{0.058,0.0,0.0}{{,}}}
{\color[rgb]{0.008,0.0,0.0}{{detailed}}}
{\color[rgb]{0.0,0.304,0.0}{\underline{information}}}
{\color[rgb]{0.1,0.0,0.0}{{about}}}
{\color[rgb]{0.0,0.001,0.0}{{the}}}
{\color[rgb]{0.0,0.015,0.0}{{return}}}
{\color[rgb]{0.107,0.0,0.0}{{of}}}
{\color[rgb]{0.008,0.0,0.0}{{the}}}
{\color[rgb]{0.058,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.147,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.108,0.0,0.0}{{the}}}
{\color[rgb]{0.23,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.167,0.0}{{during}}}
{\color[rgb]{0.0,0.02,0.0}{{the}}}
{\color[rgb]{0.0,0.038,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_omission_233.tex <==
{\color[rgb]{0.0,0.196,0.0}{{the}}}
{\color[rgb]{0.0,0.046,0.0}{{most}}}
{\color[rgb]{0.242,0.0,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.811,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.005,0.0}{{the}}}
{\color[rgb]{0.0,0.045,0.0}{{village}}}


==> examples/QGRU_omission_970.tex <==
{\color[rgb]{0.139,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.065,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.489,0.0}{{in}}}
{\color[rgb]{0.008,0.0,0.0}{{the}}}
{\color[rgb]{0.023,0.0,0.0}{{series}}}


==> examples/QGRU_salience_prob_2167.tex <==
{\color[rgb]{0.0,0.035,0.0}{{initially}}}
{\color[rgb]{0.0,0.002,0.0}{{a}}}
{\color[rgb]{0.0,0.005,0.0}{{pagan}}}
{\color[rgb]{0.061,0.0,0.0}{{culture}}}
{\color[rgb]{0.075,0.0,0.0}{{,}}}
{\color[rgb]{0.063,0.0,0.0}{{detailed}}}
{\color[rgb]{0.0,0.41,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.107,0.0}{{about}}}
{\color[rgb]{0.0,0.018,0.0}{{the}}}
{\color[rgb]{0.0,0.03,0.0}{{return}}}
{\color[rgb]{0.057,0.0,0.0}{{of}}}
{\color[rgb]{0.018,0.0,0.0}{{the}}}
{\color[rgb]{0.168,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.141,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.135,0.0,0.0}{{the}}}
{\color[rgb]{0.179,0.0,0.0}{{islands}}}
{\color[rgb]{0.145,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.023,0.0}{{the}}}
{\color[rgb]{0.0,0.04,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_salience_prob_233.tex <==
{\color[rgb]{0.0,0.173,0.0}{{the}}}
{\color[rgb]{0.0,0.104,0.0}{{most}}}
{\color[rgb]{0.0,0.169,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.047,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.138,0.0}{{the}}}
{\color[rgb]{0.0,0.209,0.0}{{village}}}


==> examples/QGRU_salience_prob_970.tex <==
{\color[rgb]{0.293,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.013,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.71,0.0}{{in}}}
{\color[rgb]{0.12,0.0,0.0}{{the}}}
{\color[rgb]{0.064,0.0,0.0}{{series}}}


==> examples/QGRU_salience_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.142,0.0}{{initially}}}
{\color[rgb]{0.0,0.151,0.0}{{a}}}
{\color[rgb]{0.0,0.116,0.0}{{pagan}}}
{\color[rgb]{0.0,0.137,0.0}{{culture}}}
{\color[rgb]{0.0,0.081,0.0}{{,}}}
{\color[rgb]{0.0,0.066,0.0}{{detailed}}}
{\color[rgb]{0.0,0.444,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.126,0.0}{{about}}}
{\color[rgb]{0.0,0.056,0.0}{{the}}}
{\color[rgb]{0.0,0.146,0.0}{{return}}}
{\color[rgb]{0.0,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.055,0.0}{{the}}}
{\color[rgb]{0.0,0.054,0.0}{{christian}}}
{\color[rgb]{0.0,0.424,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.017,0.0}{{the}}}
{\color[rgb]{0.491,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.153,0.0}{{during}}}
{\color[rgb]{0.0,0.059,0.0}{{the}}}
{\color[rgb]{0.0,0.169,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_salience_prob_integrated_233.tex <==
{\color[rgb]{0.0,0.18,0.0}{{the}}}
{\color[rgb]{0.0,0.151,0.0}{{most}}}
{\color[rgb]{0.277,0.0,0.0}{{recent}}}
{\color[rgb]{0.0,0.798,0.0}{\underline{addition}}}
{\color[rgb]{0.173,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.39,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}{{village}}}


==> examples/QGRU_salience_prob_integrated_970.tex <==
{\color[rgb]{0.246,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.016,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.097,0.0}{{in}}}
{\color[rgb]{0.304,0.0,0.0}{{the}}}
{\color[rgb]{0.178,0.0,0.0}{{series}}}


==> examples/QGRU_salience_raw_2167.tex <==
{\color[rgb]{0.0,0.027,0.0}{{initially}}}
{\color[rgb]{0.0,0.007,0.0}{{a}}}
{\color[rgb]{0.0,0.008,0.0}{{pagan}}}
{\color[rgb]{0.067,0.0,0.0}{{culture}}}
{\color[rgb]{0.066,0.0,0.0}{{,}}}
{\color[rgb]{0.051,0.0,0.0}{{detailed}}}
{\color[rgb]{0.0,0.407,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.088,0.0}{{about}}}
{\color[rgb]{0.0,0.008,0.0}{{the}}}
{\color[rgb]{0.0,0.034,0.0}{{return}}}
{\color[rgb]{0.083,0.0,0.0}{{of}}}
{\color[rgb]{0.017,0.0,0.0}{{the}}}
{\color[rgb]{0.182,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.207,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.141,0.0,0.0}{{the}}}
{\color[rgb]{0.225,0.0,0.0}{{islands}}}
{\color[rgb]{0.139,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.025,0.0}{{the}}}
{\color[rgb]{0.0,0.041,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_salience_raw_233.tex <==
{\color[rgb]{0.0,0.207,0.0}{{the}}}
{\color[rgb]{0.0,0.114,0.0}{{most}}}
{\color[rgb]{0.0,0.171,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.099,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.082,0.0}{{the}}}
{\color[rgb]{0.0,0.169,0.0}{{village}}}


==> examples/QGRU_salience_raw_970.tex <==
{\color[rgb]{0.354,0.0,0.0}{{the}}}
{\color[rgb]{0.031,0.0,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.743,0.0}{{in}}}
{\color[rgb]{0.165,0.0,0.0}{{the}}}
{\color[rgb]{0.067,0.0,0.0}{{series}}}


==> examples/QGRU_salience_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.058,0.0}{{initially}}}
{\color[rgb]{0.0,0.096,0.0}{{a}}}
{\color[rgb]{0.0,0.078,0.0}{{pagan}}}
{\color[rgb]{0.0,0.037,0.0}{{culture}}}
{\color[rgb]{0.007,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.026,0.0}{{detailed}}}
{\color[rgb]{0.0,0.481,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.08,0.0}{{about}}}
{\color[rgb]{0.0,0.046,0.0}{{the}}}
{\color[rgb]{0.0,0.099,0.0}{{return}}}
{\color[rgb]{0.027,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.022,0.0}{{the}}}
{\color[rgb]{0.022,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.341,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.051,0.0,0.0}{{the}}}
{\color[rgb]{0.407,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.008,0.0}{{during}}}
{\color[rgb]{0.0,0.063,0.0}{{the}}}
{\color[rgb]{0.0,0.135,0.0}{{\textit{norse-era}}}}


==> examples/QGRU_salience_raw_integrated_233.tex <==
{\color[rgb]{0.0,0.218,0.0}{{the}}}
{\color[rgb]{0.0,0.152,0.0}{{most}}}
{\color[rgb]{0.149,0.0,0.0}{{recent}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{addition}}}
{\color[rgb]{0.176,0.0,0.0}{{to}}}
{\color[rgb]{0.0,0.284,0.0}{{the}}}
{\color[rgb]{0.0,0.697,0.0}{{village}}}


==> examples/QGRU_salience_raw_integrated_970.tex <==
{\color[rgb]{0.255,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.016,0.0}{{other}}}
{\color[rgb]{0.0,0.909,0.0}{\underline{books}}}
{\color[rgb]{0.0,0.408,0.0}{{in}}}
{\color[rgb]{0.296,0.0,0.0}{{the}}}
{\color[rgb]{0.178,0.0,0.0}{{series}}}


==> examples/QLSTM_deeplift_2167.tex <==
{\color[rgb]{0.0,0.049,0.0}{{initially}}}
{\color[rgb]{0.0,0.059,0.0}{{a}}}
{\color[rgb]{0.0,0.058,0.0}{{pagan}}}
{\color[rgb]{0.017,0.0,0.0}{{culture}}}
{\color[rgb]{0.07,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.164,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.019,0.0}{{about}}}
{\color[rgb]{0.0,0.152,0.0}{{the}}}
{\color[rgb]{0.0,0.4,0.0}{{return}}}
{\color[rgb]{0.0,0.032,0.0}{{of}}}
{\color[rgb]{0.0,0.012,0.0}{{the}}}
{\color[rgb]{0.038,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.416,0.0}{{religion}}}
{\color[rgb]{0.0,0.034,0.0}{{to}}}
{\color[rgb]{0.0,0.025,0.0}{{the}}}
{\color[rgb]{0.09,0.0,0.0}{{islands}}}
{\color[rgb]{0.012,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.003,0.0}{{the}}}
{\color[rgb]{0.0,0.011,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_gamma_2167.tex <==
{\color[rgb]{0.0,0.056,0.0}{{initially}}}
{\color[rgb]{0.0,0.074,0.0}{{a}}}
{\color[rgb]{0.0,0.195,0.0}{{pagan}}}
{\color[rgb]{0.0,0.046,0.0}{{culture}}}
{\color[rgb]{0.0,0.006,0.0}{{,}}}
{\color[rgb]{0.0,0.243,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.112,0.0}{{about}}}
{\color[rgb]{0.0,0.159,0.0}{{the}}}
{\color[rgb]{0.0,0.387,0.0}{{return}}}
{\color[rgb]{0.0,0.033,0.0}{{of}}}
{\color[rgb]{0.0,0.007,0.0}{{the}}}
{\color[rgb]{0.0,0.025,0.0}{{christian}}}
{\color[rgb]{0.0,0.41,0.0}{{religion}}}
{\color[rgb]{0.0,0.001,0.0}{{to}}}
{\color[rgb]{0.0,0.004,0.0}{{the}}}
{\color[rgb]{0.089,0.0,0.0}{{islands}}}
{\color[rgb]{0.021,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.002,0.0}{{the}}}
{\color[rgb]{0.0,0.007,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_l2_prob_2167.tex <==
{\color[rgb]{0.0,0.376,0.0}{{initially}}}
{\color[rgb]{0.0,0.438,0.0}{{a}}}
{\color[rgb]{0.0,0.532,0.0}{{pagan}}}
{\color[rgb]{0.0,0.423,0.0}{{culture}}}
{\color[rgb]{0.0,0.474,0.0}{{,}}}
{\color[rgb]{0.0,0.515,0.0}{{detailed}}}
{\color[rgb]{0.0,0.494,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.687,0.0}{{about}}}
{\color[rgb]{0.0,0.446,0.0}{{the}}}
{\color[rgb]{0.0,0.348,0.0}{{return}}}
{\color[rgb]{0.0,0.262,0.0}{{of}}}
{\color[rgb]{0.0,0.343,0.0}{{the}}}
{\color[rgb]{0.0,0.485,0.0}{{christian}}}
{\color[rgb]{0.0,0.382,0.0}{{religion}}}
{\color[rgb]{0.0,0.37,0.0}{{to}}}
{\color[rgb]{0.0,0.681,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{islands}}}
{\color[rgb]{0.0,0.408,0.0}{{during}}}
{\color[rgb]{0.0,0.458,0.0}{{the}}}
{\color[rgb]{0.0,0.49,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_l2_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.181,0.0}{{initially}}}
{\color[rgb]{0.0,0.206,0.0}{{a}}}
{\color[rgb]{0.0,0.241,0.0}{{pagan}}}
{\color[rgb]{0.0,0.255,0.0}{{culture}}}
{\color[rgb]{0.0,0.321,0.0}{{,}}}
{\color[rgb]{0.0,0.347,0.0}{{detailed}}}
{\color[rgb]{0.0,0.365,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.421,0.0}{{about}}}
{\color[rgb]{0.0,0.373,0.0}{{the}}}
{\color[rgb]{0.0,0.411,0.0}{{return}}}
{\color[rgb]{0.0,0.407,0.0}{{of}}}
{\color[rgb]{0.0,0.395,0.0}{{the}}}
{\color[rgb]{0.0,0.487,0.0}{{christian}}}
{\color[rgb]{0.0,0.598,0.0}{{religion}}}
{\color[rgb]{0.0,0.597,0.0}{{to}}}
{\color[rgb]{0.0,0.661,0.0}{{the}}}
{\color[rgb]{0.0,0.661,0.0}{{islands}}}
{\color[rgb]{0.0,0.583,0.0}{{during}}}
{\color[rgb]{0.0,0.677,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{\textit{norse-era}}}}


==> examples/QLSTM_l2_raw_2167.tex <==
{\color[rgb]{0.0,0.317,0.0}{{initially}}}
{\color[rgb]{0.0,0.36,0.0}{{a}}}
{\color[rgb]{0.0,0.427,0.0}{{pagan}}}
{\color[rgb]{0.0,0.366,0.0}{{culture}}}
{\color[rgb]{0.0,0.405,0.0}{{,}}}
{\color[rgb]{0.0,0.444,0.0}{{detailed}}}
{\color[rgb]{0.0,0.426,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.591,0.0}{{about}}}
{\color[rgb]{0.0,0.364,0.0}{{the}}}
{\color[rgb]{0.0,0.313,0.0}{{return}}}
{\color[rgb]{0.0,0.259,0.0}{{of}}}
{\color[rgb]{0.0,0.335,0.0}{{the}}}
{\color[rgb]{0.0,0.497,0.0}{{christian}}}
{\color[rgb]{0.0,0.388,0.0}{{religion}}}
{\color[rgb]{0.0,0.372,0.0}{{to}}}
{\color[rgb]{0.0,0.668,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{islands}}}
{\color[rgb]{0.0,0.355,0.0}{{during}}}
{\color[rgb]{0.0,0.406,0.0}{{the}}}
{\color[rgb]{0.0,0.435,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_l2_raw_integrated_2167.tex <==
{\color[rgb]{0.0,0.218,0.0}{{initially}}}
{\color[rgb]{0.0,0.206,0.0}{{a}}}
{\color[rgb]{0.0,0.276,0.0}{{pagan}}}
{\color[rgb]{0.0,0.307,0.0}{{culture}}}
{\color[rgb]{0.0,0.367,0.0}{{,}}}
{\color[rgb]{0.0,0.413,0.0}{{detailed}}}
{\color[rgb]{0.0,0.371,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.6,0.0}{{about}}}
{\color[rgb]{0.0,0.354,0.0}{{the}}}
{\color[rgb]{0.0,0.379,0.0}{{return}}}
{\color[rgb]{0.0,0.296,0.0}{{of}}}
{\color[rgb]{0.0,0.331,0.0}{{the}}}
{\color[rgb]{0.0,0.467,0.0}{{christian}}}
{\color[rgb]{0.0,0.597,0.0}{{religion}}}
{\color[rgb]{0.0,0.607,0.0}{{to}}}
{\color[rgb]{0.0,0.743,0.0}{{the}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{islands}}}
{\color[rgb]{0.0,0.59,0.0}{{during}}}
{\color[rgb]{0.0,0.653,0.0}{{the}}}
{\color[rgb]{0.0,0.888,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_lime_class_2167.tex <==
{\color[rgb]{0.0,0.361,0.0}{{initially}}}
{\color[rgb]{0.0,0.111,0.0}{{a}}}
{\color[rgb]{0.0,0.389,0.0}{{pagan}}}
{\color[rgb]{0.0,0.673,0.0}{{culture}}}
{\color[rgb]{0.0,0.782,0.0}{{,}}}
{\color[rgb]{0.0,0.268,0.0}{{detailed}}}
{\color[rgb]{0.0,0.42,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{about}}}
{\color[rgb]{0.0,0.393,0.0}{{the}}}
{\color[rgb]{0.0,0.377,0.0}{{return}}}
{\color[rgb]{0.0,0.465,0.0}{{of}}}
{\color[rgb]{0.0,0.388,0.0}{{the}}}
{\color[rgb]{0.0,0.451,0.0}{{christian}}}
{\color[rgb]{0.0,0.742,0.0}{{religion}}}
{\color[rgb]{0.0,0.284,0.0}{{to}}}
{\color[rgb]{0.0,0.169,0.0}{{the}}}
{\color[rgb]{0.386,0.0,0.0}{{islands}}}
{\color[rgb]{0.225,0.0,0.0}{{during}}}
{\color[rgb]{0.282,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.207,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_lime_prob_2167.tex <==
{\color[rgb]{0.0,0.671,0.0}{{initially}}}
{\color[rgb]{0.0,0.358,0.0}{{a}}}
{\color[rgb]{0.0,0.581,0.0}{{pagan}}}
{\color[rgb]{0.0,0.577,0.0}{{culture}}}
{\color[rgb]{0.0,0.578,0.0}{{,}}}
{\color[rgb]{0.0,0.222,0.0}{{detailed}}}
{\color[rgb]{0.0,0.436,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.615,0.0}{{about}}}
{\color[rgb]{0.0,0.35,0.0}{{the}}}
{\color[rgb]{0.0,0.585,0.0}{{return}}}
{\color[rgb]{0.0,0.359,0.0}{{of}}}
{\color[rgb]{0.0,0.278,0.0}{{the}}}
{\color[rgb]{0.0,0.415,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.462,0.0}{{to}}}
{\color[rgb]{0.0,0.432,0.0}{{the}}}
{\color[rgb]{0.203,0.0,0.0}{{islands}}}
{\color[rgb]{0.014,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.126,0.0}{{the}}}
{\color[rgb]{0.0,0.571,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_lime_raw_2167.tex <==
{\color[rgb]{0.0,0.671,0.0}{{initially}}}
{\color[rgb]{0.0,0.358,0.0}{{a}}}
{\color[rgb]{0.0,0.581,0.0}{{pagan}}}
{\color[rgb]{0.0,0.577,0.0}{{culture}}}
{\color[rgb]{0.0,0.578,0.0}{{,}}}
{\color[rgb]{0.0,0.222,0.0}{{detailed}}}
{\color[rgb]{0.0,0.436,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.615,0.0}{{about}}}
{\color[rgb]{0.0,0.35,0.0}{{the}}}
{\color[rgb]{0.0,0.585,0.0}{{return}}}
{\color[rgb]{0.0,0.359,0.0}{{of}}}
{\color[rgb]{0.0,0.278,0.0}{{the}}}
{\color[rgb]{0.0,0.415,0.0}{{christian}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{religion}}}
{\color[rgb]{0.0,0.462,0.0}{{to}}}
{\color[rgb]{0.0,0.432,0.0}{{the}}}
{\color[rgb]{0.203,0.0,0.0}{{islands}}}
{\color[rgb]{0.014,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.126,0.0}{{the}}}
{\color[rgb]{0.0,0.571,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_lrp_2167.tex <==
{\color[rgb]{0.0,0.048,0.0}{{initially}}}
{\color[rgb]{0.0,0.065,0.0}{{a}}}
{\color[rgb]{0.0,0.069,0.0}{{pagan}}}
{\color[rgb]{0.026,0.0,0.0}{{culture}}}
{\color[rgb]{0.078,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.178,0.0}{{detailed}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{\underline{information}}}
{\color[rgb]{0.0,0.013,0.0}{{about}}}
{\color[rgb]{0.0,0.16,0.0}{{the}}}
{\color[rgb]{0.0,0.379,0.0}{{return}}}
{\color[rgb]{0.0,0.032,0.0}{{of}}}
{\color[rgb]{0.0,0.009,0.0}{{the}}}
{\color[rgb]{0.037,0.0,0.0}{{christian}}}
{\color[rgb]{0.0,0.4,0.0}{{religion}}}
{\color[rgb]{0.0,0.028,0.0}{{to}}}
{\color[rgb]{0.0,0.023,0.0}{{the}}}
{\color[rgb]{0.084,0.0,0.0}{{islands}}}
{\color[rgb]{0.011,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.002,0.0}{{the}}}
{\color[rgb]{0.0,0.011,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_newsgroup_omission-5_3313.tex <==
{\color[rgb]{0.0,0.0148,0.0}{{Sorry}}}
{\color[rgb]{0.0,0.0145,0.0}{{for}}}
{\color[rgb]{0.0,0.0058,0.0}{{any}}}
{\color[rgb]{0.0,0.0229,0.0}{{confusion}}}
{\color[rgb]{0.0,0.0394,0.0}{{I}}}
{\color[rgb]{0.0,0.0768,0.0}{{may}}}
{\color[rgb]{0.0,0.1378,0.0}{{have}}}
{\color[rgb]{0.0,0.2049,0.0}{{created}}}
{\color[rgb]{0.0,0.2684,0.0}{{.}}}
{\color[rgb]{0.0,0.3353,0.0}{{Jon}}}
{\color[rgb]{0.0,0.3392,0.0}{{Mandaville}}}
{\color[rgb]{0.0,0.3138,0.0}{{,}}}
{\color[rgb]{0.0,0.2861,0.0}{{Professor}}}
{\color[rgb]{0.0,0.1989,0.0}{{of}}}
{\color[rgb]{0.0,0.1048,0.0}{{History}}}
{\color[rgb]{0.0,0.0345,0.0}{{,}}}
{\color[rgb]{0.0003,0.0,0.0}{{Portland}}}
{\color[rgb]{0.0364,0.0,0.0}{{State}}}
{\color[rgb]{0.0241,0.0,0.0}{{University}}}
{\color[rgb]{0.0084,0.0,0.0}{{(}}}
{\color[rgb]{0.0,0.0144,0.0}{{Oregon}}}
{\color[rgb]{0.0,0.0234,0.0}{{)}}}
{\color[rgb]{0.0,0.0378,0.0}{{.}}}
{\color[rgb]{0.0,0.049,0.0}{{Trying}}}
{\color[rgb]{0.0,0.0503,0.0}{{to}}}
{\color[rgb]{0.0,0.0538,0.0}{{mix}}}
{\color[rgb]{0.0,0.0625,0.0}{{up}}}
{\color[rgb]{0.0,0.0468,0.0}{{the}}}
{\color[rgb]{0.0,0.0186,0.0}{{lines}}}
{\color[rgb]{0.0,0.006,0.0}{{is}}}
{\color[rgb]{0.0186,0.0,0.0}{{a}}}
{\color[rgb]{0.0655,0.0,0.0}{{dead}}}
{\color[rgb]{0.0914,0.0,0.0}{{end}}}
{\color[rgb]{0.1121,0.0,0.0}{{.}}}
{\color[rgb]{0.1238,0.0,0.0}{{matter}}}
{\color[rgb]{0.1326,0.0,0.0}{{of}}}
{\color[rgb]{0.1251,0.0,0.0}{{proving}}}
{\color[rgb]{0.1128,0.0,0.0}{{the}}}
{\color[rgb]{0.105,0.0,0.0}{{track}}}
{\color[rgb]{0.0946,0.0,0.0}{{record}}}
{\color[rgb]{0.0779,0.0,0.0}{{of}}}
{\color[rgb]{0.0532,0.0,0.0}{{the}}}
{\color[rgb]{0.0285,0.0,0.0}{{\#}}}
{\color[rgb]{0.0,0.0006,0.0}{{scientific}}}
{\color[rgb]{0.0,0.0195,0.0}{{method}}}
{\color[rgb]{0.0,0.0311,0.0}{{.}}}
{\color[rgb]{0.0,0.021,0.0}{{--}}}
{\color[rgb]{0.0,0.0227,0.0}{{I}}}
{\color[rgb]{0.0,0.0154,0.0}{{know}}}
{\color[rgb]{0.0,0.0127,0.0}{{that}}}
{\color[rgb]{0.0,0.0258,0.0}{{I}}}
{\color[rgb]{0.0,0.024,0.0}{{will}}}
{\color[rgb]{0.0,0.0126,0.0}{{have}}}
{\color[rgb]{0.0,0.0275,0.0}{{to}}}
{\color[rgb]{0.0,0.0042,0.0}{{pay}}}
{\color[rgb]{0.0265,0.0,0.0}{{tax}}}
{\color[rgb]{0.0218,0.0,0.0}{{when}}}
{\color[rgb]{0.0135,0.0,0.0}{{I}}}
{\color[rgb]{0.033,0.0,0.0}{{go}}}
{\color[rgb]{0.0267,0.0,0.0}{{to}}}
{\color[rgb]{0.0136,0.0,0.0}{{register}}}
{\color[rgb]{0.0095,0.0,0.0}{{the}}}
{\color[rgb]{0.0144,0.0,0.0}{{car}}}
{\color[rgb]{0.0273,0.0,0.0}{{.}}}
{\color[rgb]{0.0391,0.0,0.0}{{It}}}
{\color[rgb]{0.0543,0.0,0.0}{{sounds}}}
{\color[rgb]{0.0713,0.0,0.0}{{like}}}
{\color[rgb]{0.059,0.0,0.0}{{he}}}
{\color[rgb]{0.0345,0.0,0.0}{{has}}}
{\color[rgb]{0.005,0.0,0.0}{{had}}}
{\color[rgb]{0.0,0.0207,0.0}{{another}}}
{\color[rgb]{0.0,0.0488,0.0}{{set}}}
{\color[rgb]{0.0,0.0401,0.0}{{back}}}
{\color[rgb]{0.0,0.036,0.0}{{in}}}
{\color[rgb]{0.0,0.0239,0.0}{{his}}}
{\color[rgb]{0.0,0.0044,0.0}{{come}}}
{\color[rgb]{0.0116,0.0,0.0}{{back}}}
{\color[rgb]{0.0081,0.0,0.0}{{.}}}
{\color[rgb]{0.0,0.0051,0.0}{{Oh}}}
{\color[rgb]{0.0,0.0434,0.0}{{,}}}
{\color[rgb]{0.0,0.0593,0.0}{{and}}}
{\color[rgb]{0.0,0.0116,0.0}{{a}}}
{\color[rgb]{0.0721,0.0,0.0}{{prediction}}}
{\color[rgb]{0.1477,0.0,0.0}{{:}}}
{\color[rgb]{0.061,0.0,0.0}{{Milt}}}
{\color[rgb]{0.0,0.1013,0.0}{{Cuyler}}}
{\color[rgb]{0.0,0.3184,0.0}{{.}}}
{\color[rgb]{0.0,0.6142,0.0}{\underline {The}}}
{\color[rgb]{0.0,0.9091,0.0}\textbf{\underline {Xaw}}}
{\color[rgb]{0.0,0.9036,0.0}{\underline {support}}}
{\color[rgb]{0.0,0.7671,0.0}{\underline {was}}}
{\color[rgb]{0.0,0.6693,0.0}{\underline {missing}}}
{\color[rgb]{0.0,0.5036,0.0}{\underline {from}}}
{\color[rgb]{0.0,0.3404,0.0}\textit{\underline {OW2.0}}}
{\color[rgb]{0.0,0.2718,0.0}{\underline {but}}}
{\color[rgb]{0.0,0.2986,0.0}{\underline {added}}}
{\color[rgb]{0.0,0.2849,0.0}{\underline {in}}}
{\color[rgb]{0.0,0.284,0.0}{\underline {3.0}}}
{\color[rgb]{0.0,0.2461,0.0}{\underline {.}}}
{\color[rgb]{0.0,0.2537,0.0}{{This}}}
{\color[rgb]{0.0,0.2286,0.0}{{slant}}}
{\color[rgb]{0.0,0.1752,0.0}\textit{{permeates}}}
{\color[rgb]{0.0,0.1245,0.0}{{the}}}
{\color[rgb]{0.0,0.0926,0.0}{{text}}}
{\color[rgb]{0.0,0.0368,0.0}{{.}}}

==> examples/QLSTM_occlusion-3_2167.tex <==
{\color[rgb]{0.0,0.011,0.0}{{initially}}}
{\color[rgb]{0.0,0.02,0.0}{{a}}}
{\color[rgb]{0.0,0.018,0.0}{{pagan}}}
{\color[rgb]{0.0,0.064,0.0}{{culture}}}
{\color[rgb]{0.0,0.333,0.0}{{,}}}
{\color[rgb]{0.0,0.495,0.0}{{detailed}}}
{\color[rgb]{0.0,0.696,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.759,0.0}{{about}}}
{\color[rgb]{0.0,0.535,0.0}{{the}}}
{\color[rgb]{0.0,0.245,0.0}{{return}}}
{\color[rgb]{0.024,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.075,0.0}{{the}}}
{\color[rgb]{0.0,0.416,0.0}{{christian}}}
{\color[rgb]{0.0,0.723,0.0}{{religion}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{to}}}
{\color[rgb]{0.0,0.502,0.0}{{the}}}
{\color[rgb]{0.0,0.209,0.0}{{islands}}}
{\color[rgb]{0.0,0.163,0.0}{{during}}}
{\color[rgb]{0.0,0.355,0.0}{{the}}}
{\color[rgb]{0.0,0.319,0.0}{{NNP}}}


==> examples/QLSTM_occlusion-7_2167.tex <==
{\color[rgb]{0.0,0.14,0.0}{{initially}}}
{\color[rgb]{0.0,0.197,0.0}{{a}}}
{\color[rgb]{0.0,0.273,0.0}{{pagan}}}
{\color[rgb]{0.0,0.403,0.0}{{culture}}}
{\color[rgb]{0.0,0.426,0.0}{{,}}}
{\color[rgb]{0.0,0.48,0.0}{{detailed}}}
{\color[rgb]{0.0,0.596,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.625,0.0}{{about}}}
{\color[rgb]{0.0,0.747,0.0}{{the}}}
{\color[rgb]{0.0,0.867,0.0}{{return}}}
{\color[rgb]{0.0,0.866,0.0}{{of}}}
{\color[rgb]{0.0,0.867,0.0}{{the}}}
{\color[rgb]{0.0,0.907,0.0}{{christian}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{religion}}}
{\color[rgb]{0.0,0.866,0.0}{{to}}}
{\color[rgb]{0.0,0.747,0.0}{{the}}}
{\color[rgb]{0.0,0.614,0.0}{{islands}}}
{\color[rgb]{0.0,0.533,0.0}{{during}}}
{\color[rgb]{0.0,0.537,0.0}{{the}}}
{\color[rgb]{0.0,0.456,0.0}{{NNP}}}


==> examples/QLSTM_occlusion_2167.tex <==
{\color[rgb]{0.094,0.0,0.0}{{initially}}}
{\color[rgb]{0.04,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.019,0.0}{{pagan}}}
{\color[rgb]{0.011,0.0,0.0}{{culture}}}
{\color[rgb]{0.014,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.155,0.0}{{detailed}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.229,0.0}{{about}}}
{\color[rgb]{0.0,0.184,0.0}{{the}}}
{\color[rgb]{0.0,0.125,0.0}{{return}}}
{\color[rgb]{0.123,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.007,0.0}{{the}}}
{\color[rgb]{0.0,0.058,0.0}{{christian}}}
{\color[rgb]{0.0,0.221,0.0}{{religion}}}
{\color[rgb]{0.0,0.899,0.0}{{to}}}
{\color[rgb]{0.0,0.008,0.0}{{the}}}
{\color[rgb]{0.121,0.0,0.0}{{islands}}}
{\color[rgb]{0.262,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.152,0.0}{{the}}}
{\color[rgb]{0.0,0.157,0.0}{{NNP}}}


==> examples/QLSTM_omission-3_2167.tex <==
{\color[rgb]{0.044,0.0,0.0}{{initially}}}
{\color[rgb]{0.063,0.0,0.0}{{a}}}
{\color[rgb]{0.075,0.0,0.0}{{pagan}}}
{\color[rgb]{0.0,0.0,0.0}{{culture}}}
{\color[rgb]{0.0,0.344,0.0}{{,}}}
{\color[rgb]{0.0,0.448,0.0}{{detailed}}}
{\color[rgb]{0.0,0.523,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.101,0.0}{{about}}}
{\color[rgb]{0.187,0.0,0.0}{{the}}}
{\color[rgb]{0.386,0.0,0.0}{{return}}}
{\color[rgb]{0.345,0.0,0.0}{{of}}}
{\color[rgb]{0.185,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.399,0.0}{{christian}}}
\textbf{\color[rgb]{0.0,0.909,0.0}{{religion}}}
{\color[rgb]{0.0,0.673,0.0}{{to}}}
{\color[rgb]{0.27,0.0,0.0}{{the}}}
{\color[rgb]{0.797,0.0,0.0}{{islands}}}
{\color[rgb]{0.609,0.0,0.0}{{during}}}
{\color[rgb]{0.148,0.0,0.0}{{the}}}
{\color[rgb]{0.028,0.0,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_omission-7_2167.tex <==
{\color[rgb]{0.0,0.279,0.0}{{initially}}}
{\color[rgb]{0.0,0.346,0.0}{{a}}}
{\color[rgb]{0.0,0.463,0.0}{{pagan}}}
{\color[rgb]{0.0,0.641,0.0}{{culture}}}
{\color[rgb]{0.0,0.605,0.0}{{,}}}
{\color[rgb]{0.0,0.628,0.0}{{detailed}}}
\textbf{\color[rgb]{0.0,0.699,0.0}{\underline {information}}}
{\color[rgb]{0.0,0.347,0.0}{{about}}}
{\color[rgb]{0.0,0.483,0.0}{{the}}}
{\color[rgb]{0.0,0.598,0.0}{{return}}}
{\color[rgb]{0.0,0.366,0.0}{{of}}}
{\color[rgb]{0.0,0.253,0.0}{{the}}}
{\color[rgb]{0.0,0.179,0.0}{{christian}}}
{\color[rgb]{0.025,0.0,0.0}{{religion}}}
{\color[rgb]{0.159,0.0,0.0}{{to}}}
{\color[rgb]{0.567,0.0,0.0}{{the}}}
{\color[rgb]{0.909,0.0,0.0}{{islands}}}
{\color[rgb]{0.889,0.0,0.0}{{during}}}
{\color[rgb]{0.736,0.0,0.0}{{the}}}
{\color[rgb]{0.667,0.0,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_omission_2167.tex <==
{\color[rgb]{0.15,0.0,0.0}{{initially}}}
{\color[rgb]{0.062,0.0,0.0}{{a}}}
{\color[rgb]{0.0,0.044,0.0}{{pagan}}}
{\color[rgb]{0.036,0.0,0.0}{{culture}}}
{\color[rgb]{0.05,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.111,0.0}{{detailed}}}
{\color[rgb]{0.0,0.573,0.0}{\underline{information}}}
{\color[rgb]{0.131,0.0,0.0}{{about}}}
{\color[rgb]{0.0,0.02,0.0}{{the}}}
{\color[rgb]{0.0,0.052,0.0}{{return}}}
{\color[rgb]{0.209,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.005,0.0}{{the}}}
{\color[rgb]{0.0,0.03,0.0}{{christian}}}
{\color[rgb]{0.0,0.032,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.169,0.0,0.0}{{the}}}
{\color[rgb]{0.42,0.0,0.0}{{islands}}}
{\color[rgb]{0.3,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.188,0.0}{{the}}}
{\color[rgb]{0.0,0.084,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_salience_prob_2167.tex <==
{\color[rgb]{0.394,0.0,0.0}{{initially}}}
{\color[rgb]{0.248,0.0,0.0}{{a}}}
{\color[rgb]{0.178,0.0,0.0}{{pagan}}}
{\color[rgb]{0.279,0.0,0.0}{{culture}}}
{\color[rgb]{0.128,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.217,0.0}{{detailed}}}
{\color[rgb]{0.0,0.726,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.489,0.0}{{about}}}
{\color[rgb]{0.0,0.45,0.0}{{the}}}
{\color[rgb]{0.051,0.0,0.0}{{return}}}
{\color[rgb]{0.334,0.0,0.0}{{of}}}
{\color[rgb]{0.001,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.099,0.0}{{christian}}}
{\color[rgb]{0.0,0.099,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.047,0.0,0.0}{{the}}}
{\color[rgb]{0.534,0.0,0.0}{{islands}}}
{\color[rgb]{0.016,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.519,0.0}{{the}}}
{\color[rgb]{0.0,0.441,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_salience_prob_integrated_2167.tex <==
{\color[rgb]{0.0,0.05,0.0}{{initially}}}
{\color[rgb]{0.0,0.272,0.0}{{a}}}
{\color[rgb]{0.0,0.13,0.0}{{pagan}}}
{\color[rgb]{0.0,0.278,0.0}{{culture}}}
{\color[rgb]{0.029,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.162,0.0}{{detailed}}}
{\color[rgb]{0.0,0.793,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.13,0.0}{{about}}}
{\color[rgb]{0.0,0.172,0.0}{{the}}}
{\color[rgb]{0.0,0.588,0.0}{{return}}}
{\color[rgb]{0.0,0.308,0.0}{{of}}}
{\color[rgb]{0.0,0.17,0.0}{{the}}}
{\color[rgb]{0.0,0.509,0.0}{{christian}}}
{\color[rgb]{0.0,0.609,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.127,0.0}{{the}}}
{\color[rgb]{0.298,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.038,0.0}{{during}}}
{\color[rgb]{0.0,0.377,0.0}{{the}}}
{\color[rgb]{0.0,0.3,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_salience_raw_2167.tex <==
{\color[rgb]{0.37,0.0,0.0}{{initially}}}
{\color[rgb]{0.238,0.0,0.0}{{a}}}
{\color[rgb]{0.166,0.0,0.0}{{pagan}}}
{\color[rgb]{0.319,0.0,0.0}{{culture}}}
{\color[rgb]{0.124,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.126,0.0}{{detailed}}}
{\color[rgb]{0.0,0.654,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.471,0.0}{{about}}}
{\color[rgb]{0.0,0.425,0.0}{{the}}}
{\color[rgb]{0.0,0.024,0.0}{{return}}}
{\color[rgb]{0.377,0.0,0.0}{{of}}}
{\color[rgb]{0.001,0.0,0.0}{{the}}}
{\color[rgb]{0.0,0.081,0.0}{{christian}}}
{\color[rgb]{0.0,0.068,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.048,0.0,0.0}{{the}}}
{\color[rgb]{0.538,0.0,0.0}{{islands}}}
{\color[rgb]{0.0,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.49,0.0}{{the}}}
{\color[rgb]{0.0,0.399,0.0}{{\textit{norse-era}}}}


==> examples/QLSTM_salience_raw_integrated_2167.tex <==
{\color[rgb]{0.044,0.0,0.0}{{initially}}}
{\color[rgb]{0.0,0.124,0.0}{{a}}}
{\color[rgb]{0.0,0.046,0.0}{{pagan}}}
{\color[rgb]{0.0,0.039,0.0}{{culture}}}
{\color[rgb]{0.046,0.0,0.0}{{,}}}
{\color[rgb]{0.0,0.076,0.0}{{detailed}}}
{\color[rgb]{0.0,0.645,0.0}{\underline{information}}}
{\color[rgb]{0.0,0.269,0.0}{{about}}}
{\color[rgb]{0.0,0.21,0.0}{{the}}}
{\color[rgb]{0.0,0.301,0.0}{{return}}}
{\color[rgb]{0.017,0.0,0.0}{{of}}}
{\color[rgb]{0.0,0.065,0.0}{{the}}}
{\color[rgb]{0.0,0.254,0.0}{{christian}}}
{\color[rgb]{0.0,0.256,0.0}{{religion}}}
{\color[rgb]{0.0,0.909,0.0}\textbf{{to}}}
{\color[rgb]{0.0,0.047,0.0}{{the}}}
{\color[rgb]{0.261,0.0,0.0}{{islands}}}
{\color[rgb]{0.1,0.0,0.0}{{during}}}
{\color[rgb]{0.0,0.339,0.0}{{the}}}
{\color[rgb]{0.0,0.313,0.0}{{\textit{norse-era}}}}

